How rotational invariance of common kernels prevents generalization in high dimensions

Kernel ridge regression is well-known to achieve minimax optimal rates in low-dimensional settings. However, its behavior in high dimensions is much less understood. Recent work establishes consistency for kernel regression under certain assumptions on the ground truth function and the distribution of the input data. In this paper, we show that the rotational invariance property of commonly studied kernels (such as RBF, inner product kernels and fully-connected NTK of any depth) induces a bias towards low-degree polynomials in high dimensions. Our result implies a lower bound on the generalization error for a wide range of distributions and various choices of the scaling for kernels with different eigenvalue decays. This lower bound suggests that general consistency results for kernel ridge regression in high dimensions require a more refined analysis that depends on the structure of the kernel beyond its eigenvalue decay.

==> sections/Sections_ICML/new_section1.tex <==
\begin{abstract}

Kernel ridge regression is well-known to be consistent and to achieve
minimax optimal rates in low-dimensional settings. However, its
behavior in high dimensions is much less understood.  Recent work
establishes consistency for kernel regression under certain
assumptions on the ground truth function or the distributions. In
this paper we show that the rotational invariance property of
commonly studied kernels (such as RBF, inner product
kernels and fully-connected NTK of any depth) induces a bias towards
low-degree polynomials in high dimensions. In particular, we prove
this statement for general distributions and are also the first to cover
different scalings of the normalization constant. Finally, by observing that in high-dimensional real-world
datasets the risk follows a U-curve even in noiseless settings,
we argue that our theory adds additional insights to the 
necessity of feature selection in high-dimensional kernel regression for common rotationally invariant kernels.
  
%%   %% as predicted by our theory 
%%   %% and hence our theory gives intuition why feature selection is essential to 
  
%% % Even though kernel ridge regression is well-known to be consistent and
%% % achieve minimax rate optimal in fixed dimensions, their behavior in
%% % the high-dimensional setting is much less understood.  
%% Kernel ridge regression is known to be consistent and achieve optimal minmax rate for a fixed input dimension. 
%% However, its behavior is less well understood in the high-dimensional regime where the input dimension increases with respect to the sample set size.
%% % 
%% % \nr{
%% % I think that starting with "even though" sounds bad. Also, the structure of the sentence is counterintuitive sometimes. I would reformulate as the following:\\
%% % "
%% % Kernel ridge regression is known to be consistent and achieve optimal minmax rate for fixed DATA (???) dimension. 
%% % However, ITS behavior is less well understood in the high-dimensional setting.
%% % " \\
%% % Also, not really clear to me what you mean: high-dimension is still fixed dimension anyway. Do you mean increasing dimension? or do you mean in the limit of increasing data dimension?
%% % }
%% Recent work
%% establishes consistency for interpolating estimators in high dimensions ,
%% feeding to 
%% % \nr{never heard "feed to" in this context, but maybe it's just me } 
%% the modern storyline of learning theory that regularization
%% becomes obsolete 
%% % \nr{redundant?}
%% with sufficient overparameterization. In this paper
%% we question this mindset and show that kernel regression in high
%% dimensions induces a bias towards polynomials with degree inversely
%% proportional to the growth of the dimension.
%% %independent of noise.
%% %\fy{careful bias vs. bias, independent of noise is probably unclear}
%% % \nr{This is a lot for an introduction for me, since we don't know what the "dimension independent of noise" is. Maybe use some term like
%% % "effective dimension" or equally vague, so that people want to know what it is but don't feel like they are expected to know already, as is not common terminology in the literature (as far as I know)
%% % }
%% %% consistency can in fact only be
%% %% achieved for low-degree polynomials in a wide variety of settings.
%% Our framework significantly extends previous
%% distributional assumptions, includes the flat limit scaling and covers
%% most commonly employed kernels such as RBFs, inner product kernels and
%% fully-connected NTK of any depth. 
%% % \nr{isn't NTK inner product? maybe something like \\
%% % "... includes the flat limit scaling and rotationally invariant and inner product kernels, encompassing most commonly employed kernels, such as RBFs and fully-connected NTK." \\
%% % Even though this proposal sentence is too long for an abstract maybe. Needs to be nicely formulated.
%% % }
%% %%  and for ridge and \kd{we always say 
%% %% kernel interpolation - remove “ridgeless”} regression alike.
%% %% Moreover, we are the first to also establish lower
%% %% bounds for the flat limit scaling.
%% Finally, we empirically confirm that the bias follows a U-curve on
%% real world data sets independent of regularization. We hence
%% conclude that feature selection is essential to achieve good
%% generalization performance for kernel methods in high dimensions.
%% %% Together with previous results this
%% %% implies that for ground truths beyond low-degree polynomials, the risk
%% %% of kernel regression asymptotically resembles a U-curve as a function
%% %% of the input dimension. In particular it does not exhibit double or
%% %% multiple descents as suggested in previous literature. We verify that
%% %% this behavior is indeed reflected in real world data sets and finally
%% %% conclude that feature selection is essential to achieve good
%% %% generalization performance for kernel methods in high dimensions.
\end{abstract}


\section{Introduction}
The classical learning theory literature
has traditionally focused on the good generalization properties
of kernel ridge regression, including numerous
consistency and minimax optimality results (e.g. \cite{Caponnetto07}).
Even though these classical statements successfully upper bound the
risk when the dimension $d$ is fixed and relatively small compared to
the number of samples $n$, modern data sets are often in the regime
where $d > 50$ is large and rather close to $n$ and previous theory
does not apply.  High-dimensional asymptotic theory
\cite{Buhlmann11,Wainwright19} aims to fill this gap by providing
bounds that assume $d,n \to \infty$ and are often much more predictive
of practical observations even for finite $d\sim 50$.

In this paper we prove inconsistency of regression with
rotationally invariant kernels in high dimensions. The lower bounds
hold for both ridge regression and minimum norm interpolation (also
referred to as ``ridgeless'' estimator).

%% study consistency of kernel regression in the
%% high-dimensional asymptotical limit for both ridge
%% regression and minimum-norm interpolation (also referred to as
%% \emph{ridgeless regression}).
Even though recent work such as \cite{Hastie19, Bartlett20} has
established explicit asymptotic upper bounds for the bias
and variance for high-dimensional linear regression, the situation is
less clear for kernel regression. While \cite{Ghorbani19, Ghorbani20,
  Liang20b} show that the variance decreases with dimension,
the bounds on the bias are inconclusive as they lead to contradictory intuitions for the behavior of the estimator on high dimensional problems. \kd{remove: they are considering
different assumptions on the distributions and ground truth functions.}

In particular in the regime $d\asymp n^{\beta}$ , \cite{Liang20b,
  Liang20a} convey a positive statement, and prove asymptotic
consistency for functions with asypmptotically bounded Hilbert
norm. On the other hand, \citet{Ghorbani19, Ghorbani20} shed a
negative light on regression
with rotation symmetric kernels by showing that
consistency is only possible when the ground truth is a low-degree
polynomial. While \cite{Liang20a, Liang20b} study
%with $\beta \in (0,1)$
anisotropic Gaussian inputs, \cite{Ghorbani19, Ghorbani20} are limited
in their analysis technique to cover data that is uniformly sampled on the
product of two spheres.

These two types of seemingly contradictory consistency results for
different distributional settings are based on vastly different proof
techniques. Hence, the following question naturally arises
\begin{center}
  \emph{Which functions can kernel methods consistently learn in high dimensions?}
\end{center}

In this paper we unify previous
distributional assumptions and domains in one proof framework
and thereby characterize how the rotational
invariance property of common kernels induces the kernel estimator to
asymptotically converge to a low-degree polynomial.
%% We identify 
%% that actually rotational invariance is the culprit in our proof.
Specifically, 
%% main contributions are as follows  then significantly extend
%% previous results and prove that
%% kernel methods cannot consistently
%% learn ground truth functions of degree higher than $2\floor{2/\beta}$ for:
we show that this \emph{polynomial approximation barrier} persists for
\begin{itemize}
\item  a broad range of common rotationally invariant kernels
  such as radial basis functions
(RBF) with vastly different eigenvalue decay rates, inner product kernels and Neural Tangent kernels (NTK)  \cite{Jacot20}
\item a broad range of distributions including anisotropic Gaussians
  where the degree of the polynomial depends only on the growth of $\effdim := \trace(\inputcov)/\opnorm{\inputcov}$
  and not on the specific structure of $\inputcov$.
% and the
% resulting distributions when projected on the sphere
%  independent of the shape of $\inputcov$
%   when $\effdim = \tr(\inputcov)$
  \item different scale parameters $\bw$ with $\kernf_{\bw}(\xk,\xkd) = \kernf(\xk,\xkd)$ \kd{not sure what to write instead of also:} beyond the classical choice of $\bw \asymp \effdim$ 
%   but also when $\bw$ increases or decreases faster than $\effdim$ 
    %   \nr{you never defined what $\bw$ is. Is it necessary or is it common enought in the literature to omit it?}
\end{itemize}
Our results demonstrate that whenever kernels are rotationally
invariant and the data is high-dimensional, kernel regression fails to
generalize unless the ground truth function is a lower degree
polynomial. This also implies that future work should focus on the symmetries respectively asymmetries of the kernel incorporating prior knowledge on the structure of the high dimensional problem instead of relying on the analysis of the eigenvalue decay.
\kd{
studying the effect of structure on kernel learning instead of
relying on the analysis of eigenvalue decay.}
%Important impact on future directions. The  suggests it's not 
%% In this paper, we define the effective dimension $\effdim := \trace(\inputcov)/\opnorm{\inputcov}$ as the normalized trace of the covariance matrix of the data and assume that $\effdim \asymp n^{\beta}$. 
% \fy{I kinda copied 3.3., have to see where to put what, is this too technical at this point?}

This paper is organized as follows.
First of all, we show in Section~\ref{sec:priorkernelwork} 
% \nr{No need for reference here, unless you are starting the "structure of the paper section".  Also, I see that sometimes you write "Section 2.2", but here you just wrote "2.2". Check for consistency.}
that the bounded norm assumption made in \cite{Liang20b,Liang20a} is violated even for simple functions
such as $\ftrue(x) = e_1^\top x$.  We then present our assumptions in
Section~\ref{sec:2} and present our main lower bounds on the generalization error in Section~\ref{sec:3}. Finally, we demonstrate in
Section~\ref{sec:exp} on real-world data how our theory explains why
feature selection is crucial for high-dimensional kernel learning even
in the noiseless setting.



%% In other words, our results further support the narrative
%% that the inductive bias of kernel regression towards
%% polynomials is inescapable in high-dimensional settings.



%% This has important practical implications. In particular, we discuss
%% in Section~\ref{sec:discussion} how this behavior 
%% %\fy{bad wording}
%% indicates that high-dimensional kernel learning for highly nonlinear
%% maps requires additional structural assumptions. We demonstrate this
%% hypothesis on real-world data in Section~\ref{sec:exp}, where we show
%% that feature selection is crucial for high-dimensional data to obtain
%% the minimum risk for both low and high noise settings.

%% and input covariances with fast
%% eigenvalue decay when $d\asymp n$ and identity covariances when $d
%% \asymp n^{\beta}$ with $\beta \in (0,1)$
%% the bias vanishes 
%% However, the assumption of an asymptotically bounded RKHS norm is
%% seldomly discussed. For example, even for a ground truth function that
%% only depends on few variables, the RKHS does not necessarily stay
%% bounded (Fig~\ref{fig:rkhsnorm}) as you add variables. This makes the
%% consistency results rather hard to interpret.
%% %% changes with the dimension $d$, for a given
%% %% sequence of ground truth functions it is not trivially to verify that
%% %% the bounded norm assumption holds true and thus the consistency
%% %% results apply. In fact, this doesn’t seem to be the case even for
%% %% sparse linear functions as shown in Figure \ref{fig:rkhsnorm}.
%% In another line of work, \cite{Ghorbani19,Ghorbani20} analyze
%% uniformly distributed data on the product of two spheres
%% without the bounded norm assumption and show
%% that in the regime $\effdim \asymp n^{\beta}$
%% %% where the data is uniformly distributed on the
%% %% product of two spheres
%% kernel regression can at most consistently
%% estimate low degree polynomials.

% \nr{I was once told that using "actually" in a paper sounds very strong for native speakers (I don't know, since I am not one :) ). While it makes sense in this context, it could maybe be omitted altogether}

%% Can kernel methods consistently learn functions beyond polynomials with kernels in high dimensions?}

  
%% Not sure you need this level of detail here  
%% the proofs make heavily use of the
%% restrictive assumptions and in particular of a Theorem in
%% \cite{Schoenberg1988} showing that any continuous rotationally
%% invariant kernel on the hyper sphere can be expressed as an inner
%% product kernel.
%% Given the literature, our paper extends the analysis
%% to a broader set of input distributions and asymptotic regimes to
%% answer the question

%% the proofs make heavily use of the
%% restrictive assumptions and in particular of a Theorem in
%% \cite{Schoenberg1988} showing that any continuous rotationally
%% invariant kernel on the hyper sphere can be expressed as an inner
%% product kernel.


%% Interestingly, the role of regularization becomes
%% less clear in such regimes. In particular, recent papers suggest favorable generalization
%% performance for minimum norm interpolators both empirically
%% \cite{Belkin18c,Geifman20} and theoretically
%% \cite{Liang20a,Liang20b}. This line of work is motivated by the
%% remarkable observation that deep neural networks can interpolate even
%% noisy training data while still generalizing well \cite{Zhang16}.
%% %% , there exists a surge of works
%% %% analyzing interpolating linear and kernelized estimators.
%% More precisely, under the assumption that the Hilbert norm of the ground
%% truth function remains bounded \cite{Liang20a, Liang20b} 
%% % \kd{but Liu is really a bit confusing here since it is for regression - I mean we do not care but reader might be confused} \fy{maybe: or
%% %the source condition parameter is lower bounded \cite{Liu20},
%% the authors show asymptotic consistency for input covariances with fast
%% eigenvalue decay when $d\asymp n$ and identity covariances when $d
%% \asymp n^{\beta}$ with $\beta \in (0,1)$.
%% %% show that consistency
%% %% can be reached in the regime $d \asymp n$ when the eigenvalues of the
%% %% covariance matrix of the data decays sufficiently fast. These results
%% %% have been extended in \cite{Liang20b} to the regime $d \asymp
%% %% n^{\beta}$ with $\beta >0$ where the covariance matrix is the
%% %% identity.


%% importance of regularization for kernel regression
%% % \kd{just remove this?:
%% % \cite{Golub79,Wahba90,Smola98,Shawe04,Evgeniou00,Devito05,Alvarez11}.}
%% % \fy{be more precise, e.g. don't really know what papers you'd expect there}
%% %That is, numerous results not only prove
%% and includes numerous consistency and minimax optimal 
%% % \nr{optimality} 
%% results (e.g. \cite{Caponnetto07}) for ridge regression. On the other hand, minimum norm
%% interpolation has recently been proven to be
%% inconsistent \cite{Rakhlin18} for the Laplace kernel.
%% %% proved that the minimum norm
%% %% Laplace kernel interpolator cannot be consistent when
%% %% i.i.d. Rademacher noise is added to the observations.
%% These \fy{which?} statements describe the asymptotic behavior \fy{not true, also non-asymptotic} of the
%% regression estimate when increasing the amount of data samples $n\to
%% \infty$ with constant dimension $d$. While these results give good
%% intuitions for settings where the dimension $d$ is relatively small
%% compared to $n$, this is often not the case in modern data sets where
%% the dimension $d$ can even exceed the amount of samples
% \fy{whats these citations?}
% \cite{Dua17,Li18}.

%% Instead, this paper analyzes the asymptotic
%% behavior of kernel regression in high dimensional regimes where both
%% $d,n\to\infty$. Although an increasing input dimension $d$ may seem
%% rather counter intuitive, many works from the high dimensional
%% statistics domain produce much more accurate predictions by studying
%% asymptotics in high dimensional regimes compared to the ones obtained
%% form a classical view point where the dimension $d$ remains
%% constant. We refer to standard works in this field
%% \cite{Wainwright19,Buhlmann11} and references therein.


% \nr{
% I have some general (very subjective) comments on this section: to me, it feels like there is way too much detail for an introduction, both in terms of precision of the statements (intro is not for precision, but for giving nice and broad context, vague statements are ok, as long as not incorrect).  For example, above the sentence "when $\tr(\inputcov) \asymp n^\beta$" could be omitted as it worsens the "information to noise ratio". The dotted list above could be omitted and compacted in a sentence (how comprehensive to make it is up to you, but I just feel that this is too much info here). \\
% Second, and important as well, is that there is no clear structure to the section. Usually the introduction is structured as [general story] $\rightarrow$ [structure (in section 2 we present ..., in section 3 we say..., etc...) $\rightarrow$ [contribution (sometimes, but maybe needed here to precisely highlight what's new wrt the enemy Ghorbani)]. \\
% Here instead, the contribution section is blended with the structure section, and it feels a little untidy.
% }

% \fy{the only thing is that hastie linear regression stuff
%   really suggests the same}



%% We conclude with 
%% One implication of our results is that when the ground truth function
%% depends nonlinearly on many features there is no hope to learn the
%% ground truth function using rotationally invariant kernels in high
%% dimensions.  On the other hand if it only depends on few dimensions,
%% our experiments suggest that the risk curve resembles a
%% U-shaped curve with respect to the input dimension for a fixed sample size. In fact, our experiments suggest that the increase in the risk is primarily due to a growing bias term with respect to the amount of features which aligns well with our theoretical predictions. This stands in stark contrast to the
%% double and multiple descent curves as suggested in
%% \cite{Liang20b}.
%% % \kd{don't get that: for certain ground truth functions that are
%% % also omnipresent in the linear interpolation literature
%% % \cite{Yang20,DAscoli19,Hastie19}}. 
%% Finally, we verify this behavior also for real world data sets (see Figure
%% \ref{fig:realworld}) and conclude that feature selection is indeed
%% often necessary to achieve good generalization even for ridge
%% regression, to control the bias.


%% of both lines of work
%% and consider distributions with covariance matrix $\inputcov$ in the
%% regime $\tr(\inputcov) \asymp n^{\beta}$ with $\beta >0$ \emph{and}
%% distributions where the data is additionally projected to the sphere.
%% We show that for this broad class of distributions, indeed, kernel
%% regression with rotationally invariant kernels cannot consistently
%% learn ground truth functions of degree higher than $2\floor{2/\beta}$
%% when $\tr(\inputcov) \asymp n^\beta$. The results hold for the
%% classical scaling $\bw = \effdim$ for common radial basis functions
%% (RBF), inner product kernels and Neural Tangent kernels (NTK)
%% \cite{Jacot20}.  Moreover, we are the first to prove that bias lower
%% bound persists for the flat limit when $\bw \to \infty$ for
%% $\alpha$-exponential kernels.

%% while we focus on the normalization or bandwidth parameter $\bw =
%% \effdim$ as in previous work, we are also the first to prove that the


%% The main contribution of this paper is to answer this question to the
%% negative for distributions with covariance matrix $\inputcov$ in the
%% regime $\tr(\inputcov) = \effdim \asymp n^{\beta}$ with $\beta >0$
%% \emph{and} when the data is projected to the sphere with commonly used
%% rotationally invariant kernels.  More specifically, we show that the
%% bias for both kernel ridge regression and interpolation, is lower
%% bounded by the projection error of the ground truth functions onto the
%% space of polynomials of degree at most $2 \floor{2/\beta}$.

%depending on the effective dimension $\effdim$ of the setting.
%% Our bound holds true for general distributions with
%% covariance matrix $\inputcov$ in the regime $\tr(\inputcov) = \effdim
%% \asymp n^{\beta}$ with $\beta >0$ and also still applies when the data
%% is furthermore projected to the sphere.
%% Our results use a unified proof technique the settings studied in
%% \cite{Ghorbani19,Ghorbani20,Liang20a,Liang20b,Liu20} that also allows
%% us to extend them to arbitrary $\inputcov$ as long as $\tr(\inputcov)
%% \asymp n^{\beta}$.
%% In fact, we show
%% that the noiseless estimator of bounded kernel functions converges
%% asymptotically in $L_2(P)$ norm to a polynomial. Furthermore, the
%% degree of the polynomial in our main theorem depends only on $\beta$
%% and not on the explicit structure of the covariance matrix. This
%% implies that the lower bound cannot be overcome by spiked covariance
%% data distributions.

%% While we focus on the scale parameter $\bw = \effdim$ as in previous
%% work, we also prove that the bias lower bound persists for the flat limit
%% when $\bw \to \infty$.

%% and prove for certain radial basis
%% function kernels including the Laplace kernel that the bias bound
%% persists even in the flat limit. This is also the point where we
%% empirically find that the bias attains its minimum for the Laplace
%% kernel.




%% Together with the fact \cite{Liang20b,Ghorbani19,Ghorbani20}
%% that the variance decreases with dimension, we further argue
%% in Section~\ref{sec:discussion} that the bias
%% lower bound implies that for a fixed sample size
%% the risk curve follows a U-shaped curve.
%% we can see that
%% the variance vanishes in high dimensions, resulting in a dominant bias
%% which steadily increases with respect to the dimension $d$. As a
%% result we conclude that the risk follows an U-shaped curve where the
%% variance decreases and the bias increases as the dimension grows.


%% Our research shows that even very simple (i.e. sparse) non
%% polynomial functions have a non vanishing bias in high dimensional
%% regimes. Therefore, assuming that the ground truth function depends on
%% many features we can conclude that there is no hope to learn the
%% ground truth function using rotationally invariant kernels due to a
%% non vanishing bias term.
%% \fy{dunno yet how to bring that in}
%% On the other hand, when the ground truth function only depends on few
%% dimensions, we can conclude that feature selection is necessary in
%% order to control the bias. We can also empirically observed this for
%% real world data sets in Figure \ref{fig:realworld}.
%  Finally, in the
% presence of noise we argue that ridge regularization is relevant to
% achieve optimal performance because we enter again a low dimensional
% regime after selecting the features.
% 





==> sections/Sections_ICML/new_section2.tex <==

\section{Problem setting}
\label{sec:2}


In this section, we briefly introduce kernel regression estimators in
reproducing kernel Hilbert space and subsequently introduce our assumptions on 
the kernel, data distribution and high-dimensional regime.
\kd{We then introduce our assumptions
on the kernel, data distribution and high-dimensional regime.}
%compare them to the assumptions made in related papers. 
% \nr{related work?}.


\subsection{Kernel Ridge Regression}
We consider nonparametric regression in a \emph{reproducing kernel
  Hilbert space} (RKHS, see e.g. \cite{Wahba90,Smola98})
with functions on the domain $\XX \subset \R^d$ induced by a positive
semi-definite kernel $\kernf: \XX \times \XX \to \R$. That is, for any
set of input vectors $\{\xind{1}, \cdots,\xind{m}\}$ in $\XX$, the
empirical kernel matrix $\kermat$ with entries $\kermat_{i,j} =
\kerfunc{\xind{i},\xind{j}}$ is positive semi-definite.  We denote by
$\langle.,.\rangle_{k}$ the corresponding inner product of the Hilbert
space and by $\| . \|_{\Hilbertspace} := \sqrt{\langle.,.\rangle_{k}}$
the corresponding norm.
% For more background we refer to standard literature on RKHS .


%% For every positive definite kernel, there
%% exists a unique corresponding reproducing kernel Hilbert space
%% $\Hilbertspace$ (RKHS, see standard sources
%% \cite{Wahba90,Berlinet04,Smola98}), consisting of functions mapping
%% $\XX$ to $\RR$.

%% that are aggregated to the data matrix $\datamatrix \in \XX^{n\times d}$ with rows $x_i$ and response vector $y\in\R^n$. 

We observe tuples of input vectors and response variables $(x,y) $
with $x \in \XX$ and $y \in \R$.  Given $\numobs$ samples, the ridge
regression estimator %% the ground truth function of
%% the underlying system by solving the following minimisation problem
minimizes the penalized square loss
\vspace{-0.1in}
\begin{equation}
\begin{split}
\label{eq:krr}
    \fhatridge = \underset{f \in \Hilbertspace}{\arg\min} ~~\sum_{i=1}^n \left(\y_i - f(\xind{i})\right)^2 + \lambda \| f \|_{\Hilbertspace},
    \end{split}
\end{equation} 
where $\lambda>0$ is the ridge parameter.  To attain consistency of
ridge regression as $n\to\infty$, $\lambda$ is usually chosen such
that $\frac{\lambda}{n} \to 0$. %sequence that vanishes.  Recently
Interpolants with zero training loss have attracted attention of the
theoretical community due to the curiously good generalization properties
of neural networks with zero training error.  In particular, both
\citet{Ghorbani19,Ghorbani20} and \citet{Liang20b,Liang20a} analyze the kernel
"ridgeless" estimate, or equivalently, the \emph{minimum norm
  interpolant}
 \begin{equation}
 \label{eq:constraint_min_p}
     \begin{split}
         \hat{f}_0 = \underset{f \in \Hilbertspace}{\arg\min} ~ \| f \|_{\Hilbertspace} ~~ \textrm{such that}~~ \forall i:~f(\xind{i}) = \y_i 
     \end{split}
 \end{equation}
Note that this is equivalent to taking $\lambda\to 0$ for the ridge
estimate in~\eqref{eq:krr} for fixed $n$.  The theoretical results in
Section~\ref{sec:3} hold for both ridge regression and the minimum
norm interpolant.
 
For evaluation, we assume that the observations are i.i.d. samples
from a joint distribution $(\xind{i}, y_i)_{i=1}^n \sim
\jointp{X}{Y}$, and we refer to $\ftrue(x) := \EE [y \mid X= x]$ as
the \emph{ground truth} function that minimizes the population square
loss $\EE (Y-f(X))^2$.  We evaluate the estimator using the population
risk conditioned on the input data $\datamatrix$
%, defined by
\begin{align}
    \label{eq:biasvariance}
    \begin{split}
    &\Risk(\fhatridge) \define \EEobs \|\fhatridge - \ftrue\|_{\Ell_2(\PP_X)}^2 \\ 
    &= \underbrace{\|  \EEobs \fhatridge - \ftrue  \|^2_{\Ell_2(\PP_X)} }_{=: \text{ Bias }\Bias}+ \underbrace{\| \EEobs \fhatridge - \fhatridge \|^2_{\Ell_2(\PP_X)}}_{=: \text{ Variance } \Var}. \nonumber
        \end{split}
\end{align}
where $\EEobs$ is the expectation over the observations $\y_i \sim
\PP(Y|X=\x_i)$. In particular, when $y = \ftrue(x) + \eps$, $\EEobs
\fhatridge$ is often equivalent to the noiseless estimator when
$\eps=0$. Consistency in terms of
$\Risk(\fhatridge)\to 0$ as $n \rightarrow \infty$ can only be reached
if the bias vanishes.  In this paper we lower bound the bias $\Bias$
which, in turn, implies a lower bound on the risk.


\subsection{Prior work on the consistency of kernel regression}
\label{sec:priorkernelwork}


For ridge regression estimates in RKHS, a rich body of work
shows consistency and rate optimality when
appropriately choosing the ridge parameter $\lambda$
%% for some sequence $\lambda \to 0$ as
%% $\numobs \to \infty$
both in the non-asymptotic setting, e.g.~\cite{Caponnetto07}, and the asymptotic
setting, e.g.~\cite{Christmann07}, as $n \to \infty$.  \kd{remove need space: It is well
known that in the fixed dimensional setting the risk vanishes for
general ground truth functions with bounded Hilbert norm when
appropriately choosing the ridge parameter $\lambda$.}

%% Motivated by deep overparametrized neural networks interpolating the
%% training data while still generalizing well,
Recent papers explicitly study the bias in the context of minimum norm
interpolation in kernel regression \cite{Liang20b,Liang20a}
and show how it vanishes when borrowing the condition from low-dimensional analysis that the
ground truth functions have bounded Hilbert norm.
\kd{
where it
is often treated as the ``easy'' part since interpolation usually has
lower bias than the regularized counterpart.  However, the authors
simply borrow the condition from low-dimensional analysis that the
ground truth functions have bounded Hilbert norm.}
Even though this
assumption is perfectly reasonable for a fixed ground truth and
Hilbert space, it is rarely discussed what it means for a sequence of functions
 to have asymptotically bounded norm as the dimension $\dim$
grows. After all, the Hilbert space and thus also the norm change with
$\dim$.

%Besides the fact that is hard to
%interpret consistency when $d$ grows with $n$, 

%% minimum norm interpolation in the kernel regression domain and even
%% prove consistency in the high-dimensional regime.  In particular, the
%% risk bounds in \cite{Liang20b,Liang20a} imply consistency under the
%% assumption that the Hilbert norm of the sequence of ground truth
%% functions stays asymptotically bounded as $d\to \infty$.
%This assumption was replaced in \cite{Liu20} for ridge
%regression with a weaker assumption on the source condition with
%constant parameter $r$.
%In the high-dimensional setting however,
%% However, it is rarely discussed which sequence of functions have this property
%% in high dimensions since the Hilbert space and thus also the norm change with $\dim$.

We now show how even innocuous functions might have diverging
Hilbert norm and hence question the generality of the consistency
results that rely on bounded Hilbert norm assumption
\cite{Liang20b,Liang20a}.\footnote{Although \citet{Liu20} replace the bounded Hilbert norm
  assumption with a weaker bounded source condition, we
  expect this condition not to hold with increasing dimension either.
  We defer the detailed discussion to future work.}
In particular, for tensor product kernels including exponential inner product kernels (also studied in \cite{Liang20b,Liang20a}) defined on $x,x'\in\XX^{\otimes d} \subset \RR^d$, 
we can show the following lemma. 

%% with
%% translation invariant $q^d: [-\frac{1}{2},\frac{1}{2}] \times
%% [-\frac{1}{2},\frac{1}{2}] \to \mathbb{R}$.
%% we show provide a rigorous
%% example: for tensor kernels of the form $\kerfunc{\xk}{\xkd} =
%% \prod_{j=1}^d q(x_j,x_j')$, any sparse product function of the form
%% $\ftrue(x) = \prod_{j=1}^d f_j(x_j)$ will have an Hilbert norm that
%% diverges, i.e. $\|\ftrue\|_\Hilbertspace \to \infty$ as $d\to\infty$.
\begin{lemma}[Informal]
  \label{lm:rkhs}
For any $f$ that is a non-constant sparsely parameterized product
function $f(\xk) = \prod_{j=1}^m f_j(\xel{j})$ for some fixed $m \in
\N$, %for any sequence $\Hilbertspace_d$ defined above,
\vspace{-0.1in}
\begin{equation*}
  \| f \|_{\Hilbertspace_d} \overset{d \to \infty}{\to} \infty.
\end{equation*}
\end{lemma}



\begin{figure}
    \centering
         \minipage{0.35\textwidth}
         \includegraphics[width=\linewidth]{Plots_v2/RKHSNorm.pdf}
         \vspace{-0.2in}
    \endminipage
    \caption{\small{The approximation of the Hilbert norm induced by the Laplace and exponential inner product kernels of the function $\ftrue(\x) = \x_1$ plotted with respect to the dimension $d$ on the space $\XX = [0,1]^d$. See Section ~\ref{sec:expnorm} for experimental details.}}
    \vspace{-0.20in}
    \label{fig:rkhsnorm}
\end{figure}



In words, for simple sequences of sparse product functions, the Hilbert norm
diverges as the dimension $d\to\infty$. The precise conditions on the
kernel and Hilbert norm sequence $\Hilbertspace_d$ can be found
in~\suppmat~\ref{sec:norm}. Figure~\ref{fig:rkhsnorm} illustrates this
phenomenon for $\fexp (x) = e_1^\top x$ for the Laplace and
exponential inner product kernel.
%% We can now illustrate the increasing Hilbert norm in Figure~\ref{fig:rkhsnorm} where we empirically show how for $\fexp (x) = e_1^\top x$ the Hilbert norm seems to diverge for common
%% kernels like the exponential inner and Laplacian
%% kernel. 
% 
% Note that for the Gaussian kernel we know form Theorem 4.44 \cite{Steinwart08} that any constant non zero function is not contained in the RKHS and hence neither any sparse function. 
% %In Appendix~\ref{sec:norm}, Theoretically, 


Do we really fail to learn sparsely parameterized functions
consistently or is it simply an artifact of the analysis in
\cite{Liang20b,Liang20a}?  A recent line of work by
~\citet{Ghorbani19, Ghorbani20} allows a clear but rather negative conclusion when
\kd{paints a clear but rather grim picture}
the data is restricted to be uniformly distributed on two
spheres. In particular, without requiring the Hilbert norm of
$\ftrue $ to be bounded for all $\numobs$, they prove that kernel
regression estimates can indeed only consistently learn polynomials of
degree at most $\frac{\log \numobs}{\log \effdim}$ (which we refer to
as the \emph{polynomial approximation barrier}).
While the results provide some intuition for the behavior of kernel
regression, the proofs heavily rely on significant simplifications
that hold for the rather specific distributional assumptions on the
sphere.  It is hence unclear whether they could generalize to more
general settings that include the ones in \cite{Liang20b}.

%% \fy{would cut or move:
%% For one, \cite{Schoenberg1988} showed how all rotationally
%% invariant kernels reduce on the sphere to inner product kernels allowing significant simplifications in the analysis. Moreover, the proof heavily relies on the uniform distribution assumption because this allows the use of the Gegenbauer polynomials as an orthogonal basis of $\Ell_2(\PP_X)$.}

This paper demonstrates that using a different proof technique
we can indeed show that the polynomial approximation barrier holds for a broad spectrum of data distributions
including the ones  studied in
\cite{Liang20b,Liang20a}. 

%% that enables a significant extensions of the assumptions 
%% imposing less restrictive assumptions could extend the \emph{polynomial
%%   approximation barrier} in \cite{Ghorbani19,Ghorbani20} to general distributions including the ones studied in
%% \cite{Liang20b,Liang20a}. 

\subsection{Our problem setting}
\label{sec:oursetting}

%\kd{Alex found this sentence confusing}
% The framework we study in this paper covers distributions that depend
% on a covariance matrix, both in $\R^d$ and projected onto a sphere.
% We now specify all relevant assumptions on the kernel and our model of
% the data distribution.
%% and the data
%% distribution.

The framework we study in this paper covers random variables that are
generated from a covariance matrix model, i.e. $\Xrv = \inputcov^{1/2}
\standardrv$ with vector $\standardrv$ consisting of i.i.d entries, or when additionally projected onto the sphere.
%% distributions obtained when additionally projecting
%% the data to the sphere.
We now specify all the relevant assumptions on
the kernel and data distribution.
%our model of the data distribution.

\paragraph{Kernels}

Throughout this paper, we focus on continuous and rotationally invariant
kernels. A vast majority of the commonly used kernels such as fully connected NTK, RBF and inner product kernels satisfy this property as they depend only on the squared
Euclidean norm of $\xk$ and $\xkd$ and the inner product
$\xk^\top\xkd$, i.e. there is a function $\rotkerfunc$ such
that we can write $\kerfunc{\xk}{\xkd} = \rotkerfunc(\|\xk\|_2^2,
\|\xkd\|_2^2, \xk^\top \xkd)$.
%% Most commonly used kernels fall into
%% this category, including any
%% radial basis function (RBF) and any inner product kernel, but also for
%% instance Neural Tangent Kernels (NTK) of fully connected networks
%% \cite{Jacot20,Arora19}.
% \nr{check ending of this sentence. Probably "this category, including any" should be commented as well.}
One set of assumptions on the kernel functions that are sufficient for
our main results involves local regularity of $\kernf$ around the
sphere where the data concentrates in high dimensions.
%% We additionally require the following assumptions to hold
%% for the kernel function $\kernf$ locally around the sphere where the
%% data concentrates in high dimensions.





  


\begin{itemize}
\item[\Akonebracket] \textit{Local power expansion}: 
  %% Define the neighborhood $\convergeset{\delta} \subset \R^d \times \R^d$  as
  %% \begin{equation*}
  %% \begin{split}
  %%   \convergeset{\delta} :=& \{(\xk,\xkd) \in  \R^d \times \R^d \mid \\
  %%   &(\|\xk\|_2^2, \|\xkd\|_2^2) \in [1-\delta, 1+\delta] \times
  %% [1-\delta, 1+\delta]\}.
  %% \end{split}
  %% \end{equation*}
%   A kernel $\kernf$ has a local power expansion if $\rotkerfunc$ can be expanded as a power series
  The function $\rotkerfunc$ can be expanded as a power series
  \begin{equation}
    \label{eq:kerneldefg}
    \begin{split}
    \kerfunc{\xk}{\xkd} &= \rotkerfunc(\|\xk\|_2^2, \|\xkd\|_2^2, \xk^\top \xkd) \\
    &= \sum_{j=0}^{\infty} \rotkerfunccoeffj{j}(\|\xk\|_2^2,\|\xkd\|_2^2) (\xk^\top \xkd)^j 
    \end{split}
   \end{equation}
  that converges for $\xk, \xkd$ in a neighborhood of the sphere
  %\begin{equation*}
  $\{x\in \R^d \mid \|x\|^2 \in [1-\delta,1+\delta]\}$
  %\end{equation*}
  for some
   $\delta > 0$. Furthermore, all $g_i$ are positive semi-definite
   kernels.

\item[\Aktwobracket] \textit{Restricted Lipschitz
  continuity:} The restriction of $k$ on $\{(x,x)| x \in \R^d,
 \| x \|_2^2 \in [1-\delta_L, 1+\delta_L]\}$ is
  a Lipschitz continuous function for some constant $\delta_L>0$.
%   \nr{how about saying "is L-Lipschitz continuous..."? otherwise L is not defined}
\end{itemize}

Furthermore, independent of \Akone-\Aktwo, our results also hold for \emph{$\alpha$-exponential}
kernels that are defined as $k(\xk,\xkd) = \exp(- \|\xk -
\xkd\|_2^\alpha ) $ for $\alpha \in (0,2)$. We show in
  Corollary~\ref{cor:kernels} that these assumptions cover a
  broad range of commonly studied kernels in practice.
  %% and any constant $\tau_0 \in
  %% \mathbb{R}$ following a slightly different proof technique without
  %% relying on the assumptions \Akone-\Aktwo.

  
  

  
  
  
\paragraph{Data Distribution and scale parameter}
In the sequel we denote by $a \asymp b$ that asymptotically as
$n\to\infty$, the ratio $\frac{a}{b}$ converges to a positive constant
$\frac{a}{b}\to \gamma>0$.

  
\begin{figure*}[t]
  \begin{center}
     \begin{subfigure}{0.32\textwidth}
       \includegraphics[width=\linewidth]{Plots_v2/beta_F2.pdf}
       \vspace{-0.2in}
       \caption{Ground truth $\ftrue = 2 \xel{1}^2$}
       \label{fig:fig2a}
     \end{subfigure}
     \begin{subfigure}{0.32\textwidth}
       \includegraphics[width=\linewidth]{Plots_v2/beta_F3.pdf}
       \vspace{-0.2in}
       \caption{Ground truth $\ftrue = 2 \xel{1}^3$}
       \label{fig:fig2b}
     \end{subfigure}
          \begin{subfigure}{0.32\textwidth}
       \includegraphics[width=\linewidth]{Plots_v2/sin_curve.pdf}
       \vspace{-0.2in}
       \caption{Degeneration of estimator}
       \label{fig:sine}
     \end{subfigure}
     \vspace{-0.1in}
     \end{center}
    
     
\caption{\small{(a) and (b): The bias of the minimum norm interpolant
    $\Bias(\fhatinterpol)$ normalized by $\Bias(0)$ as a function of
    $\beta$ for (a) different
    covariance models $\prob_1$- $\prob_3$  (see Section \ref{sec:expsynthetic}) with
    $n=4000$ and (b) different choices of $n$ and samples generated from an isotropic Gaussian with $d = \floor{n^{\beta}}$ ($\prob_1$). The horizontal lines $\textbf{B}(f_{\textrm{lin}})$ correspond to the risk of the optimal
    linear model for the different input data distributions. (c): The minimum norm interpolator/ridgeless estimate $\fhatinterpol$ of  $\ftrue(\x) = \sin(2\pi
    \xel{1})$  plotted in the
    direction $\ev_1$ through $(0,1/2,\cdots,1/2)$ when fitting noiseless observations with covariates drawn uniformly from $[0,1]^d$ with $n=100$ and varying $d$.
    %% for 
    %% respect to $\xel{1}$ and $\xel{i} = 1/2$ for all $i>1$ for
    %% distinct choices of the dimensions $d$. In total $100$
    %% i.i.d. samples are drawn uniformly from $[0,1]^d$ with noiseless
    %% observation generated from $\ftrue(\x) = \sin(2\pi \xel{1})$.
}}

\label{fig:polymodels}
\vspace{-0.2in}
\end{figure*}

\begin{itemize}
\item[\Adonebracket] \textit{Covariance model}: For symmetric matrices
  $\inputcov \in \R^{d\times d}$, we refer to $\effdim \define
  \trace(\inputcov)/\opnorm{\inputcov}$ as the effective dimension. The input data distributions are then elements of one of the following sets depending
  on $\inputcov$:
  %% $\prob_X \in
  %% \probsetcov$ or $\prob_X \in \probsetsphere$ dependent on $\inputcov$ defined as:
 \begin{equation}
 \begin{split}
    \probsetcov &= \{\prob_X \mid X = \inputcov^{\frac{1}{2}} \standardrv \text{ with } \standardrv \sim \prob^{\otimes d}, \prob \in \probsetw \} \\
  \probsetsphere &= \{\prob_X \mid X = \sqrt{\effdim} \frac{Z}{\|Z\|} \text{ with } Z \sim \prob \in \probsetcov\} \nonumber
 \end{split}
 \end{equation}
 % this does not belong in formal assumption
 where the set $\probsetw$
 contains the normal distribution and any almost surely bounded zero
 mean and unit variance distribution. 
\item[\Adtwobracket] \textit{High dimensional regime}: We assume that
  the trace of $\inputcov$ grows with the sample size $\numobs$ as
  $\effdim \asymp n^{\beta}$ with
  $\beta \in (0,1]$. 
\end{itemize}
In the sequel we assume without loss of generality that for simplicity $\opnorm{\inputcov}=1$ and hence $\effdim =
  \trace(\inputcov)$. In words, when $\prob_X \in \probsetcov$, the data has covariance
$\inputcov$, and when $\prob_X \in \probsetsphere$, the data can be generated by
projecting $Z\sim \prob_Z \in \probsetcov$ onto the sphere of radius
$\sqrt{\effdim}$, but unlike \citet{Ghorbani19,Ghorbani20} we do not enforce the random variable to be uniformly distributed. \kd{i have added the last sentence} 
%is the covariance matrix of the data. 
In our analysis, the kernel function $\rotkerfunc$ itself stays
constant for any $d$. However as $\effdim, n\to\infty$ we
need to adjust the scaling of the input as the norm concentrates
around $\EE~ \| \x \|_2^2 = \effdim$.  
% I would remove this comment since the scaling is important for any kernel functions
% The
% scaling is especially crucial for NTK, where the correspondence with
% infinitely wide neural networks, to the best of our knowledge, only
% holds for test samples $\frac{\Xrv}{\sqrt{\bw}}$ on the sphere (see e.g.
% Theorem~3.2~\cite{Arora19}). 
Hence, as $\numobs
\to\infty$, we consider the sequence of scale dependent kernels
\vspace{-0.05in}
\begin{equation}
  \label{eq:scalekernel}
  \sckerfunc{\bw}{x}{x'} = \rotkerfunc\left(\frac{\|\xk\|_2^2}{\bw},
  \frac{\|\xkd\|_2^2}{\bw}, \frac{ \xk^\top \xkd}{\bw}\right)
\end{equation}
where $\bw$ can vary with sample size $\numobs$. In Section~\ref{sec:tauconst} we study
the standard scaling $\frac{\bw}{\effdim}\to c>0$, which leads to a non vanishing and non diverging expected squared norm $\EE~ \| \x \|_2^2/\bw \to c$,
% Why is this comment causing an error - strange
%\fy{ have to decide about using $ \effdim $ or just trace}
before discussing $ \frac{\bw}{\effdim} \to 0$ and $
\frac{\bw}{\effdim}\to \infty$ respectively in
Section~\ref{sec:otherbw}.
Our distributional assumptions include and generalize previous
works, which are summarized in Table~\ref{tab:settings}.

  

% I would not mention this because we actually recover their settings. 
% For RBFs, $\bw$ is
% simply the bandwidth, for inner product kernels and NTKs, it's usually
% set to $\bw = d$
% \cite{Ghorbani19,Ghorbani20,ElKaroui10,Liang20a,Liang20b,Liu20}. As a result, any
% input sample has expected norm . In fact, our choice of the
% scale parameter recovers all all the previously studied settings as discussed 
% in the next paragraph. The only case which we do not cover is the one in 
%% Our setting covers a very broad range of
%% settings.

%% For example, \cite{ElKaroui10,Liang20a,Liu20} consider $\prob_X \in \probsetcov$ with
%% $\tr(\inputcov) \asymp d$ and scale parameter $\bw = d \asymp \effdim$
%% and \cite{Liang20b} when $d \asymp n^{\beta}$ and $\inputcov =
%% \idmat_d$ for $\beta \in (0,1)$.
%% %% First of all, we directly recover the setting studied in the
%% %% papers \cite{ElKaroui10,Liang20a,Liu20} when $d \asymp n$ and
%% %% $\tr(\inputcov) \asymp d$ and the one studied in the paper
%% %% \cite{Liang20b} when $d \asymp n^{\beta}$ and $\inputcov =
%% %% \idmat_d$. Furthermore we recover
%% Furthermore, \cite{Ghorbani19, Ghorbani20} study $\prob_X \in
%% \probsetsphere$ for $\inputcov = \idmat_d$ respective $\inputcov =
%% UU^\top + d^{-\kappa} \idmat$ (using notation as in \cite{Ghorbani20}
%% Sec 2.1.)
%% %% choosing $\inputcov = \idmat_d$ respective $\inputcov = UU^\top +
%% %% d^{-\eta} \idmat$ (using notation as in \cite{Ghorbani20} Sec 2.1.)
%% %% and projecting the data onto the sphere.
%% %We also cover $\tr(\inputcov)/d \to 0$ in
%% Finally, we refer to Section \ref{sec:otherbw} for the case where 
%% $\tr(\inputcov)/d \to 0$ in \cite{Liang20a,Liu20}.

%% This case is discussed in Section
%% \ref{sec:otherbw} where we cover special cases for
%% $\frac{\bw}{\effdim} \to 0$ and $\to\infty$.  we remark that
%% for $\tr(\inputcov)/d \to 0$, the upper bounds of the variance
%% in \cite{Liang20a,Liu20} diverge 
%% resulting in an diverging upper bound of the variance of the minimum
%% norm interplators in \cite{Liang20a}. 



%% \citet{Liang20a} derive a bound for the risk
%% for kernel "ridge-less" regression in high dimensional settings based
%% on the bias-variance decomposition. While the bound of the Variance
%% \cite[Theorem~2]{Liang20a} only applies to the specific setting used
%% in the paper, the authors highlight that their bound on the bias
%% \cite[Theorem~3]{Liang20a} does only make very few assumptions and
%% thus can be applied to much more general settings. Informally stating,
%% the bound has the form
%% \begin{equation}
%% \label{eq:rakhlinbound}
%%     \Bias \leq \| \ftrue \|_{\Hilbertspace} ~C_1(\lambda_1(\kermat),..., \lambda_n(\kermat)) + C_2(n),
%% \end{equation} 
%% where $C_2(n) \to 0$ as $n \to \infty$ and $C_1(\lambda_1(\kermat),..., \lambda_n(\kermat))$ depends only on the eigenvalues of the empirical kernel matrix $\kermat$. In particular, under the assumption that the Hilbert norm $\| \ftrue \|_{\Hilbertspace}$ stays bounded for any d, \citet{Liang20a} shows that the Bias can vanish even in high dimensional regimes. Unfortunately, this assumption is not further discussed in the paper and simply assumed to be true. \\
%% As a first step in this paper, we highlight that the RKSH norm $\| \ftrue \|_{\Hilbertspace}$ can go to infinity as $d \to \infty$ even for very simple ground truth functions $\ftrue$. Therefore, we can conclude that although $C_1\to 0$ from Equation ~\ref{eq:rakhlinbound}, we can not conclude that the Bias vanishes for general ground truth functions. In fact, we will see that our observations hold true for very simple functions, and therefore, as a conclusion we question whether the assumption that the Hilbert norm $\| \ftrue \|_{\Hilbertspace}$ is bounded holds true for any function of practical interests.



%% Assuming that the input data is spherical, it is sufficient for our analysis to impose the following assumptions for the kernel $k_{\Sphere}: \Sphere^{d-1} \times \Sphere^{d-1} \to \RR$: 
%% \begin{itemize}
%%     \item[(B.1)] The kernel $k_{\Sphere}$ is positive definite, continuous and rotationally symmetric. 
%% \end{itemize}
%% For the more general case where the input data is not spherical but
%% lives in $\RR^d$

%% A well-known result by Schoenberg \cite{Schoenberg1988} then implies
%% that the restriction of $\kernf$ onto the sphere can be expressed as
%% an inner product kernel $\kressphere(\xk,\xkd) = \rotkerfunc(\xk^\top
%% \xkd)$ where $\rotkerfunc$ is a sum of Gegenbauer polynomials. When 
%%  $\rotkerfunc$ is locally analytic around $0$ we can write
%% \begin{equation}
%% \label{eq:Scheonbergseries}
%%     \rotkerfunc(\xk^\top \xkd) = \sum_{j=0}^{\infty} \rotkerfunccoeff (\xk^\top \xkd)^j
%% \end{equation}
%% with constants $\rotkerfunccoeff$ in $\RR$. \fy{RBF not included anymore?}
%% When the data lies on the sphere $\XX \subset \Sphere{d-1}$, our main
%% results are relatively easy to show using the series
%% expansion~\eqref{eq:Scheonbergseries}.  For data distributions on more
%% general $\XX \subset \R^d$ we require a few additional assumptions on the kernel function.
%%  Based on the decomposition we get form
%% Schoenberg's theorem \cite{Schoenberg1988}, we  extend the power
%% series to also include terms depending on the squared euclidean norm
%% of $\xk$ and $\xkd$:
%% Where $g_i: \R\times \R \to \R$ are some
%% functions depending only on the squared Euclidean norm of $\xk$ and
%% $\xkd$. Assuming that this power series converges for any $\xk,\xkd
%% \in \RR^d$ would be overly restrictive. In fact, we only
%% require that it converges in certain neighbourhoods of the hyper
%% sphere. More detailed, we assume that the kernel function $k:
%% \RR^d\times \RR^d \to \RR$ satisfies the
%% following assupmtions.



  %%   In  particular, there exists a power series as described in Equation
  %% \ref{eq:kerneldefg}, for which we can find $\delta>0,\delta'>0$ such
  %% that for any
  %% $(x,x') \in \RR^d \times \RR^d$, with
  %% $(||\xk||_2^2, ||\xkd||_2^2) \in [1-\delta, 1+\delta] \times
  %% [1-\delta, 1+\delta]$ and $\xk^\top \xkd \in [-\delta',\delta']$, the
  %% power series converges and equals $k(\xk,\xkd)$.  In particular, we
  %% assume that the function $g$ from Equation \ref{eq:kerneldefg} is
  %% continuous and for any $i \leq \floor{2/\beta}+1$, $g_i$ is
  %% $(\floor{2/\beta}+1-i)$-times continuously differentiable in an
  %% neighbourhood of $(1,1)$.
  
  
  
%% This fact
%% follows  trivially  from  the  local  Taylor  expansion  around  zero,
%% $h(\xk^\top\xkd) = \sum_{j=0}^{\infty} h_i  ~ (\xk^\top \xkd)^j$.
%% In addition, Proposition ~\ref{prop:ntkass} shows that the Assumptions
%% also hold true for NTK \fy{NTK kernels is doppelt gemoppelt} of any
%% depth and a broad range of different activation functions. For RBF
%% kernels we can show that the Gaussian kernel $k(\xk,\xkd)$ satisfies
%% the assumptions, since $\exp(- \| \xk - \xkd \|_2^2) =
%% \sum_{j=0}^{\infty} \frac{2^j}{j!}  (\xk^\top\xkd)^j \exp(\|\xk\|_2^2
%% + \| \xkd \|_2^2)$. Yet, it is not exactly which other RBF kernel
%% functions satisfy the Assumption B.3. 


%% --- Moved this part back to after thm 3.1
%% As a result, for this case it is
%% sufficient to require that the assumptions A.1 and A.2 hold true for
%% the restriction of the kernel function onto the hyper sphere $
%% \kernfuncressphere{d}$ \fy{why not need A.3?}. In fact, assumption A.2 holds trivially true
%% since any inputs $\x$ has norm $1$ by assumptions. Furthermore, we
%% know from \citet{Schoenberg1988} that any continuous rotational
%% symmetric function on the hyper sphere can be written as an inner
%% product kernel, i.e. $\kernfuncressphere{d}(\xk,\xkd) =
%% \rotkerfunc(\xk^\top \xkd)$, which we know from the previous
%% discussion satisfies assumption A.1-A.3 under weak assumptions.


  
%% More generally, our high-dimensional regime covers
%% $\frac{\trace(\inputcov)}{\|\inputcov\|_2} \asymp n^\beta$
%% Note that
%% the only restriction which we impose on the dimension $d$ of the input
%% data $d$ is that $\trace(\inputcov) \leq d$, which is a consequence of
%% the fact that $\| \inputcov \|_2 = 1$. Together with the assumption
%% that $\trace(\inputcov) \asymp n^{\beta}$, we cover a very broad range
%% of settings including the ones studied in
%% \cite{ElKaroui10,Liang20a,Liang20b}.
%% \newline Furthermore, we study the case where the data
%% is obtained by normalising $\xi{i}$, i.e.
%% \begin{equation}
%%     \s_i =\xind{i}/ \|\xind{i} \|_2^2
%% \end{equation}
%% This results in the case where the data is distributed on the hyper sphere. As a consequence, our results can be extended to cover the settings studied by \citet{Ghorbani19,Ghorbani20}.





%respectively $\kernfsphere$ \fy{this is
%  not true, the $\kerfunc$ changes domain so can't stay the same}
%% remain the same for any $d$. To react on the change of the dimension
%% $d$, we study scale dependent kernels $k_{\bw}$ with
%% $\sckerfunc{\bw}{x}{x'} = \rotkerfunc(\frac{\|\xk\|_2^2}{\bw},
%% \frac{\|\xkd\|_2^2}{\bw}, \frac{ \xk^\top \xkd}{\bw}) $. 
%% The
%% assumption that the kernel function depends on a scale parameter which
%% changes with respect to $d$ is common practice in the literature
%% \cite{Ghorbani19,Ghorbani20,ElKaroui10,Liang20a,Liang20b,Liu20}, where
%% all cited papers choose $\bw = d$.
%% We remark that in the asymptotic setting, some dependence of
%% $\bw$ on $d$ is required in order to adapt to the changing
%% norm of the vectors $\xind{i}$.
%% More, generally, the expected norm depends on the effective dimension
%% \begin{equation}
%%   \label{eq:effdim}
%%     \effdim \define \EE~ \| \x \|_2^2  = \trace(\EE \x \x^\top) = \trace(\inputcov) 
%% \end{equation}
%% Most of the discussion in this paper will focus on the choice of
%% $ \bw = \effdim$. We also provide ...



% 
% \begin{itemize}
% \item[(B.1)] \textit{Kernel has a local power expansion}:
%   Define the neighborhood $\convergeset{\delta}{\delta'} \subset \R^d \times \R^d$  as
%   \begin{equation*}
%     \convergeset{\delta}{\delta'} := \{(\xk,\xkd) \in  \R^d \times \R^d \mid (\|\xk\|_2^2, \|\xkd\|_2^2) \in [1-\delta, 1+\delta] \times
%   [1-\delta, 1+\delta] \:\text{ and }\: \xk^\top \xkd \in [-\delta',\delta']\}.
%   \end{equation*}
%   
%   A kernel $\kernf$ has a local power expansion if $\rotkerfunc$ can be expanded as a power series
%   \begin{equation}
%     \label{eq:kerneldefg}
%     \kerfunc{\xk}{\xkd}= \rotkerfunc(\|\xk\|_2^2, \|\xkd\|_2^2, \xk^\top \xkd) = \sum_{j=0}^{\infty} \rotkerfunccoeffj{j}(\|\xk\|_2^2,\|\xkd\|_2^2) (\xk^\top \xkd)^j 
%    \end{equation}
%    that converges in a neighborhood $\convergeset{\delta,\delta'}$ of the sphere for some $\delta, \delta'>0$ and where $g_i$ is
%   $(\floor{2/\beta}+1-i)$-times continuously differentiable in an
%   neighbourhood of $(1,1)$.   
%   %%   In  particular, there exists a power series as described in Equation
%   %% \ref{eq:kerneldefg}, for which we can find $\delta>0,\delta'>0$ such
%   %% that for any
%   %% $(x,x') \in \RR^d \times \RR^d$, with
%   %% $(||\xk||_2^2, ||\xkd||_2^2) \in [1-\delta, 1+\delta] \times
%   %% [1-\delta, 1+\delta]$ and $\xk^\top \xkd \in [-\delta',\delta']$, the
%   %% power series converges and equals $k(\xk,\xkd)$.  In particular, we
%   %% assume that the function $g$ from Equation \ref{eq:kerneldefg} is
%   %% continuous and for any $i \leq \floor{2/\beta}+1$, $g_i$ is
%   %% $(\floor{2/\beta}+1-i)$-times continuously differentiable in an
%   %% neighbourhood of $(1,1)$.
% \item[(B.2)] \textit{Restricted Lipschitz
%   Continuity:} The restriction of $k$ on $\{(x,x)| x \in \R^d,
%   \| x \|_2^2 \in [1-\delta_L, 1+\delta_L]\}$ is
%   a Lipschitz continuous function for some constant $\delta_L>0$.
% \end{itemize}
% 
% \fy{replace A and B throught text}
% We remark that the Assumptions (B.1) and (B.2) apply to a very broad
% range of kernels including RBF, inner product and NTK kernels. More
% generally, any inner product kernel $\kerfunc{\xk}{\xkd} =
% \rotkerfunc(\xk^\top \xkd)$ with $\rotkerfunc$ locally analytic around
% zero satisfies the assumptions.
% %% This fact
% %% follows  trivially  from  the  local  Taylor  expansion  around  zero,
% %% $h(\xk^\top\xkd) = \sum_{j=0}^{\infty} h_i  ~ (\xk^\top \xkd)^j$.
% Similarly,
% the  Assumptions  hold  true  for   any  RBF  kernel  $k(\xk,\xkd)  =
% \rotkerfunc(\| \xk - \xkd \|_2^2)$ which is locally analytic
% around $2$. We  refer to Lemma ~\ref{lm:RBFass} for a proof. Finally,
% Proposition ~\ref{prop:ntkass}  shows that  the Assumptions  also hold
% true for the NTK  kernels of any depth and a  broad range of different
% activation functions.
% 

%% The motivation for our choice of the
%% scale parameter is that the re-scaled inputs have squared mean
%% $\EE \| \bw \xind{i} \|_2^2 =1$.

%% \fy{completely rewrite}
%%  We remark that our choice of
%% the scale parameter only agrees with the one from the mentioned paper
%% if $\effdim = d$. While this is the case for the paper
%% \cite{Liang20b} and also for the paper \cite{Ghorbani19} when
%% projecting onto the hyper sphere, we


%% \paragraph{Kernel regression}

%% Don't see how we need this
%% As a consequence, we can see that
%% the bias $\Bias(\fhatridge)$ can be expressed as
%% \begin{equation}
%% \label{eq:biassimplified}
%%    \Bias(\fhatridge) = \EE_{X} \| \EE_y \fhatridge(X) - \ftrue(X) \|^2, 
%% \end{equation}
%% where $\ftrue(\textbf{\x})$ is the vector with entries $\ftrue(\datamatrix)_i
%% = \ftrue(\xi{i})$ and $\kstar(X)$ is the vector with entries $\kstar_i =
%% k_{\tau}(\xind{i}, X)$. Finally, the same applies for the spherical input
%% data, where for some random input $\Srv$ on the hyper sphere
%% $\Sphere$, we write $\kstar_{\Sphere}$ instead of $\kstar(X)$,
%% $\kermat_{\Sphere}$ instead of $\kermat$ and $\ftrue(\Ss)$ instead of
%% $\ftrue(Xs)$.






==> sections/Sections_ICML/new_section3.tex <==




%     Observe that a phase transition occurs bias
%     drops to zero at $\beta = 0.5$ respectively $0.33$. 
%     The phase
%     transitions hence scale with the inverse of the polynomial degree
%     the ground truth, in line with Theorem~\ref{thm:main_thm}.}


\section{Main Results}
\label{sec:3}

We now present our main results that hold for a wide range of
distributions and kernels and show that
kernel methods can at most consistently learn low-degree polynomials.
%% lower bound the bias for both
%% kernel ridge and ridgeless regression and hence show inconsistency of
%% kernel estimators for all but low-degree polynomials.
%% The proof heavily relies on the fact that asymptotically, the
%% noiseless estimator can be approximated with high probability by a
%% low-degree polynomial.  
%% asymptotically almost
%% everywhere like a polynomial with bounded degree. This insight
%% underlies our main theorem on the inconsistency of kernel estimation
%% for all but a very limited set of ground truth functions.
Section~\ref{sec:tauconst} considers the case $\bw \asymp \effdim$
while Section~\ref{sec:otherbw} provides lower bounds for
the regimes $\frac{\bw}{\effdim} \to 0$ and $\frac{\bw}{\effdim} \to\infty$.

%% Our results therefore build upon the
%% intuitions gained from the papers \cite{Ghorbani19,Ghorbani20} and
%% extend them to a much broader class of data distributions. \kd{Not
%%   sure how much more we need to say here- i feel it becomes a bit
%%   repetitive. }  \kd{Say something like in a first step of this
%%   section blabla}


\subsection{Inconsistency of kernel regression for $\bw \asymp \effdim$}
\label{sec:tauconst}


%% The functions for which kernel estimation can reach consistency lies
%% in the space of polynomials of degree at most some constant integer $m$ depending only on $\beta$.
%% For the brevity and clarity of our results, Theorem
%% ~\ref{thm:main_thm} only shows the case where the bandwidth is chosen
%% to be $\bw = \effdim$ as defined in Section~\ref{sec:oursetting}. The
%% more general case where $\bw \asymp \effdim$ follows then trivially
%% from a straightforward modifications of the results.
For simplicity of exposition, we present a result for the case $\bw=\effdim$ based on the assumptions \Akone-\Aktwo. The more general case $\bw\asymp\effdim$ is deferred to \suppmat~\ref{sec:proofmainthm}.
% We can now present our main result that is stated for
% $\bw = \effdim$, but holds more generally for $\bw\asymp\effdim$
% when appropriately scaling the assumptions. 
% %are modified appropriately.
In the sequel we denote by $\polyspace{m}$ the space of polynomials of
degree at most $m \in \N$.
% \nr{You repeated "we present..." twice, and at the beginning of other sections. Can you change it here? Also, what do you mean by "scaling the assumptions"? Do you have the complete proof in the appendix? If so, you can write 
% "For simplicity of exposition, we present a result for the case $\bw=\effdim$. The more general case $\bw\asymp\effdim$ is deferred to Appendix 1234."
% }
%% The case where $\bw
%% \asymp \effdim$ follows then after a trivial modifications of the
%% results.

%% Denoting $\xel{j}$
%% as the $j$-th entry of the vector $\x\in\R^d$, the space is formally
%% defined as
%% \begin{equation*}
%%   \label{eq:polys}
%% \polyspace{m} =
%% \left\{ \sum_{j = 1}^{l} c_{j} \prod_{i=1}^d (\xel{i})^{\alpha_{j}^i}
%% \lvert l \in \NN, c^l_{j} \in \RR, \alpha_{j}^i \in \NN, \sum_{i=1}^d
%% \alpha_{j}^i \leq m \right\}.
%% \end{equation*}
%% where $\x_{(i)}$ is the $i$-th entry of
%% the vector $\x$.


%%%%%%%%%%%%%%%%%%%%5%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% Theorem: Poly approx %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\begin{figure*}[t]
\begin{subfigure}{0.32\linewidth}
    \centering
    \includegraphics[width=\textwidth]{Plots_v2/TauLaplace.pdf}
           \vspace{-0.2in}
    \caption{Laplacian kernel}
    \label{fig:taulaplace}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.32\linewidth}
    \centering
    \includegraphics[width=\textwidth]{Plots_v2/TauGauss.pdf}
           \vspace{-0.2in}
    \caption{Gaussian kernel}
    \label{fig:taugauss}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.32\linewidth}
    \centering
    \includegraphics[width=\textwidth]{Plots_v2/TauExp.pdf}
       \vspace{-0.2in}
    \caption{Exponential inner product kernel}
    \label{fig:tauexpo}
  \end{subfigure}  
  \vspace{-0.10in}
%%      \minipage{0.32\textwidth}
%%      \includegraphics[width=\linewidth]{Plots_v2/TauLaplace.png}
     
%% \endminipage
%%      \minipage{0.32\textwidth}
%%   \includegraphics[width=\linewidth]{Plots_v2/TauGauss.png}
%% \endminipage
%%      \minipage{0.32\textwidth}
%%   \includegraphics[width=\linewidth]{Plots_v2/TauExp.png}
%% \endminipage
\caption{\small{The bias of the minimum interpolant
    $\Bias(\fhatinterpol)$ normalized by $\Bias(0)$ as a function of the normalization constant
    $\bw$ for different choices of $d = \effdim$.
  %% and (a) Laplacian kernel, \textbf{Middle:} Gaussian kernel and
  %% \textbf{Right:} exponential inner product kernel.
  The ground truth function is $f(x) = 2\xel{1}^3$ and $n= 2000$ noiseless
  observations are fit where the input vectors are sampled from an isotropic Gaussian with $d = \floor{n^{1/2}}$.}}
\label{fig:taudependence}
\vspace{-0.2in}
\end{figure*}

\begin{theorem}[Polynomial approximation barrier]
  \label{thm:main_thm}
  Assume that the kernel $\kernf$, respectively its restriction onto the sphere $\kernfuncressphere{d}$ satisfies \Akone-\Aktwo~or is an $\alpha$-exponential kernel.
  %% , is the $\alpha$-exponential kernel with $\alpha\in (0,2)$ or satisfies the assumptions \Akone - \Aktwo.
  Furthermore assume that the ground truth $\ftrue$ is bounded almost surely
  and the input distribution satisfies \Adone-\Adtwo.
  %% is bounded $|\ftrue| \leq \ubfunc$ almost surely for some $\ubfunc >
  %% 0$.
  Then, for some $m \in \NN$ specified below, the following results hold for both the ridge~\eqref{eq:krr} and ridgeless estimator~\eqref{eq:constraint_min_p} $\fhatridge$ 
  \begin{enumerate}
%   \item There exists a polynomial $\polyf \in \polyspace{m}$ so that for any  $\eps>0$ and as $n \to \infty$,  
%   with probability $\geq 1- \exp(-\Cgenprob{\epsd}
%   \log(n)^{((1+\epsilon)/2ilon)/2d})$ over the draws of a test sample $\Xrv$, 
%   \begin{equation}
%     \label{eq:polyapprox}
%     \left| \EEobs \fhatridge(\Xrv) - \polyf(\Xrv) \right| \leq \epsilon
%     ~~ a.s.,
%   \end{equation}
%     where $\EEobs \fhatridge(\Xrv)$ is the estimator with expectation
%   taken over the observation noise \nr{which noise? maybe I missed it, but up to now we never talked about noise. Wasn't it simply intended as the expectation of $Y \sim P(Y \vert X)$?}. 
%   with probability $\geq 1- \exp(-\Cgenprob{\epsd}
%   \log(n)^{((1+\epsilon)/2ilon)/2d})$ over the draws of a test sample $\Xrv$, 
%   \begin{equation}
%     \label{eq:polyapprox}
%     \left| \EEobs \fhatridge(\Xrv) - \polyf(\Xrv) \right| \leq \epsilon
%     ~~ a.s.,
%   \end{equation}
%     where $\EEobs \fhatridge(\Xrv)$ is the estimator with expectation
%   taken over the observation noise \nr{which noise? maybe I missed it, but up to now we never talked about noise. Wasn't it simply intended as the expectation of $Y \sim P(Y \vert X)$?}. 

  \item The bias of the kernel estimators $\fhatridge$ is
    asymptotically lower bounded for any $\eps > 0$ as $n\to \infty$,
    \vspace{-0.05in}
  \begin{equation}
    \label{eq:biaslb}
    \Bias(\fhatridge) \geq \underset{\polyf \in
      \polyspace{m}}{\inf} \| \ftrue -
    \polyf \|_{\Ell_2(\prob_X)} - \eps ~~~a.s. 
  \end{equation}
\item For bounded kernel functions on the support of $\prob_X$ the averaged estimator $\EEobs \fhatridge$ converges in $\Ell_2(\prob_X)$ to a polynomial $\polyf  \in \polyspace{m}$  as $n \to \infty$,
  \vspace{-0.1in}
  \begin{equation}
  \label{eq:polyapproxlp}
    \left\| \EEobs \fhatridge - \polyf \right\|_{\Ell_2(\prob_X)} \to 0
    ~~ a.s..
  \end{equation}
  \end{enumerate}
  \vspace{-0.1in}
  More precisely, if $g_i$ is $(\floor{2/\beta}+1-i)$-times
  continuously differentiable in a neighborhood of $(1,1)$ and there
  exists $\jthresh > \floor{2/\beta}$ such that
  $\rotkerfunc_{\jthresh}(1,1) >0$, then the
  bounds \eqref{eq:polyapproxlp},\eqref{eq:biaslb} hold with $m = 2
  \floor{2/\beta}$ for $\prob_X
  \in \probsetcov$ and $m = \floor{2/\beta}$ for $\prob_X
  \in \probsetsphere$.
  %% where we additionally assume that $g_i$
  %% is $(\floor{2/\beta}+1-i)$-times continuously differentiable in a
  %% neighborhood of $(1,1)$ and there exists $\jthresh >
  %% \floor{2/\beta}$ such that $\rotkerfunc_{\jthresh}(1,1) >0$:
  %% More precisely,
  %% \begin{enumerate}
  %%   \item when $X$ is drawn from a distribution that satisfies
  %%     Assumptions A.1-A.2, the bias lower bound~\eqref{eq:biaslb} and
  %%     polynomial approximation~\eqref{eq:polyapprox} hold with $m = 2
  %%     \floor{2/\beta}$.
  %%   \item When $X = \frac{Z}{\|Z\|}$ with $Z$ drawn from a
  %%     distribution that satisfies Assumptions A.1-A.2, the bias lower
  %%     bound~\eqref{eq:biaslb} and polynomial
  %%     approximation~\eqref{eq:polyapprox} holds
  %%     %%  for all kernel functions
  %%     %% restricted to the sphere $\kressphere(\xk,\xkd) = \rotkerfunc(\xk^\top \xkd)$ with $\rotkerfunc$ locally analytic around $0$ and 
  %%     with $m = \floor{2/\beta}$.
  %%   %% \item Assume that the eigenvalues of $\kermat$ are lower bounded.
  %%   %%   Then above results also hold for the minimum norm interpolator
  %%   %%   $\fhatinterpol$ in~\eqref{eq:constraint_min_p}
  %% \end{enumerate}

  %%   The results hold trivially for $\lambda \geq c > 0$ and for decaying
  %% $\lambda \to 0$ and $\lambda = 0$ (the minimum norm interpolator
  %%   $\fhatinterpol$ in~\eqref{eq:constraint_min_p}) if the
  %%   eigenvalues of $\kermat$ are lower bounded by a positive constant for all $n 
\end{theorem}

Corollary~\ref{cor:kernels} gives examples for kernels that satisfy the
assumptions of the theorem.
The almost sure statements refer to the distribution over the input
data but hold also true with probability $\geq 1- \exp(-\Cgenprob{\epsd}
   \log(n)^{(1+\epsilon')/2})$ over the draws of $\X$ (see
remark ~\ref{rm:astoinp} for further details). 
% \nr{doesn't almost sure convergence always imply convergence in probability?}.  

The first point in Theorem \ref{thm:main_thm} shows that even with
noiseless observations, the estimator
$\fhatridge$ can at most consistently learn ground truth functions $\ftrue$
that are a polynomial of degree less than $m$. 
We refer to $m$ as the $\beta$-dependent
\emph{polynomial approximation barrier}
%% formalized in form of a lower
%% bound on the bias in the second part of
%% Theorem~\ref{thm:main_thm}.
While the first point only implies that the bias and hence also the
risk cannot vanish if the ground truth function is not a polynomial,
we show in the second part of Theorem~\ref{thm:main_thm} that the
averaged estimator $\EEobs \fhatridge$ converges in the
$\Ell_2(\prob_X)$ to a polynomial of degree at most $m$ when the
kernel is bounded on the support of
$\prob_X$.\footnote{In~\suppmat~\ref{sec:prop1_proof} we provide a
  closed form expression for the polynomial in the proof of the
  Theorem \ref{thm:main_thm} and show that the statement also holds
  for bounded observations $y_i$.}  We refer
to~\suppmat~\ref{sec:proofmainthm} for a slightly weaker statement
which also includes unbounded kernels. Figure \ref{fig:sine}
illustrates how the estimator converges to polynomials with lower
degrees as dimension grows when $\ftrue$ is the sine function.
%% can be consistently
%% approximated in $\Ell_2(\prob_X)$-norm by a polynomial of degree at
%% most $m$
%% Furthermore, we can straight forwardly see from the proof
%% in~\suppmat~\ref{sec:prop1_proof} that the statement also holds for
%% the estimator $\fhatridge$ assuming that the observations $\y_i$ are
%% bounded.


Further the reader might note that \citet{Ghorbani20} achieve a lower
barrier $m=\floor{1/\beta}$ for their specific setting which
demonstrates that our results are not exactly tight. However, this was
not our main focus in this work as our the main message is to
illustrate the generality of the settings for which consistency
\emph{cannot be reached}. We leave consistency results in for our general settings  and tighter bounds as interesting future work.
We now present a short proof sketch to both provide intuition for why
the polynomial approximation barrier holds. For a full proof see~\suppmat~\ref{sec:proofmainthm}.
%% and highlight the technical
%% difficulties.
%% The same
%%   argument holds for $\prob_X \in \probsetcov$ and with an extra
%%   factor of $2$ for other kernels that satisfy \Akone-\Aktwo.
  %% \kd{we cover also far more
  %%   general kernels than just RBF and NTK, though they do not have a
  %%   name}\fy{check}
%We provide the full proof in \suppmat~\ref{sec:proofmainthm}.
  
%% The second statement explicitly illustrates that kernel regression
%% estimators cannot be consistent if the ground truth cannot be
%% approximated by a polynomial of degree at most $m$. We call this
%% limitation the \textit{polynomial barrier} which is clearly only
%% occurring in high dimensional regimes for universal kernels like the
%% Gaussian kernel.




\paragraph{Proof sketch}
The proof of the main theorem is primarily based
 on the concentration Lipschitz continuous functions of vectors with i.i.d. entries. In fact, we can show that
%  of the
% maximum of $\numobs$ inner products in high dimensions, i.e. that with
% high probability
\vspace{-0.1in}
\begin{equation}
\label{eq:concentration}
    \underset{i}{\max}\frac{\left| \xind{i}^\top \Xrv  \right|}{\bw} \leq n^{-\beta/2}(\log n)^{(1+\epsilon)/2} ~~~a.s.
\end{equation}
where we use $\trace(\inputcov) \asymp \numobs^\beta$.
For smooth inner product kernels (or any kernel on the sphere) $\kernf_{\bw}$, the local series expansion (we use assumption \Akone~ and hence also the rotational invariance of $\kernf$) takes a simple form and almost surely reads
\vspace{-0.1in}
\begin{equation}
    \kernf_{\bw}(\xind{i},\Xrv) = \sum_{j=0}^{m} g_j ~
    \left(\frac{\xind{i}^\top\Xrv}{\bw}\right)^j 
    +
    O\left(n^{-\theta} \right)
 \end{equation}
with $\theta$ some constant such that $1<\theta <(m+1)\frac{\beta}{2}$
that exists because $m\geq \floor{2/\beta}$. Hence, as $n\to\infty$,
$ \kernf_{\bw}(\x_i, X)$ converge to low-degree polynomials.
%% we can approximate
%% the vector $\kervec$ with entries $\kervec_i = \kernf_{\bw}(\x_i, X)$
%% in $\ell_1$ norm by a vector of low degree polynomials.
Using the closed form solution of $\fhatridge$ based on the
representer theorem we can hence conclude the first point in Theorem
\ref{thm:main_thm} given that $\kermat +\lambda I \succ cI$ for some
constant $c>0$.  For ridge regression $\lambda$ is usually lower
bounded and hence the result follows naturally. However for the
minimum norm interpolator, we also need to show that the eigenvalues
of the kernel matrix $\kermat$ itself are asymptotically lower bounded
by a positive non-zero constant.  The main technical difficulty is
then to show that this holds true for kernels beyond inner product
kernels where $g_j$ is no longer a constant. \qed \\
% and in particular for the
% $\alpha$-exponential kernels for $\alpha\in (0,2)$. There, it is not
% even clear whether $g_j$ are positive semi-definite and we are forced to 
% use a completely different proof technique.  \qed \\

% %% As a result, the kernel function $k$ looks like a polynomial of degree at most $m$ plus an error term which vanishes at rate $o(n^{-1})$ with high probability over the draws of $\Zrv$ and almost surely over the draws of $\Z = \{\z_1,...,\z_n\}$ .
% % Maybe not that important here, already cite him enough
% %We can then apply a
% %similar argument to the one used in \cite{ElKaroui10} to
% For the case of minimum norm interpolation, we can also use the above
% expression to show that the eigenvalues of the kernel matrix $\kermat$
% with entries $K_{ij}=\kernf_\bw(x_i,x_j)$ are almost surely lower
% bounded by a positive constant. By the representer theorem, the
% regression estimate can then be written in closed form for any
% $\lambda\geq 0$ as
% %% is a linear combination
% %% of $\kerfunc{x_i}{X}$ and we can write for any $\lambda \to 0$ and
% %% $\lambda >0$
% \begin{equation}
% \label{eq:biaslower}
%     \fhatridge(x) = \y^\top (\kermat + \lambda \idmat_n)^{-1}\kerx{x}
% \end{equation}
% where $\kerx{x} \in \R^n$ has entries $\kerx{x} =
% \kernf_{\bw}(\xind{i}, x)$.  Hence, asymptotically, the estimate
% $\fhatridge$ can be approximated arbitrarily well by an $m$-th degree
% polynomial with high probability. The bias lower bound
% ~\eqref{eq:biaslower} follows after controlling the influence
% of the low probability regions on the bias.\qed \\


%   The two additional $\beta$-dependent
% conditions on the kernel function $\kernf$ in Theorem
% ~\ref{thm:main_thm} ensure smoothness and that the eigenvalues of the
% kernel matrix are lower bounded, since $(\X^\top \X)^{\circ \jthresh}
% \to \idmat$ in operator norm with $\circ$ being the Hadamard
% product. Similar assumptions can also be found in previous works
% \cite{Liang20b,Ghorbani20}. It is straight forward to verify that all
% kernels discussed in Section ~\ref{sec:oursetting} satisfy these
% conditions hold for any $\beta>0$. 
% 


%% We want to close this section by a short discussion of the assumptions
%% on the kernel. First of all, the two additional $\beta$-dependent
%% conditions on the kernel function $\kernf$ in Theorem
%% ~\ref{thm:main_thm} ensure smoothness and that the eigenvalues of the
%% kernel matrix are lower bounded, since $(\X^\top \X)^{\circ \jthresh}
%% \to \idmat$ in operator norm with $\circ$ being the Hadamard
%% product. Similar assumptions can also be found in previous works
%% \cite{Liang20b,Ghorbani20}. It is straight forward to verify that all
%% kernels discussed in Section ~\ref{sec:oursetting} satisfy these
%% conditions hold for any $\beta>0$. 


The assumptions in Theorem \ref{thm:main_thm} cover a broad range of
commonly used kernels, including the ones in previous works. The
following corollary summarizes some relevant special cases
\begin{cor}
\label{cor:kernels}
Theorem \ref{thm:main_thm} applies to
\begin{enumerate}
 \item The exponential inner product kernel
 \item The $\alpha$-exponential kernel for $\alpha \in (0,2]$ 
 \item The fully-connected NTK of any depth with regular activation functions including the ReLu
\end{enumerate}
\end{cor}

The precise regularity conditions of the activation functions for the
NTK and the proof can be found
in~\suppmat~\ref{sec:proofcrkernels}. In addition, we provide a
detailed comparison with the kernels discussed in previous works
in~\suppmat~\ref{sec:discussionass}.
%\kd{do we really need to  introduce homogenity and Hermite polynomials here?}
% \kd{ This is repetitive:
% \Akone-\Aktwo hold for the exponential inner
% product kernel, the Gaussian kernel and NTK of any depth and a broad
% range of activation functions (Proposition ~\ref{prop:ntkass}).}

%% Besides, the Assumptions in Theorem \ref{thm:main_thm} include the
%% inner product kernels studied in \cite{Liang20b,Liang20a} and
%% \cite{Ghorbani19,Ghorbani20}. These kernels are of particular
%% relevance since we already know form \citet{Schoenberg1988} that any
%% continuous rotationally invariant kernel function can be expressed by
%% an inner product kernel.  In this case the the assumptions simplify
%% drastically, as
%% $\kernfuncressphere{d}(\xk,\xkd)=\rotkerfunc(1,1,\xk^\top \xkd) =
%% \sum_{j=0}^{\infty} \rotkerfunc_j~(\xk^\top \xkd)^j$.  In the case
%% when $\XX=\R^d$ our assumptions allow more general kernel functions
%% beyond NTK and inner product kernels studied
%% in~\cite{Liang20b,Liang20a}. We refer to Appendix
%% ~\ref{sec:discussionass} for a detailed comparison with the
%% literature.

% 
% When comparing our assumptions with the literature, it is important to
% distinguish between the two domains $\XX = \R^d$ and $\XX =
% \Sphere{d}$. In particular when restricted to
% $\XX=\Sphere{d}$ as in \cite{Ghorbani19,Ghorbani20},
% \citet{Schoenberg1988} shows that any continuous rotationally invariant
% kernel function can be expressed by an inner product kernel.
% In this case the the assumptions simplify drastically, as
% $\kernfuncressphere{d}(\xk,\xkd)=\rotkerfunc(1,1,\xk^\top \xkd) =
% \sum_{j=0}^{\infty} \rotkerfunc_j~(\xk^\top \xkd)^j$.
% In the case when $\XX=\R^d$ our assumptions allow more general kernel
% functions beyond NTK and inner product kernels studied
% in~\cite{Liang20a,Liang20b}. We refer to~\suppmat
% ~\ref{sec:proofmainthm} for a detailed comparison with the
% assumptions in the literature.


%% $\alpha$-exponential kernels $\kerfunc{\xk}{\xkd} = \exp(- \| \xk -
%% \xkd \|_2^\alpha)$ for $\alpha \in (0,2)$ although they follow a
%% slightly different proof technique.




%% \kd{ i think this is enough, we refer to the appendix
%%   for a detailed discussion where we compare which IP exactly are
%%   covered}\fy{no, i'm left hanging here as a reader if you don't tie
%%   it back}
%% Our
%% assumptions for this type of kernels largely overlaps with the ones
%% in~\cite{Ghorbani20,Liang20b} and hold true for very general kernel
%% functions including any of the studied kernels in the mentioned
%% papers.
% 
% \begin{remark}
%   \label{rm:rbf}
%   %Under the assumption that
%   When the eigenvalues of $(K + \lambda I)$ are almost surely lower bounded by a non zero positive constant, the assumptions \Akone-\Aktwo~ can be replaced by weaker assumptions including general RBF kernels. For instance, this holds trivially true when the ridge parameter $\lambda \geq c_{\lambda}>0$ is bounded away from zero.  We refer to Proposition \ref{prop:main_thm_ext} in the~\suppmat~ for more details.
%   
%   
% %   we do not explicitly require that the eigenvalues of
% %     For ridge regression estimates where \kd{I see why you want to say this but i am not sure whether this is needed: $\frac{\lambda}{n}\to 0$ } but
% %   $\lambda>0$, \Akone-\Aktwo~can be replaced by weaker assumptions as
% %   we do not explicitly require that the eigenvalues of $K$ are almost
% %   surely lower bounded by a positive non zero constant. 
% %   For
% %   interpolation, we can allow weaker versions of \Akone-\Aktwo The
% %   assumptions \Akone-\Aktwo~can be replaced with weaker assumptions
% %   including more general RBF functions given that the eigenvalues of
% %   $K$ are almost surely lower bounded by a positive non zero
% %   constant.\fy{i still think this is a bit weird because aren't you
% %     essentially trying to characterize when this is true, so why do
% %     you say: if this is true, we need fewer assumptions...} 
% %   }
%   
%   
% %   For ridge regression estimates where \kd{I see why you want to say this but i am not sure whether this is needed: $\frac{\lambda}{n}\to 0$ } but
% %   $\lambda>0$, \Akone-\Aktwo~can be replaced by weaker assumptions as
% %   we do not explicitly require that the eigenvalues of $K$ are almost
% %   surely lower bounded by a positive non zero constant. 
% %   For
% %   interpolation, we can allow weaker versions of \Akone-\Aktwo The
% %   assumptions \Akone-\Aktwo~can be replaced with weaker assumptions
% %   including more general RBF functions given that the eigenvalues of
% %   $K$ are almost surely lower bounded by a positive non zero
% %   constant.\fy{i still think this is a bit weird because aren't you
% %     essentially trying to characterize when this is true, so why do
% %     you say: if this is true, we need fewer assumptions...}  We refer
% %   to Proposition \ref{prop:main_thm_ext} in the~\suppmat~ for more
% %   details.
% %   }
% \end{remark}


\begin{savenotes}
\begin{table*}[ht!]
  {\small
    \begin{center}
%      \begin{minipage}
\begin{tabular}{c|c|c|c|c|c|c }
  Functions $f^\star$ & Kernels & Domain & Choice of $\bw$ &
  $\inputcov$ & Regime & Paper \\ \hline & & & & & &
  \\ $ \polyspace{m}$& \vtop{\hbox{IP, $\alpha$-exp,}\hbox{ NTK}} &
  $\RR^d$, $\Sphere{d}(\sqrt{\effdim})$ & \vtop{\hbox{$\bw =
      \effdim$}\hbox{$~~~= \tr(\inputcov)$}} & arbitrary $\inputcov$ &
  $\effdim\asymp n^{\beta}$ & Ours \\ $\polyspace{m}$& RBF &$\RR^d$,
  $\Sphere{d}(\sqrt{\effdim})$ & $\bw \to \infty$ & arbitrary
  $\inputcov$ & $\effdim \asymp n^{\beta}$ & Ours
  \\ $\|\ftrue\|_{\Hilbertspace} = O(1)$& IP, NTK & $\RR^d$ & $\bw =
  d$ & $\inputcov = \idmat_d$ & $d \asymp n^{\beta}$ &
  ~\cite{Liang20b} \\ $\|\ftrue\|_{\Hilbertspace} = O(1)$\footnotemark &IP,
  RBF& $\RR^d$ & $\bw = d$ & \vtop{\hbox{$\tr(\inputcov) \asymp
      d$}\hbox{$\tr(\inputcov)/d \to 0$}} & $d \asymp n$ &
  \vtop{\hbox{~\cite{Liang20a},}\hbox{~~~~~\cite{Liu20}}}
  %% \\
  %% $\|\ftrue\|_{\Hilbertspace} = O(1)$ $^{**}$ &IP,RBF& $\RR^d$ &
  %% $\bw = d $ & $\tr(\inputcov)/d \to 0$ & $d \asymp n$ &
  %% \vtop{\hbox{~\cite{Liang20a},}\hbox{~~~~~\cite{Liu20}}}
  \\
  $\polyspace{m'}$ & IP, NTK & $\Sphere{d}(\sqrt{\effdim})$ & $\bw = d $
  & $ \inputcov = \idmat_d$ & $d \asymp n^{\beta}$ &
  ~\cite{Ghorbani19}
  \\
  $\polyspace{m'}$ & IP, NTK &
  $\Sphere{d}(\sqrt{\effdim})$ & \vtop{\hbox{$\bw \approx
      \effdim$}\hbox{$~~~\asymp \tr(\Sigma_d)$}} & \vtop{\hbox{$\strut
      \inputcov = UU^\top $}\hbox{$ + d^{-\kappa}\idmat $}} & $\effdim
  \asymp n^{\beta}$ & ~\cite{Ghorbani20} \\
\end{tabular} \vspace{-0.1in} 
% \end{minipage}
  \end{center}}
 \caption{\small{
   Compilation of the different settings studied in the literature and our paper.
   The left-most column denotes the necessary conditions on the
   function space of the ground truth $\ftrue$ for the corresponding
   consistency results. 
   %% Note that any continuous rationally invariant kernel on the sphere is an inner product kernel.
   Here, $m = 2\floor{2/\beta}$ and $m' = \floor{1/\beta}$. The
   RBF kernels require different additional assumptions that we discuss in detail~\suppmat~\ref{sec:discussionass}.
   %% $^{(\star)}$: RBFs with polynomial eigenvalue decay rate of order $d+\alpha$ and $\alpha<2$. $\|\ftrue\|_{\Hilbertspace} = O(1)$,
 }}
 \label{tab:settings}
 \vspace{-0.2in}
\end{table*}
\end{savenotes}

\subsection{Inconsistency of kernel interpolation for $\bw \not\asymp \effdim$}
\label{sec:otherbw}

As Section~\ref{sec:tauconst} establishes the polynomial approximation
barrier for the classical scaling $\frac{\bw}{\effdim} \asymp 1$, an
important question remains unaddressed: can we avoid it with different
scalings?  When $\frac{\bw}{\effdim} \to 0$, intuitively the estimates
converge to the zero function almost everywhere and hence the bias is
lower bounded by the $\Ell_2(\prob_x)$ norm of $\ftrue$ implying that
no function can be learned consistently (see~\suppmat~
\ref{sec:simplertaucase} for a rigorous statement).  When $\bw$
increases faster than $\effdim$, however, the behavior is unclear a
priori. Simulations in Figure~\ref{fig:taulaplace}, \ref{fig:tauexpo}
suggest that the bias could in fact decrease for $\bw \gg \effdim$ and
attain its minimum at the so called \emph{flat limit}, when $\bw \to
\infty$.  To the best of our knowledge, the next theorem is the first
to show that the polynomial approximation barrier persists in the flat
limit for RBF kernels whose eigenvalues do not decay too fast.


%%%%%%%%%%%%%%%%%%%%5%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% Theorem: different tau %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{theorem}
  \label{thm:otherchoicesoftau}
   Let $\kernf$ be an RBF kernel with Fourier transform
 $\ftkernf$ such that for any $d$, $\underset{\|\theta\| \to
   \infty}{\lim} \|\theta\|^{d+\alpha} \ftkernf(\theta) = \cphi > 0$
 for some $\alpha \in(0,2)$.
Under the assumptions \Adone-\Adtwo~
%of Theorem~\ref{thm:main_thm}
on the data distribution, the polynomial approximation bound~
  \eqref{eq:polyapproxlp} and bias lower bound \eqref{eq:biaslb}
  hold for the flat limit interpolator $\underset{\bw \to \infty}{\lim}\fhatinterpol$ with the same $\beta$-dependence for $m$ as in Theorem~\ref{thm:main_thm}.
 %%  of, and again with
 %% $m = 2
 %%  \floor{2/\beta}$ for $\prob_X
 %%  \in \probsetcov$ and $m = \floor{2/\beta}$ for $\prob_X
 %%  \in \probsetsphere$.
%\end{enumerate}
% Under the assumptions \Adone-\Adtwo~
% %of Theorem~\ref{thm:main_thm}
% on the data distribution, the bias of the minimum norm interpolator
% \eqref{eq:constraint_min_p} in the flat limit
% $\bw\to\infty$ satisfies
% %% \begin{enumerate}
%% \item If $\frac{\bw}{\effdim} = \Omega(n^\eps)$ for any $\eps>0$,
%%   %that is $\bw = \Omega(n^{-\beta+\epsilon})$,
%%   asymptotically as $n\to\infty$
%%     \begin{equation}
%%     \Bias(\fhatridge)\geq \EE_{\Xrv} \left| \ftrue(\Xrv) \right|^2 - \gamma  ~~~ a.s..
%% \end{equation} 
%For the minimum norm interpolator, when $\bw \to 0$
% 
% \begin{equation}
%      \lim_{\bw \to \infty} \Bias(\fhatinterpol) \geq  \underset{\polyf \in \polyspace{m}}{\inf} \| \ftrue - \polyf\|_{\Ell_2(\prob_X)}^2  - \gamma ~~~a.s.
% \end{equation}

% 
% 
%  for any $\gamma >0$ and any RBF kernel with Fourier transform
%  $\ftkernf$ such that for any $d$, $\underset{\|\theta\| \to
%    \infty}{\lim} \|\theta\|^{d+\alpha} \ftkernf(\theta) = \cphi > 0$
%  for some $\alpha \in(0,2)$, and with $m = 2
%   \floor{2/\beta}$ for $\prob_X
%   \in \probsetcov$ and $m = \floor{2/\beta}$ for $\prob_X
%   \in \probsetsphere$.
% %\end{enumerate}
\end{theorem}

In particular, the assumptions hold for instance for the
$\alpha$-exponential kernels with $\alpha \in (0,2)$ (see
\cite{Blumenthal60}) and the popular Matern RBF kernels with $\nu <2$.
The proof  of the theorem can be found in~\suppmat~\ref{sec:flatlimit} and is based on the flat limit literature on RBFs
\cite{Lee2014,Driscoll02,Schaback05,Larsson05}
%% and holds true for any
%% RBF function with polynomial eigenvalue decay of rate $d +\alpha$ for
%% $\alpha \in (0,2)$.  This holds for instance of $\alpha$-exponential
%% kernels with $\alpha \in (0,2)$ (see \cite{Blumenthal60}) and 
%% the popular Matern RBF kernels with $\nu <2$.
While Theorem \ref{thm:otherchoicesoftau} only applies for the
interpolating estimator $\fhatinterpol$, we argue that the bias
can only increase with the ridge penalty and hence attains
its minimum at $\lambda = 0$.
%% is well known to control the bias variance trade-off and
%% hence we expect the bias to be minimal for $\lambda = 0$.

% \fy{need here?}In fact, for
% the $\alpha$-exponential kernel, we can directly show
% in~\suppmat~\ref{sec:simplertaucase} that the flat limit solution of
% $\fhatridge$ with $\lambda>0$ is just a constant.

\footnotetext{ \cite{Liu20} actually requires the weaker assumption that the source condition parameter $r>0$.}

%(see e.g. \cite{Rasmussen03} Chapter 4).
%% Theorem ~\ref{thm:otherchoicesoftau} shows that the lower bound on
%% the bias from Theorem ~\ref{thm:main_text} cannot be overcome in any
%% of the three studied cases.




% RBF$^{***}$: Our results also cover general RBF functions when $d \asymp \tr(\Sigma_d) \asymp n$ (see Appendix \ref{sec:AC})
































% In our work, we show that the polynomial approximation barrier is not
% specific to \emph{uniform} distributions on the sphere or two
% hyperspheres, but rather a very general phenomenon. In particular, 
% %compared to \cite{Ghorbani19,Ghorbani20} \fy{again and again?}
% we extend the settings for which the statements
% in Theorem~\ref{thm:main_thm} holds, in three significant ways:
% %We explicitly prove that it holds for
% \begin{enumerate}
% \item We allow general linear covariance model distributions described in Assumption \Bdone and the resulting distributions when projected on the sphere (see Table~\ref{tab:settings})
%   \item We cover rotationally invariant kernels with vastly different eigenvalue decay rates, related to spikiness. 
%   \item We are the first to include the cases when the scale parameter $\bw$ decreases or increases faster than $\effdim$.
% \end{enumerate}
% 
% 



%  In the "ridge-less" case, where $\lambda = 0$ and $\tilde{\bw} \overset{n\to \infty}{\to} 0$ the analysis turns out to be significantly more challenging. Here, we only study the extreme case where we analyse the flat limit, i.e. the solution obtained when for any fixed $n,d$ taking the limit of $\tilde{\bw} \to 0$,
% \begin{equation}
%     \forall n,d: ~~ \fhat_{\textrm{PS}}(\datamatrixtar) := \lim_{\tilde{\bw} \to 0} \fhat(\datamatrixtar) = \lim_{\tilde{\bw} \to 0} \y^\top  \kermat^{-1} \kstar.
% \end{equation}
% In general, it is not clear whether this solution exists. However, we can apply \cite[Theorem~3.12]{Lee2014} and \cite[Theorem~2.1]{Blumenthal60} to show that for any $\alpha \in (0,2)$, $\hat{f}_{\textrm{PS}}$ exists and exactly the \textit{Polyharmonic Spline Interpolator} introduced by \citet{Wahba90} with the closed form expression:
% \begin{equation}
%     \fhat_{\textrm{PS}}(\datamatrixtar) = \begin{pmatrix}y \\ 0 \end{pmatrix}^\top \begin{pmatrix} -D^{\alpha} & 1 \\ 1^\top & 0 \end{pmatrix}^{-1} \begin{pmatrix} d^{\alpha,*} \\ 1 \end{pmatrix}.
% \end{equation}
% % Here $D^{\alpha}$ is $n\times n$ matrix with entries $D^{\alpha}_{i,j} = \| \zind{i}-\zind{j} \|_2^{\alpha}$ and $d^{\alpha,*}$ is the vector with entries $d^{\alpha,*}_i = \| \zind{i} - \z^* \|_2^{\alpha}$ and with $\zind{i} = \bw\xind{i}$ and $\z^* = \bw \x^*$. We can now state the main theorem of this section. 



%% In particular, our results are independent of the
%% explicit structure of the covariance matrix $\inputcov$ but solely
%% depend on $\effdim = \tr(\inputcov)$.
% This point might be rather confusing : 
% One consequence of the unified treatment is that we conclude that
% functions with bounded RKHS norm can indeed only be lower degree
% polynomials almost everywhere (see formal discussion in~\suppmat
% \fy{could point to a formal corollary in appendix?}).
%% , an important object well-studied in the
%% literature.


%Our results hence 
% 
% \subsection{The role of regularization in high dimensional regression}
% %% discuss their consequences in the context of the modern
% %% storyline of learning with overparameterized models and 
% %% for the use of kernel methods in practice.
% 
% We now want to highlight some consequences of the polynomial approximation
% barrier in light of a dominating narrative in modern machine learning.
% %% for overparameterized
% %% models in modern learning theory. Even though these
% 
% %% Even though these also hold for \cite{Ghorbani19,Ghorbani20},
% %% we have shown them to hold in broader distributional settings.
% 
% In particular, many recent works have studied minimum norm
% interpolators in the high-dimensional regime and e.g. show for linear
% regression that asymptotically, their risk follows a double descent
% curve as overparameterization ratio $\frac{d}{n}$ increases (see
% ~\cite{Hastie19,Bartlett20}.  The main reason is that the variance has
% a peak at $d = n $ and decreases after that $\frac{d}{n}$
% \cite{Yang20}.  As a consequence, the community argues that in high
% dimensions, regularization is not necessary.
% 
% %% Similarly, the upper bound on the variance has been shown to decrease
% %% with dimension for high-dimensional kernel
% %% regression in \cite{Liang20a, Liang20b,Ghorbani19,Ghorbani20}.
% %% \fy{but not as a function of $\beta$ or ratio...}
% %% %% as reported for neural networks
% %% %% in practice \fy{ref}.
% %% Together with the polynomial approximation barrier
% %% with the bias dominating the variance \fy{we kinda need rates for that}
% 
% %% suggests a different role
% %% of increasing the dimensionality for kernel regression.
% %% %% as opposed to in
% %% %% linear regression,
% %% More specifically, increasing dimension does not only simply reduce
% 
% %% Therefore, as dimension
% %% increases, the bias term dominates rather quickly and hence the risk
% %% follows the usual bias variance curve instead of a double descent
% %% curve \cite{Yang20,DAscoli19}. We make these observations also
% %% empirically in Figure \ref{fig:realworld} for synthetic and real world
% %% data sets which underlines our conclusions.
% 
% 
% While the story is clean for linear regression, we would like to
% paint a more nuanced picture for kernel regression in high dimensions.
% %% Ridge or ridgeless kernel learning?: Furthermore, as opposed
% %% to the usual narrative, we conjecture
% %% regularization is not obsolete in kernel learning. The argument goes
% %% as follows: 
% First of all, when the ground truth function is not a low-degree polynomial
% %function as a function of entries of $x$,
% our Theorem~\ref{thm:main_thm} implies that we simply cannot learn it
% with a rotation-symmetric kernel with and without ridge regularization
% irrespective of the variance. In the case when it inherently only
% depends on a few variables however, we could in principle achieve consistency
% by first selecting the relevant features and then performing
% kernel ridge regression on the lower dimensional problem. But do we
% really need to 
% For low dimensions at least, ridge regularization can indeed be necessary,
% as \cite{Rakhlin18} show for the Laplacian kernel and
% observations with Rademacher noise that the minimum norm
% interpolant is inconsistent.
% %% as
% %% follows: first select the relevant features and then compute the kernel
% %% ridregression in the reduced dimensions. For the Laplacian kernel and
% %% observations with Rademacher noise we can then invoke \cite{Rakhlin18}
% %% who show that the ridgeless regression is not consistent.
% On the other hand, we know that ridge regression is sufficient to
% obtain a consistent estimator for any universal kernel (see
% Theorem~12 in~\cite{Christmann07}). In summary, we argue that even in high
% dimensions, regularization is not necessarily obsolete when using
% kernel regression.  We confirm this conjecture for some real-world
% data sets in Section~\ref{sec:expreal}.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%% \kd{This paragraph needs to be completely rewritten} While there
%% exists multiple paper on kernel ridge and especially "ridge-less"
%% regression claiming that consistency can be reached for rotationally
%% symmetric kernels in high dimensional regimes
%% \cite{Liang20a,Liang20b,Liu20,Ghorbani19,Ghorbani20}, we highlight
%% that the current literature is unclear about the set of ground truth
%% functions for which this is true. On the one hand,
%% \citet{Ghorbani19,Ghorbani20} showed that we can at most approximate
%% polynomials of a certain degree when assuming that the input data sets
%% are drawn from the uniform distribution on the hyper sphere,
%% respectively on the product of two hyper spheres of different
%% radii. In contrast, on the other hand, in the papers
%% \cite{Liang20a,Liang20b,Liu20} linear covariance data models are
%% studied, where less restrictive assumptions on the ground truth
%% function are imposed. In particular, these results do not limit the
%% ground truth function to polynomials. In the last section, we have
%% already questioned the applicability of the bias bound from
%% \cite[Theorem~3]{Liang20a}. Still, it is yet unclear how the
%% discrepancy in the results for the linear covariance data models
%% \cite{Liang20b,Liu20} with the ones for spherical input data
%% \cite{Ghorbani19,Ghorbani20} can be reached can be explained.
% 
% \begin{theorem}[No consistency beyond polynomials]
%   \label{thm:main_thm}
%   Assume that the kernel $\kernf$, respectively its restriction onto the hyper sphere $\kernfuncressphere{d}$, is the $\alpha$-exponential kernel with $\alpha\in (0,2)$ or satisfies the assumptions A.1 - A.3, where we additionally assume that $g_i(1,1) \geq 0$ and $g_i$  is
%   $(\floor{2/\beta}+1-i)$-times continuously differentiable in an
%   neighbourhood of $(1,1)$. In addition, we assume that there exists $\jthresh > \floor{2/\beta}$ such that $\rotkerfunc_{\jthresh}(1,1) >0$.
%   
%   
%   %% \kd{We can now remove this:
%   %% and the eigenvalues of $\kermat$ are lower bounded by a positive
%   %% constant for all $n$.}
%   Furthermore assume that the ground truth that
%   is bounded $|\ftrue| \leq \ubfunc$ almost surely for some $\ubfunc >
%   0$.  Then the following results hold for $m = 2 \floor{2/\beta}$ in
%   the case of the marginal distribution $\prob_X \in \probsetcov$ and $m =
%   \floor{2/\beta}$ in the case of $\prob_X \in \probsetsphere$:
%   
%   \begin{enumerate}
%   
%   \item As $n \to \infty$, for any $\eps$ there exists a polynomial $\polyf \in \polyspace{m}$ so that 
%   with probability $\geq 1- \exp(-\Cgenprob{\epsd}
%   \log(n)^{((1+\epsilon)/2ilon)/2d})$ over the draws of a test sample $\Xrv$, 
%   \begin{equation}
%     \label{eq:polyapprox}
%     \left| \EEobs \fhatridge(\Xrv) - \polyf(\Xrv) \right| \leq \epsilon
%     ~~ a.s.,
%   \end{equation}
%     where $\EEobs \fhatridge(\Xrv)$ is the estimator with expectation
%   taken over the observation noise.  Furthermore, assume that the kernel function $\kernf$ is bounded
%   on the support of $\prob_X$, then we can find $\polyf$ such that
%   \begin{equation}
%     \left\| \EEobs \fhatridge - \polyf \right\|_{\Ell_2(\prob_X)} \leq \epsilon
%     ~~ a.s..
%   \end{equation}
% 
% 
%   \item The
%   bias of the kernel ridge and ridgeless estimators $\fhatridge$ is
%   asymptotically lower bounded for any $\gamma > 0$ as $n\to \infty$,
%   \begin{equation}
%     \label{eq:biaslb}
%     \Bias(\fhatridge) \geq \underset{\polyf \in
%       \polyspace{m}}{\inf} \EE_{X} \left( \ftrue(\Xrv) -
%     \polyf(\Xrv)\right)^2 - \gamma ~~~a.s..
%   \end{equation}
%   \end{enumerate}
%   %% More precisely,
%   %% \begin{enumerate}
%   %%   \item when $X$ is drawn from a distribution that satisfies
%   %%     Assumptions A.1-A.2, the bias lower bound~\eqref{eq:biaslb} and
%   %%     polynomial approximation~\eqref{eq:polyapprox} hold with $m = 2
%   %%     \floor{2/\beta}$.
%   %%   \item When $X = \frac{Z}{\|Z\|}$ with $Z$ drawn from a
%   %%     distribution that satisfies Assumptions A.1-A.2, the bias lower
%   %%     bound~\eqref{eq:biaslb} and polynomial
%   %%     approximation~\eqref{eq:polyapprox} holds
%   %%     %%  for all kernel functions
%   %%     %% restricted to the sphere $\kressphere(\xk,\xkd) = \rotkerfunc(\xk^\top \xkd)$ with $\rotkerfunc$ locally analytic around $0$ and 
%   %%     with $m = \floor{2/\beta}$.
%   %%   %% \item Assume that the eigenvalues of $\kermat$ are lower bounded.
%   %%   %%   Then above results also hold for the minimum norm interpolator
%   %%   %%   $\fhatinterpol$ in~\eqref{eq:constraint_min_p}
%   %% \end{enumerate}
% 
%   %%   The results hold trivially for $\lambda \geq c > 0$ and for decaying
%   %% $\lambda \to 0$ and $\lambda = 0$ (the minimum norm interpolator
%   %%   $\fhatinterpol$ in~\eqref{eq:constraint_min_p}) if the
%   %%   eigenvalues of $\kermat$ are lower bounded by a positive constant for all $n$.   
% \end{theorem}

%% Hence, we can show that:
%\kd{We can merge it with the main theorem, but i find this quite elegant.}
%% \begin{prop}
%% The results form Theorem \ref{thm:main_thm} also apply for the $\alpha$-Exponential kernel when $\alpha <2$.
%% \end{prop}

%% For 
%% The bias of any ... is approximated by 
%% by the approximation error of $\ftrue$
%%   by a polynomial of degree $m$ truncated at $\ubpoly \geq
%%   \ubfunc$. That is, if the function does not lie in $\polyspacetrunc{m}{C}$, for some $\ubpoly \leq \ubfunc$.


%% Assume that the Assumption A.1-A.3 hold true and the assumption
%% B.1-B.2 for the kernel $k$, respectively the Assumption
%% $\tilde{\textrm{B}}$.1 for the kernel $\kerns$.  Furthermore, assume
%% that the minimum Eigenvalues of $(\lambda \textrm{I}_n + \kermat)$,
%% respectively $(\lambda \textrm{I}_n + \Ks)$ are almost surely lower
%% bounded by a non zero positive constant. Let $m =\floor{2/\beta}$. We
%% have that:
%% \begin{enumerate}
%% \item
%% For any $\epsilon>0$ and any $n$ sufficiently large, there exists a polynomial $p \in \mathcal{P}_{\leq 2m}$, such that  with probability $\geq 1- \exp(-C \log(n)^{((1+\epsilon)/2ilon)/2d})$ over the draws of  $X$,
%% \begin{equation}
%% \label{eq:degenratedf}
%%     \left| f^*(\datamatrix)^\top (K + \lambda \textrm{I}_n)^{-1} \kstar(\Xrv) - p(\Xrv) \right| \leq \epsilon ~~ a.s.,
%% \end{equation}
%% and similarly there exists a polynomial $p_{\mathcal{S}} \in \mathcal{P}_{\leq m, \mathcal{S}}$ such that with probability $\geq 1- \exp(-C \log(n)^{((1+\epsilon)/2ilon)/2d})$ over the draws of  $S$,
%% \begin{equation}
%% \label{eq:degenratedf}
%%     \left| f^*(\Ss)^\top (\Ks + \lambda \textrm{I}_n)^{-1} \kstars(\Srv) - p_{\mathcal{S}}(\Srv) \right| \leq \epsilon ~~ a.s.,
%% \end{equation}
%% with $\epsd>0, C>0$ some positive constants.
%% \item
%% For any $C\geq C_{f^*}$, any $\gamma >0$ and any $n$, the bias can be lower bounded by 
%% \begin{equation}
%%     \textbf{B}(\hat{f}_{\lambda})  \geq  \underset{\overline{p} \in \overline{\mathcal{P}}_{\leq 2 m,C}}{\inf} \mathbb{E}_{X} \left| f^*(X) - \overline{p}(X)\right|^2  - \gamma ~~~a.s,
%% \end{equation}
%% and similarly, 
%% \begin{equation}
%%         \textbf{B}(\hat{f}_{\lambda,\mathcal{S}})  \geq  \underset{\overline{p_{\mathcal{S}}} \in \overline{\mathcal{P}}_{\leq m,C, \mathcal{S}}}{\inf} \mathbb{E}_{\Srv} \left| \ftrue(\Srv) - \overline{p}_{\mathcal{S}}(\Srv)\right|^2  - \gamma ~~~a.s.
%% \end{equation}
%% \end{enumerate}
%% \end{theorem}



%% \paragraph{Proof sketch}
%%  For the brevity of the notation, we call $\zind{i} = \sqrt{\bw}\xind{i}$ and $\Zrv = \sqrt{\bw} \Xrv$ where $\Xrv$ is a random variable independently drawn form the same distribution as $\xind{i}$. Essentially, any of the presented results are a consequence the strong concentration of Lipschitz continuous functions of vectors of i.i.d random variables \cite[Corollary~4.10]{Ledoux2001}. As a consequence, we will show in Corollary \ref{cr:testsample} that for any $\eps >0$, with high probability over the draws of $\Zrv$,
%% \begin{equation}
%% \label{eq:oultineproof}
%%     \underset{i}{\max}\left| \zind{i}^\top \Zrv \right| \leq n^{-\beta/2}(\log n)^{(((1+\epsilon)/2ilon)/2ilon)/2}
%% \end{equation}
%% Here, we only provide the main intuition for the proof of Theorem \ref{thm:main_text} for the case where the kernel function $k$ is an inner product kernel. This is offers the simplest way to gain an intuition for the phenomenon causing the bias to be bounded. As a consequence of the concentraiton inequality from Equation \ref{eq:oultineproof}, we can show that we can discard the higher order term of the local power series expansion:
%% \begin{equation}
%%     \kernf(\zind{i},\Zrv) = \sum_{j=0}^{m} g_j ~ (\zind{i}^\top\Zrv)^j + O\left(n^{-(m+1)\beta/2} (\log n)^{(m+1)((((1+\epsilon)/2ilon)/2ilon)/2} \right) ~~a.s..
%% \end{equation}
%% Since we choose $m = \floor{\beta/2}$, we can see that $n \left(n^{-(m+1)\beta/2} (\log n)^{(m+1)((((1+\epsilon)/2ilon)/2ilon)/2}\right) \to 0$. As a result, the kernel function $k$ looks like a polynomial of degree at most $m$ plus an error term which vanishes at rate $o(n^{-1})$ with high probability over the draws of $\Zrv$ and almost surely over the draws of $\Z = \{\z_1,...,\z_n\}$ .

%% \fy{need to write a line on represneter theorem}
%% The proof hinges on the closed-form expression of the ridge(less)
%% estimate.  For some $x\in \X$, let $\kerx{x} \in \R^n$ be the
%% vector with entries $\kerx{x} = k_{\bw}(\xi{i}, x)$. For any $\lambda
%% >0$ we can write obtain
%% \begin{equation}
%% \label{eq:kernelridge}
%%     \fhatridge(x) = \y^\top (\kermat + \lambda \idmat_n)^{-1}\kerx{x}.
%% \end{equation}
%% As a next step, we show that
%% \begin{equation}
%% \label{eq:sec4outlinproof}
%%    \EE_Y \fhatridge(X) = \ftrue(\Xrv)^\top (\kermat + \lambda \In)^{-1}\kerx{\Xrv} = \sum_{i=0}^n \sum_{j=0}^{m} g_j ~ (\zind{i}^\top\Zrv)^j + o(1)~~a.s.,
%% \end{equation}
%% holds true with high probability over the draws of $\Xrv$. Here, we use the assumption that the Eigenvalues of $\kermat+ \lambda \In$ are lower bounded. The rest of the proof is then just a straight forward application of this fact. \qed

%% For decreasing risk estimates and the minimum norm interpolator
%% Theorem~\ref{thm:main_thm} requires that the $\kermat+ \lambda \In$ is
%% asymptotically lower bounded by a positive constant. The following
%% proposition characterizes for which kernels this condition is satisfied.
%% which is due to the well known Representer Theorem, \fy{schoelkopf
%%   didn't invent representer theorem, too standard to cite}
%% For interpolation, 
%% we assume
%% that the kernel matrix $K$ is almost surely invertible with respect to
%% the draws over the data sets $\datamatrix$. We remark that this assumption is
%% guaranteed to be the case for any universal kernels such as the
%% Gaussian or Laplacian RBF kernels.

%% Clearly, whenever $\lambda$ does not go to zero but
%% instead is lower bounded by some positive constant, the Eigenvalues of
%% $ \lambda \In + K$ are also lower bounded and therefore Theorem
%% \ref{thm:main_text} applies for any of the kernels satisfying the
%% Assumptions B.1 and
%% $\tilde{\textrm{B}}$.4-$\tilde{\textrm{B}}$.5. \fy{see it would be better to be able to reference so that you don't have undefined references} Unfortunately, this is
%% not guaranteed for the minimum norm interpolant when the ridge parameter $\lambda\to 0$.  Showing that this holds true for different kernels is the main
%% technical challenge of this paper. In fact, we can show that:
%% \fy{mention that we need at least universality}
%% \kd{No, we just need that the kernel matrix $\kermat$ is almost surely invertible}



%% We want to highlight that compared to \cite{Liang20a, Liang20b}, we
%% need the minimum eigenvalues of the kernel matrix to be lower bounded
%% by a constant (similar as in \cite{Ghorbani19, Ghorbani20})
%% as we do not restrict ourselves to norm bounded functions.
%% The proof of the lower bounded eigenvalue functions is
%% in fact the more involved part of our analysis and requires
%% separate treatment for different types of kernels. 
%% The following proposition shows that the eigenvalues holds
%% indeed for most kernels that have so far been analyzed
%% in the literature.

%% %%%%%%%%%%%%%%%%%%%%5%%%%%%%%%%%%%%%%%%%%%%%%%
%% %%%%%%% Proposition lower bounded EV %%%%%%%%%%%
%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% \begin{prop}[Lower bounded kernel eigenvalues]
%%   \label{prop:kernelslowerboundev}

%%   For $\prob_X \in \probsetcov, \probsetsphere$, the eigenvalues of
%%   the kernel matrix $\kermat$ can be almost surely lower bounded by a
%%   positive constant $c>0$ for the following
%%   kernel functions
%%   \begin{enumerate}
%%   \item Any inner product kernel with Taylor expansion
%%     $\kerfunc{\xk}{\xkd} = \rotkerfunc(\xk^\top \xkd) =
%%     \sum_{j=0}^{\infty} \rotkerfunccoeff ~(\xk^\top \xkd)^j$ with
%%     $\rotkerfunccoeff \geq 0$ and $\jthresh > \floor{2/\beta}$ such
%%     that $\rotkerfunccoeffj{\jthresh} > 0$.
%%   \item The $\alpha$-exponential kernel $k(\xk,\xkd) =
%%     \exp(-\| \xk- \xkd \|_2^{\alpha})$ with
%%     $\alpha \in (0,2)$.
%%   \item Any neural tangent with a homogeneous activation function and Hermit polynomial extension with coefficients $\hermitcoeff \in \RR$ and $\jthresh > \floor{2/\beta}$ such that $\hermitcoeffj{\jthresh}$. In particular, this holds true for the Relu activation function $\actfun{\xk} = \max(0,\xk)$. \kd{This is a bit long - but i do not want to introduce homogenity and Hermit poly extension here}
%%   \end{enumerate}
%%   %% In addition, when $\prob_X \in \probsetsphere$, the eigenvalues are lower
%%   %% bounded for any rotation invariant kernel
%%   %% for which the series expansion $\kerfunc{\xk}{\xkd} =
%%   %% \sum_{j=0}^{\infty} \rotkerfunccoeff ~(\xk^\top \xkd)^j$ as in
%%   %% Equation~\eqref{eq:Scheonbergseries} only has non-negative
%%   %% coefficients $\rotkerfunccoeff \geq 0$, and there exists $\jthresh >
%%   %% \floor{2/\beta}$ such that $\rotkerfunccoeffj{\jthresh} > 0$.
%%   %% \fy{i think we have to adjust that after this sum switching adjustment?}
%% %% \end{enumerate}
%% \end{prop}


%% In fact, we can show a much more general result for the case where the
%% input data is $\datamatrix$ than the one presented in Proposition
%% \ref{prop:kernelslowerboundev}. However, we remark that it is not
%% trivial to verify that these assumptions hold true for arbitrary
%% kernels. We refer to Proposition \ref{prop:Evlowerbound} in the
%% Appendix for the statement and a discussion on the applicability of
%% this proposition.


% \fy{Discussion on kernels and short comparison with previous}

%% While Theorem ~\ref{thm:main_thm} applies to a very broad range of rotationally invariant kernel functions, it is not clear for which RBF kernel functions this is the cae besides the Gaussian kernel. We address this issue in Section \ref{sec:RBFK} from the Appendix, where we show that thee Assumption A.1-A.2 can be weakend when assuming that the Eigenvalues of the kernel matrix $\kermat$ are almost surely lower bounded by a non zero positive constant. We refer to Corollary \ref{cr:RBFmain_thm} for the precise statement. In fact, we can show that this is the case for the  $\alpha$-Exponential kernels with  $\alpha \leq 2$.

% 
% \fy{add sth on the $\beta$-dependent assumption: lower bounded EV and
%   for all kernels we and others consider, this holds for all
%   $\beta>0$} \fy{something about assumptions on sphere are easier and
%   Schoenberg as below} When the input data lives on the hyper sphere
% $\Sphere{d}$, as in \cite{Ghorbani19,Ghorbani20}, the required
% assumptions on $\rotkerfunc$ become weaker. For example, A.2 trivially
% holds true given A.1 as $\|x\|=1$. Furthermore, we know from
% \citet{Schoenberg1988} that any continuous rotational symmetric
% function on the hyper sphere can be written as an inner product
% kernel, i.e. $\kernfuncressphere{d}(\xk,\xkd) = \rotkerfunc(\xk^\top
% \xkd)$, which we know from the previous discussion satisfies
% assumption A.1-A.3 under weak assumptions.
% 
% \fy{something along those lines} We note that our lower bound is not
% tight, as it has an additional factor of 2 compared to
% \cite{Ghorbani20}. We conjecture that that the tight bound should hold
% for $m=\floor{1/\beta}$. However since the focus of this work was to
% illustrate the barrier for different settings, tightening the bound
% will be left to future work
%   



%% Surprisingly, we find that bound from Theorem ~\ref{thm:main_text}
%% depends only on the growth rate of the trace $\trace(\inputcov)$ with
%% respect to $n$, but not on the explicit structure of the covariance
%% matrix $\inputcov$. Hence, given that $\beta$ is some constant, we find
%% that the Bias $\textbf{B}(\hat{f}_{\lambda})$ never vanishes if the
%% ground truth is sufficiently non linear. In fact, our results do not
%% depend on the sparsity of the ground truth function, meaning that the
%% issue also holds true for arbitrarily sparse ground truth
%% functions. As a consequence, we prove the intuitions gained from
%% \cite{Ghorbani19} who shows a stronger version of Theorem
%% \ref{thm:main_text} for the uniform distribution on the hyper sphere.
%% As a result, we can see that we can never reach consistency if the
%% projection error of the ground truth function onto the space of
%% truncated polynomials is not vanishing, respectively zero. Finally, we
%% mention \cite[Theorem~4]{Bartlett20}, where it was shown that for the
%% linear regression the explicit structure of the data covraiance matrix
%% plays an important role to determine whether consistency can be
%% reached. While this result leads to the question whether the explicit
%% structure of the covariance matrix also determine consistency for
%% kernel regression, our analysis clearly shows that this is not true
%% for general non linear functions. \newline Interestingly, our proof
%% does not just only imply that the bias does not vanish, but also that
%% the noiseless estimator looks asymptotically almost everywhere like a
%% polynomial. This clearly demonstrates that both kernel ridge and
%% "ridge-less" regression have an implicit bias towards simple models in
%% high dimensions, which is also responsible for the non vanishing bias
%% if the ground truth function is sufficiently non polynomial. Finally,
%% we remark that Proposition \ref{prop:poly} can also applies for the
%% estimator $\hat{f}_{\lambda}$ even when noise is present under the
%% assumption that the observation noise is bounded. \newline We will now
%% discuss the implications for the three explicit examples of kernels
%% mentioned in Proposition \ref{prop:kernelslowerboundev}.

%% \textbf{Inner Product Kernels:} 
%% \kd{ Need to rewrite:}
%% The inner product kernels are widely used in the literature \cite{Liang20b,Liu20,Liang20a,Ghorbani19,Ghorbani20,ElKaroui10} which allows a good comparison with the existing results. In particular, \citet{Liang20b} claims that the risk vanishes in regimes where $d \asymp n^{\beta}$ with $\beta \in (0,1)$ and $\inputcov = \textrm{I}_d$. While it is not exactly clear which ground functions satisfy the assumption in the paper \cite{Liang20b}, as a consequence of our results, we can clearly show that this is not true given that the ground truth function $f^*$ is not a polynomial of degree at most $\floor{2/\beta}$.

%% \textbf{The role of eigenvalue decay} The second example of kernels
%% for which we can show that Theorem ~\ref{thm:main_text} applies are the
%% $\alpha$-Exponential RBF kernels of the form $k(\xk,\xkd) =
%% \exp(-\| \xk - \xkd \|_2^{\alpha})$ with special
%% cases including the Laplace kernel ($\alpha =1$) and the Gaussian
%% kernel ($\alpha = 2$). These kernels have shown strong performance on
%% multiple high dimensional data sets as shown in the papers
%% \cite{Geifman20,Belkin18a}. In addition, we can see from
%% \cite[Theorem~2.1]{Blumenthal60} that these kernels cover a broad
%% spectrum of different Eigenvalue decays, including both exponential
%% decay, i.e. when $\alpha =2$, and a broad range of polynomial decays,
%% i.e. when $\alpha <2$. As a consequence, we can conclude that the
%% phenomenon described in Theorem ~\ref{thm:main_text} and Corollary
%% ~\ref{prop:poly} appears to be independent of the Eigenvalue decay of
%% the kernels. Furthermore, our results indicate that the strong
%% performance observed in \cite{Geifman20}

%% \textbf{Neural Tangent Kernels:} 

%% \kd{Thanks to Parnians hint, our statements hold for many more activation functions than just Relu :)}

%% As a last example, we discuss the Neural Tangent Kernels (NTK) with
%% activation function. Interestingly, from the above discussion, we know
%% that the NTK of any depth satisfies the assumptions in Corollary
%% ~\ref{prop:Evlowerbound} and thus also in Theorem
%% ~\ref{thm:main_text}. These results extend the observations for NTK's
%% on the Hyper sphere by \citet{Ghorbani19,Ghorbani20}. Furthermore, we
%% remark that the benefits of the depth for NTK kernels has also been
%% questioned in the paper \cite{Bietti20}. However, our results are
%% orthogonal to the results of \citet{Bietti20}, because their main
%% argument is that the NTK of any depth has the same Eigenvalue
%% decay. Since our results do not depend on the Eigenvalue decay, we
%% highlight that our observation that the depth does not help to
%% overcome the bias bound from Theorem ~\ref{thm:main_text} is not a
%% consequence of the results form the paper \cite{Bietti20}.
 



%% Surprisingly, we find that bound from Theorem ~\ref{thm:main_text}
%% depends only on the growth rate of the trace $\trace(\inputcov)$ with
%% respect to $n$, but not on the explicit structure of the covariance
%% matrix $\inputcov$. Hence, given that $\beta$ is some constant, we find
%% that the Bias $\textbf{B}(\hat{f}_{\lambda})$ never vanishes if the
%% ground truth is sufficiently non linear. In fact, our results do not
%% depend on the sparsity of the ground truth function, meaning that the
%% issue also holds true for arbitrarily sparse ground truth
%% functions. As a consequence, we prove the intuitions gained from
%% \cite{Ghorbani19} who shows a stronger version of Theorem
%% \ref{thm:main_text} for the uniform distribution on the hyper sphere.
%% As a result, we can see that we can never reach consistency if the
%% projection error of the ground truth function onto the space of
%% truncated polynomials is not vanishing, respectively zero. Finally, we
%% mention \cite[Theorem~4]{Bartlett20}, where it was shown that for the
%% linear regression the explicit structure of the data covraiance matrix
%% plays an important role to determine whether consistency can be
%% reached. While this result leads to the question whether the explicit
%% structure of the covariance matrix also determine consistency for
%% kernel regression, our analysis clearly shows that this is not true
%% for general non linear functions. \newline Interestingly, our proof
%% does not just only imply that the bias does not vanish, but also that
%% the noiseless estimator looks asymptotically almost everywhere like a
%% polynomial. This clearly demonstrates that both kernel ridge and
%% "ridge-less" regression have an implicit bias towards simple models in
%% high dimensions, which is also responsible for the non vanishing bias
%% if the ground truth function is sufficiently non polynomial. Finally,
%% we remark that Proposition \ref{prop:poly} can also applies for the
%% estimator $\hat{f}_{\lambda}$ even when noise is present under the
%% assumption that the observation noise is bounded. \newline We will now
%% discuss the implications for the three explicit examples of kernels
%% mentioned in Proposition \ref{prop:kernelslowerboundev}.

%% \textbf{Inner Product Kernels:} 
%% \kd{ Need to rewrite:}
%% The inner product kernels are widely used in the literature \cite{Liang20b,Liu20,Liang20a,Ghorbani19,Ghorbani20,ElKaroui10} which allows a good comparison with the existing results. In particular, \citet{Liang20b} claims that the risk vanishes in regimes where $d \asymp n^{\beta}$ with $\beta \in (0,1)$ and $\inputcov = \textrm{I}_d$. While it is not exactly clear which ground functions satisfy the assumption in the paper \cite{Liang20b}, as a consequence of our results, we can clearly show that this is not true given that the ground truth function $f^*$ is not a polynomial of degree at most $\floor{2/\beta}$.

%% \textbf{The role of eigenvalue decay} The second example of kernels
%% for which we can show that Theorem ~\ref{thm:main_text} applies are the
%% $\alpha$-Exponential RBF kernels of the form $k(\xk,\xkd) =
%% \exp(-\| \xk - \xkd \|_2^{\alpha})$ with special
%% cases including the Laplace kernel ($\alpha =1$) and the Gaussian
%% kernel ($\alpha = 2$). These kernels have shown strong performance on
%% multiple high dimensional data sets as shown in the papers
%% \cite{Geifman20,Belkin18a}. In addition, we can see from
%% \cite[Theorem~2.1]{Blumenthal60} that these kernels cover a broad
%% spectrum of different Eigenvalue decays, including both exponential
%% decay, i.e. when $\alpha =2$, and a broad range of polynomial decays,
%% i.e. when $\alpha <2$. As a consequence, we can conclude that the
%% phenomenon described in Theorem ~\ref{thm:main_text} and Corollary
%% ~\ref{prop:poly} appears to be independent of the Eigenvalue decay of
%% the kernels. Furthermore, our results indicate that the strong
%% performance observed in \cite{Geifman20}

%% \textbf{Neural Tangent Kernels:} 

%% \kd{Thanks to Parnians hint, our statements hold for many more activation functions than just Relu :)}

%% As a last example, we discuss the Neural Tangent Kernels (NTK) with
%% activation function. Interestingly, from the above discussion, we know
%% that the NTK of any depth satisfies the assumptions in Corollary
%% ~\ref{prop:Evlowerbound} and thus also in Theorem
%% ~\ref{thm:main_text}. These results extend the observations for NTK's
%% on the Hyper sphere by \citet{Ghorbani19,Ghorbani20}. Furthermore, we
%% remark that the benefits of the depth for NTK kernels has also been
%% questioned in the paper \cite{Bietti20}. However, our results are
%% orthogonal to the results of \citet{Bietti20}, because their main
%% argument is that the NTK of any depth has the same Eigenvalue
%% decay. Since our results do not depend on the Eigenvalue decay, we
%% highlight that our observation that the depth does not help to
%% overcome the bias bound from Theorem ~\ref{thm:main_text} is not a
%% consequence of the results form the paper \cite{Bietti20}.






%% Even though I'd mention it in talks, maybe can indeed skip the NTK point
%% As mentioned in \cite{Ghorbani20} \fy{Maybe sth on NTK, e.g.
%% rotation symmetric NTK be good enough to explain NN in high-d.}



%% \subsection{Discussion of results}
%% \fy{I don't have time to spell it out, but what we want to write}

%% \paragraph{Our extensions}
%% \begin{itemize}
%% \item We show that kernel regression is consistent for ridge regression and min-norm interpolants unless they're polynomials for a broader range of distributions, for similar scaling and beyond that \fy{could maybe put after $\tau$ to make the contrast starker}
%% \item Sasha 2 + ours: Functions with bounded norm have to low degree polynomials in the high probability region around the sphere
%% \end{itemize}

%% These points have been made by Ghorbani but we show for more general
%% \begin{itemize}
%%     \item has ``implicit bias'' towards polynomials (not so sure how much this point adds)
%%   \item  NTK on fully connected networks can only learn polynomials, independent of depth - maybe not the right object to analyze. The fact that the properties of the NTK are independent of depth have also been noted in another context by Bietti and Bach in terms of the normalized eigenvalue decay.
%% \end{itemize}

%% These are in the essence not much different than Ghorbani, but
%% obviously other distribution, plus we make the point explicitly
%% \begin{itemize}
%%   \item \item Re Tsybakov/Wyner/Belkin et al: Spiky kernels, aka have been shown to better behavior than ... for interpolation. We want to note the inconsistency result is in fact independent of the spikiness or eigenvalue decay, in particular it holds for $\alpha$-exponential kernels
%%   \item for sparse functions there's hope, tradeoff in the bias (see exps) independent of noise
%% \end{itemize}



%% In this section, we discuss the relevance of regularisation in a
%% broader perspective and incorporate our results with the literature on
%% classical low dimensional settings. Our discussion concentrates again
%% on the setting described by the Assumptions A.1 and A.3, however, we
%% do not necessarily require that the regime is high dimensional,
%% i.e. Assumption A.2. Furthermore, in order to be able to apply the
%% classical results guaranteeing consistency, we require that the
%% support of $X$ is compact.

%% We call a kernel on a compact space $\XX$ \textit{universal} if its
%% corresponding RKHS is dense in the set of continuous functions
%% $C(\XX)$ with respect to the infi/nity norm
%% \cite[Definition~11]{Christmann07}. This definition applys to a braod
%% range of popular kernel functions including the Laplace kernel as
%% shown in \cite[Example~1]{Sriperumbudur11}. We can now summarise the
%% positive results on consistency of kernel ridge regression from
%% \cite[Thoerem~12]{Christmann07} and the negative results for the
%% special case of the Lapalace kernel by \citet{Rakhlin18} in the
%% following corollary:



%% Assume that the data is distributed according to Assumptions A.1 and
%% A.3. In addition, assume that the support of $X$ is compact and the
%% dimension $d$ is constant. Then, under a suitable choice of the ridge
%% parameter, kernel ridge regression for any universal kernel is
%% consistent. In particular, this holds true for the Laplace kernel.

%% In contrast, assume that the observations are generated by adding
%% $i.i.d$ Rademacher noise $\xi_i$ to the ground truth function,
%% i.e. $\y_i = \ftrue(\xi{i}) + \xi_i$ with $P(\xi_i = 1) = P(\xi_i =
%% -1) = 1/2$. Then, the kernel "rigde-less" regression for the Laplace
%% kernel is never consistent.

%% As a result of this corollary, we can see that regularisation is
%% explicitly required for the Laplace kernel to be consistent in fixed
%% dimensions $d$. Furthermore, as a result of our research, we can
%% conlcude:

%% As a result, we can conclude that the bias does never vanish when
%% $\ftrue$ is a highly non linear function. For instance, choosing
%% $\ftrue(\x) = \sin(\x_{(1)})$ would satisfy our assumptions and hence
%% can never be consistently learned in the described high dimensional
%% regimes. As a consequence of Corollary \ref{cr:lowdimcons} and
%% Corollary \ref{cr:highdimcons}, we can conclude that sufficiently non
%% polynomial functions in the sense that Equation
%% \ref{eq:polyrestriction} does not vanish can only be learned if the
%% input dimension is constant and regularisation is used.




%\label{sec:additionalresults}

%% \fy{write}: Before, $\frac{\bw}{\effdim} \asymp 1$.
%% Here we consider the regimes $\frac{\bw}{\effdim} \to \infty$ 

%% This subsection studies cases where $\bw$ is not equal to
%% $\frac{1}{\effdim}$. Clearly, it is not difficult to verify that we
%% can extend Theorem \ref{thm:main_text} to the case where $\bw \asymp
%% \frac{1}{\effdim}$. Hence, we are only interested in settings where
%% $\bw = o(\frac{1}{\effdim})$ or $\bw =
%% \omega(\frac{1}{\effdim})$. Unfortunately, since this Lemma
%% \ref{lm:innerpr} implies that in this case, the norm of $\bw
%% \xind{i}$, $ \| \bw\xind{i} \|_2^2 $, either almost surely diverges or
%% goes to zero, we cannot make the same general statement as before. The
%% following paper proves for the $\alpha$-exponential kernel
%% $\kerfunc{\xk}{\xkd} = \exp(-\| \xk-\xkd \|_2^{\alpha})$ with $\alpha
%% \in (0,2)$ how the kernel estimator cannot be overcome the polynomial
%% approximation barrier when $\bw\effdim\to\infty$ polynomially and
%% $\bw\effdim \to 




==> sections/Sections_ICML/new_section4.tex <==


\vspace{-0.05in}
\subsection{Discussion of theoretical results}
\label{sec:contributions}

%% We would now like to pinpoint our contributions in the context of
%% previous work in more detail.
In our work, we show that the polynomial approximation
barrier~\eqref{eq:biaslb} is a rather general phenomenon and not
restricted to a few specific distributions or choices of $\bw$.
%% our unified treatment
%% we
%% unify and extend the settings of previous works and explicit novel
%% insights that we gain as a direct consequence. 
In particular, we show that it holds beyond the sphere
and depends solely on the growth rate of
$\effdim=\tr(\inputcov)/\opnorm{\inputcov}$, where
the covariance matrix $\inputcov$ defines the
input distributions as in Assumption~\Adone.  We summarize our
setting and alongside those of previous works in Table~\ref{tab:settings}.
We now want to discuss 
the consequences of our unified treatment of previous works
and highlight novel insights that could prove important
in practical settings and for future work.
\vspace{-0.1in}
\paragraph{Implications of the unified treatment}
First, the fact that our results hold true for \emph{arbitrary}
covariance matrix structures stands in contrast to linear regression
where consistency can (only) be guaranteed for spiky
covariance matrices \cite{Bartlett20,Muthukumar20}. 
%where specific covariance structures can reach consistency
Furthermore, for inner product kernels, we can combine our negative
result together with the positive result in \cite{Liang20b} to
conclude that functions with bounded Hilbert norm asymptotically
converge to polynomials in the $\Ell_2(\prob)$ sense where $\prob$
satisfies \Akone (see Corollary~\ref{cr:rkhsnorm_liang} for a precise
statement).

\vspace{-0.1in}
\paragraph{Eigenvalue decay}
Furthermore, by explicitly showing that the polynomial barrier
persists for all $\alpha$-exponential kernels with $\alpha \in (0,2]$
  (that have vastly different eigenvalue decay rates), we provide a
  counterpoint to previous work that suggests consistency for $\alpha \to 0.$
  %% %% rotationally invariant kernels with vastly different eigenvalue
  %% decay rates determining the smoothness respectively spikiness of the
  %% estimator.  This is particularly interesting in light of previous
  %% work that suggests that $\alpha \to 0$ could improve generalization.
  In particular, \cite{Belkin19} prove minimax optimal rates for the
  Nadaraya-Watson estimators with singular kernels for fixed
  dimensions and empirical work by \cite{Belkin18c,Wyner17} suggests that
  spikier kernels have more favorable performances.  Our results
  suggest that in high dimensions, the effect of
  eigenvalue decay (and hence ``spikiness'') may very well be dominated by
  asymptotic effects of rotationally invariant kernels.
  We discuss possible follow-up questions in Section~\ref{sec:discussion}.
  %% for a discussion on resulting future
%% directions.

\vspace{-0.1in}
\paragraph{Feature selection}
We now want to discuss practical implications of our theoretical
results.  For ground truths that are inherently higher-degree
polynomials that depend on all dimensions, our theory predicts that
consistency of kernel learning with standard RBF or inner product
kernels is out of reach if the data is high-dimensional. In practice
however, it is possible that not all dimensions carry equally relevant
information.  Especially in the case when the function depends only on
a few input dimensions, we expect the bias to have a U-shape:
including more features should first decrease the bias (until it
includes all relevant features) before it increases again as
high-dimensional asymptotics start to kick in. We want to emphasize
that although it may ring a familiar bell, this behavior \emph{is not}
due to the classical bias-variance trade-off, since it even applies to
the noiseless case. In Section~\ref{sec:expreal} we show that this
U-curve behavior can indeed be observed for real-world data.
\vspace{-0.1in}

% 
% %% We would now like to pinpoint our contributions in the context of
% %% previous work in more detail.
% In our work, we show that the polynomial approximation barrier is a
% rather general phenomenon, not restricted to a few select
% distributions and choices of bandwidth. We now want to discuss how we
% unify and extend the settings of previous works and explicit novel
% insights that we gain as a direct consequence. 
% % \emph{changes to a vacuous one}.
% % \nr{When I read this last part of the sentence, it seems like you are saying: the inductive bias is less and less strong (since it changes to a vacuous). If I didn't misunderstand, you mean quite the opposite, i.e. the inductive bias becomes very strong and the resulting estimators are instead vacuous, not the inductive bias.}
% % 
% 
% %% \fy{this E.1 stuff i wouldn't do, no one does looks bad and attracts too much attention) since we already have it in intro might cut altogether}
% %% In our work, we show that the polynomial approximation barrier is
% %% a rather general phenomenon, not restricted to a few select distributions
% %% and choices of bandwidth.
% %% %% not
% %% %% specific to \emph{uniform} distributions on the sphere or the product of two spheres, but rather a very general phenomenon.
% %% In particular, 
% %% %compared to \cite{Ghorbani19,Ghorbani20} \fy{again and again?}
% %% we extend previous work in three significant ways:
% %% %% the settings for which the statements
% %% %% in Theorem~\ref{thm:main_thm} holds 
% %% %We explicitly prove that it holds for
% %% \begin{enumerate}
% %% \item[(E.1)] We allow general covariance model distributions (assumption \Bdone) both in $\RR^d$ and projected onto the sphere. As a result, we unify the settings studied in the existing literature (see Table~\ref{tab:settings})
% %%   \item[(E.2)] We cover rotationally invariant kernels with vastly different eigenvalue decay rates determining the smoothness respectively spikiness of the estimator. 
% %%   \item[(E.3)] We are the first to include the cases when the scale parameter $\bw$ decreases or increases faster than $\effdim$.
% %% \end{enumerate}
% 
% %% Our proof
% %% framework includes and extends previous assumptions on the
% %% distribution and kernels, and establishes a polynomial approximation
% %% barrier for the ridge regression estimate and minimum norm
% %% interpolant.
% \fy{paragraph captions will go}
% \paragraph{consequences of unifying} First, we show that the polynomial approximation
% barrier~\eqref{eq:biaslb} holds for distributions beyond the sphere
% and depends solely on the growth rate of $\effdim=\tr(\inputcov)/\opnorm{\inputcov}$,
% where $\inputcov$ induces the distributions as defined in
% Assumption~\Adone.  We summarize our setting and compare it with
% previous work in Table~\ref{tab:settings}.  Together with the
% consistency result in \cite{Liang20b}, for inner product kernels we
% can also conclude that functions with bounded Hilbert norm
% asymptotically converge to polynomials in the $\Ell_2(\prob)$ sense
% where $\prob$ satisfies \Akone (see Corollary~\ref{cr:rkhsnorm_liang}
% for a precise statement).  Finally, the fact that our results hold
% true for arbitrary covariance matrix structures stands in contrast to
% linear regression where specific covariance structures can reach
% consistency \cite{Bartlett20,Muthukumar20}.
% 
% \paragraph{eigenvalue decay}
% Furthermore, we explicitly show that the polynomial barrier
% persists for all $\alpha$-exponential kernels for $\alpha \in (0,2]$
%   that have vastly different eigenvalue decay rates.  
%   %% rotationally invariant kernels with vastly different eigenvalue
%   decay rates determining the smoothness respectively spikiness of the
%   estimator.  This is particularly interesting in light of previous
%   work that suggests that $\alpha \to 0$ could improve generalization.
%   In particular, \cite{Belkin19} prove minimax optimal rates for the
%   Nadaraya-Watson estimators with singular kernels for fixed
%   dimensions and empirical work by \cite{Belkin18c,Wyner17} suggests that
%   spikier kernels have more favorable performances.  Based on our
%   results, we can conclude that in high dimensions, the effect of
%   eigenvalue decay (and hence ``spikiness'') is dominated by
%   asymptotic effects that are specific to rotation invariant kernels.
%     We refer to
% Section~\ref{sec:discussion} for a discussion on resulting future
% directions.
% 
% \paragraph{feature selection}
% We now want to discuss some practical implications of our theoretical
% results.%%  Our theory predicts that as the dimension increases compared
% %% to the number of samples, kernel estimators cannot predict better than
% %% low-degree polynomials. 
% For ground truths that are inherently higher-degree polynomials
% depending on all dimensions, our theory predicts that consistency of
% kernel learning with \kd{standard instead of vanilla ?} RBF or inner product kernels is out of
% reach if the data is high-dimensional. In practice however, it is
% possible that not all dimensions carry relevant information.  In
% particular, in the case when the function depends only on a few
% dimensions, we expect that as we increase dimensionality, the bias
% first decreases until it includes all relevant features and then
% increases again due as high-dimensional asymptotics start to kick in\fy{reprhase}, forming a
% U-curve. We want to emphasize that albeit it may ring a familiar bell,
% this behavior \emph{is not} due to the
% classical bias-variance trade-off, since it even applies
% to the noiseless case. In Section~\ref{sec:expreal} we show that this
% U-curve behavior can indeed be observed on real-world data.



% In the process of unifying the existing spherical
% (\cite{Ghorbani19,Ghorbani20}) and covariance model distributions
% (\cite{Liang20b,Liang20a}) to achieve E.1, we were able to
% cleanly identify that the polynomial approximation barrier $m$ depends
% only on the growth rate $\beta$ of $\effdim = \tr(\inputcov)$, i.e. $\effdim \asymp n^{\beta}$.  
% \kd{I see why you like this point here, but the statement can also lead to 
% confusions. What you say here is a bit too much - I would rather say that 
% this opens an interesting discussion how}
% Furthermore, our unified treatment in Theorem~\ref{thm:main_thm} and consistency results for
% functions (sequences) with asymptotically bounded norm \cite{Liang20a} together 
% indicate that functions with bounded Hilbert norm are in some regions asymptotically polynomials as we require
% Equation \eqref{eq:biaslb} to vanish. In fact, we can partially answer this question in Corollary~\ref{cr:rkhsnorm_liang}
% in~\suppmat~\ref{sec:rkhsnorm_liang}.
% \kd{remove:
% Furthermore, our unified
% treatment in Theorem~\ref{thm:main_thm} and consistency results for
% functions (sequences) with asymptotically bounded norm \cite{Liang20a}
% implies the interesting fact that bounded Hilbert norm functions of inner product kernels
% are asymptotically polynomials (see Corollary~\ref{cr:rkhsnorm_liang}
% in~\suppmat~\ref{sec:rkhsnorm_liang}).} ​
%% inputs drawn from
%% a covariance model $\prob_X$ as in Assumption~\Adone, functions
%% with bounded Hilbert norm asymptotically converge to
%% polynomials. Corollary~\ref{cr:rkhsnorm_liang} provides a precise statement. in the $\Ell_2(\prob_X)$ sense. 

%% consequences
%% bounded hilbert norm vanishes

% spikiness doesn't matter


%% First, we allow general covariance model distributions (assumption
%% \Bdone) both in $\RR^d$ and projected onto the sphere. As a result, we
%% unify the settings studied in the existing literature (see
%% Table~\ref{tab:settings}).  In the process of unifying the existing
%% spherical (\cite{Ghorbani19,Ghorbani20}) and covariance model
%% distributions (\cite{Liang20b,Liang20a}), we were able to cleanly
%% identify that the polynomial approximation barrier $m$ depends only on
%% the growth rate $\beta$ of $\effdim = \tr(\inputcov)$, i.e. $\effdim
%% \asymp n^{\beta}$.  \kd{I see why you like this point here, but the
%%   statement can also lead to confusions. What you say here is a bit
%%   too much - I would rather say that this opens an interesting
%%   discussion how} Furthermore, our unified treatment in
%% Theorem~\ref{thm:main_thm} and consistency results for functions
%% (sequences) with asymptotically bounded norm \cite{Liang20a} together
%% indicate that functions with bounded Hilbert norm are in some regions
%% asymptotically polynomials as we require Equation \eqref{eq:biaslb} to
%% vanish. In fact, we can partially answer this question in
%% Corollary~\ref{cr:rkhsnorm_liang}
%% in~\suppmat~\ref{sec:rkhsnorm_liang}.  \kd{remove: Furthermore, our
%%   unified treatment in Theorem~\ref{thm:main_thm} and consistency
%%   results for functions (sequences) with asymptotically bounded norm
%%   \cite{Liang20a} implies the interesting fact that bounded Hilbert
%%   norm functions of inner product kernels are asymptotically
%%   polynomials (see Corollary~\ref{cr:rkhsnorm_liang}
%%   in~\suppmat~\ref{sec:rkhsnorm_liang}).}
%% previous works on the
%% consistency
%% of kernel regression (see Table~\ref{tab:settings}).
%% the
%% polynomial approximation barrier on the data distribution and show how
%% the parameter $\beta$ with $\effdim \asymp n^{\beta}$ determines the
%% maximum degree of the polynomials which can be consistently
%% approximated .



%% Further, we cover rotationally invariant kernels with vastly different eigenvalue decay rates determining the smoothness respectively spikiness of the estimator. This is particularly interesting in light of previous work that
%% suggests that $\alpha \to 0$ could improve generalization:
%% \cite{Belkin19} prove minimax optimal rates for the Nadaraya-Watson
%% estimators with singular kernels for fixed dimensions and empirical
%% work by \cite{Wyner17} suggests that spikier kernels have more
%% favorable performances.  Based on our results, we can conclude that in
%% high dimensions, the effect of eigenvalue decay (and hence
%% ``spikiness'') is dominated by asymptotic effects that are specific to
%% rotation invariant kernels. Instead, we show in the next section
%% how we can overcome the polynomial barrier for sparse ground truth functions 
%% by using feature selection. Indeed, we can even observe for real world datasets
%% that this is necessary in order to achieve optimal performance. 


%%  We also refer to a discussion of
%%  important implications and future avenues in Section~\ref{sec:discussion}.
 
%% \fy{why remove bandwidth. isn't that one of the most importnat}
%% \kd{I would remove this:
%% E.3 provides a partial (negative) answer to the important question \nr{question OF} whether
%% increasing the bandwidth at a faster rate than $\effdim$ could
%% mitigate the inconsistency for nonpolynomials. This is interesting
%% in view of both the positive result in \cite{Belkin19} for
%% singular kernels in fixed dimensions and the negative result
%% for any adaptive bandwidth for Laplace kernels \cite{Rakhlin18}.
%% }







\section{Experiments}
\label{sec:exp}



\begin{figure*}[t]
  \centering
          \begin{subfigure}{0.32\linewidth}
        \centering
  \includegraphics[width=\textwidth]{Plots_v2/interpolationmse.pdf}
         \vspace{-0.2in}
    \caption{Bias variance trade-off}
    \label{fig:biasvar}
    \end{subfigure}  
    \hfill
  \begin{subfigure}{0.32\linewidth}
    \centering
  \includegraphics[width=\textwidth]{Plots_v2/Building1_noiseless_old.pdf}
         \vspace{-0.2in}
    \caption{Residential housing - original}
    \label{fig:rh}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.32\linewidth}
    \centering
  \includegraphics[width=\textwidth]{Plots_v2/Building1_old.pdf}
         \vspace{-0.2in}
    \caption{Residential housing - add. noise}
    \label{fig:rh2}
      \end{subfigure}
             \vspace{-0.1in}
          \caption{\small{% $5$-folds cross validated
              \fy{change caption with new order}
             (a): The bias-variance trade-off of the minimum norm interpolant normalized by $\Bias(0)$ for 
             a synthetic experiment as a function of selected features (see details in Section \ref{sec:expreal}). The trends are reversed compared to the usual bias-variance curve as a function of model complexity and reflect our theoretical results: the bias term dominates the risk as dimension increases while the variance monotonically decreases with dimension. This behaviour can also be observed for the \textit{residential housing} dataset (b) without and (c) with additive synthetic noise where the risk of
            Ridge regression and interpolation follow similar trends that we hence attribute to the bias. }}
    \label{fig:realworld}
    \vspace{-0.2in}
\end{figure*}
% 
% \kd{remove - too long:
% 
% In this section we describe our synthetic and real-world experiments that
% demonstrate how the predictions from our high-dimensional asymptotic
% results in Section~\ref{sec:3} already kick in when $d\sim 50$. \kd{This sounds like the focus is to show that the asymptotics kick in early which is a bit misleading} Furthermore,
% we provide synthetic and
% real-world experiments in Section~\ref{sec:expreal} that illustrate how
% the risk follows a U-curve for both noisy and noiseless data
% and hence underline the importance of feature selection in high dimensional
% kernel learning.}

In this section we describe our synthetic and real-world experiments to further illustrate our theoretical results and underline the importance of feature selection in high dimensional
kernel learning.


\subsection{Hilbert space norm increases with dimension $d$}
\label{sec:expnorm}
In Figure \ref{fig:rkhsnorm} we demonstrate how the Hilbert norm of
the simple sparse linear function $\fexp(\x) = \xel{1}$ grows with
dimension $d$.  We choose the scale
parameter $\bw = d$ and consider the Hilbert space induced by the
scaled 
%% the Hilbert norm on $\XX = [0,1]^d$ of the function $\fexp(\x) =
%% \xel{1}$ for the
Gaussian $\kernf(\xk,\xkd) = \exp(-\frac{\| \xk-\xkd
  \|^2}{\bw})$, Laplace $\kernf(\xk,\xkd) = \exp(\frac{ \| \xk-\xkd
  \|_2}{\sqrt{\bw}})$ and exponential inner product $\kernf(\xk, \xkd)
= \exp(-\frac{\xk^T\xkd}{\bw})$ kernels.
%% where we choose $\bw = d$.  In
%% order to estimate the norm we draw $7500$ i.i.d random samples from
%% the uniform distribution on $\XX$.
To estimate the norm, we draw $7500$ i.i.d random noiseless
observations from the uniform distribution on $\XX=[0,1]^d$.
\kd{remove:and
compute the minimum norm interpolant $\fexp(\X)^\top \kermat
\fexp(\X)$, where $\fexp(\X)$ is the vector with entries $\fexp(\X)_i
= \fexp(\x_i)$.}


\subsection{Illustration of polynomial approximation barrier}
\label{sec:expsynthetic}
We now provide details for the numerical experiments in
Figure~\ref{fig:polymodels},\ref{fig:taudependence} that illustrate
the lower bounds on the bias in Theorem~\ref{thm:main_thm} and
Theorem~\ref{thm:otherchoicesoftau}.
%% our lower bounds on the bias for
%% different scale parameters~\eqref{eq:biaslb}
%% %,\eqref{eq:biasflatlimit}. 
For this purpose we consider the
following three different distributions that satisfy the assumptions
of the theorems and are covered in previous works
\begin{itemize}
    \item \textbf{$\prob_1$, $\prob_2$:} $\standardrv_{(i)} \sim \Normal(0,1)$, $d = \floor{n^{\beta}}$ and $\inputcov = \textrm{I}_d$. $\prob_1$: $X = \inputcov^{1/2} \standardrv$, $\prob_2$: $X = \frac{\sqrt{d} \inputcov^{1/2} \standardrv}{ \|\inputcov^{1/2} \standardrv \|} $ .
    \item \textbf{$\prob_3$:} $X = \inputcov^{1/2} \standardrv$, $\standardrv_{(i)} \sim \Uniform([-u,u]^d)$, with $u$ s.t. unit variance, $d = n$ and $\inputcov$ diagonal matrix with entries $(1 - ((i-1)/d)^{\kappa})^{1/\kappa}$ and $\kappa \geq 0$ s.t. $\trace(\inputcov) = n^{\beta}$ .
\end{itemize}
We primarily use the Laplace kernel with $\bw = \tr(\inputcov)$
except in \ref{fig:taudependence}.
% \kd{I would just remove this:
% Model 1 is also a special case of the setting studied in
% \cite{Liang20b}, Model 2 corresponds to the one in \cite{Ghorbani19}
%  and Model 3 to the one in \citet{Liang20a}. }
% We use the same kernels as in Section \ref{sec:expnorm}  with $\bw = \trace(\inputcov)$ and in particular if not further 
% specified the Laplace kernel.
% $\kerfunc{\xk}{\xkd} = \exp\left(- \frac{ \| \xk-\xkd \|_2}{
%   \sqrt{\bw}}\right)$.
%% In this section, we
%% empirically study kernel regression for the Laplace kernel
%% $\kerfunc{\xk}{\xkd} = \exp\left(- \frac{ \| \xk-\xkd \|_2}{
%%   \sqrt{\bw}}\right)$ with $\bw = \trace(\inputcov)$.
\footnote{We choose the Laplace kernel because of its numerical
  stability and good performance on the high dimensional datasets
  studied in \cite{Belkin18c,Geifman20}. Other kernels can be found in
  the \suppmat~\ref{sec:appexp}.} and study two 
sparse monomials as ground truth functions, $\fexp_1(\x) = 2 \xel{1}^2$ and
$\fexp_2(\x) = 2 \xel{1}^3$. In order to estimate the bias, we fit the
minimum norm interpolant on noiseless observations and approximate the
expected squared error using $5n$ i.i.d. test samples. \\

\vspace{-0.05in} In Figure~\ref{fig:fig2a} and \ref{fig:fig2b}, we
plot the dependence of the bias on the parameter $\beta$ which
captures the degree of high-dimensionality, i.e. how large dimension
$d$ is compared to the number of samples $n$. We vary $\beta$ by
fixing $n$ and increasing $d$ (see also~\suppmat~\ for plots for fixed
$d$ and varying $n$). In Figure \ref{fig:fig2a} we demonstrate the
important consequence of our unifying framework that the polynomial
barrier only depends on the growth of the effective dimension
$\tr(\inputcov)$, parameterized by $\beta$ indepdent of the specific
choice of the distribution.\footnote{The differences in the absolute
  bias values between data models are due to the differences of
  $\|\fhatinterpol - \ftrue\|_{\Ell_2(\prob_X)}$ that explicitly
  depend on the underlying input model $\prob_X$.} The horizontal lines
that indicate the bias of the optimal linear fit $\flin$, show how for
large $\beta$, the kernel learning with the Laplace kernel performs
just as well as a linear function.  Figure \ref{fig:fig2b} shows the
bias curve as a function of $\beta$ just for model 1 but different
choices of $n$. The bias curves are identical from which we conclude
that we already enter the asymptotic regime for $d,n$ as low as $d\sim
50$ and $n\sim 2000$.
%% which
%% implies that our asymptotic theory is already applicable for
%% relatively low $n,d$.

Figure \ref{fig:taudependence} illustrates how the bias depends on the
scale parameter $\bw$ for different $\beta$ with $n=2000$. We generate
samples using $\prob_1$ and the ground truth $\fexp_2$ and plot the bias
of the minimum norm interpolator for the Laplace, exponential inner
product and Gaussian kernel.  For the latter, the minimum is obtained
around $\bw = d$.  For the Laplace and exponential inner product
kernel, the bias achieves its minimum at the flat limit $\bw
\to\infty$.  Given that our lower bounds hold for both $\bw = d$ and
$\bw \to\infty$ (Theorems~\ref{thm:main_thm} and
\ref{thm:otherchoicesoftau}), we speculate that there might not
exist an intermediate scaling regime for $\bw$ that can
break the polynomial approximation barrier.


% In Figure~\ref{fig:fig2a} and \ref{fig:fig2b}, we study the dependence of
% the bias on the parameter $\beta$ which captures the degree of
% high-dimensionality, i.e. number of dimensions compared to number of
% samples.  We vary $\beta$ by fixing the number of samples and
% increasing the dimensionality $d$ (see also~\suppmat~\ for plots for
% fixed $d$). In Figure \ref{fig:fig2a} we demonstrate the important
% consequence of our unifying framework that the polynomial barrier only
% depends on the growth of the effective dimension, parameterized by
% $\beta$ and not on the specific model choice, or domain.
% \footnote{Note that the differences in the absolute values
% for the normalized bias among data models are due to the differences
% in the $\Ell_2(\prob_X)$ norms of $\fhatinterpol - \ftrue$ that depend
% on the underlying input distributions.}
% Furthermore, Figure \ref{fig:fig2b} shows the bias curve for different
% choices of $n$. The bias curves as a function of $\beta$ look
% identical and hence we can conclude that we indeed enter the asymptotic
% regime already for $d\sim 50$ and $n\sim 2000$ which implies that our
% asymptotic theory is already applicable for relatively low $n,d$.
% 
% %% and shows that we already enter the asymptotic regime for relatively low dataset sizes $n$. 
% 
% %% Finally we want to note that the differences in the absolute values
% %% for the normalized bias among data models are due to the differences
% %% in the $\Ell_2(\prob_X)$ norms of $\fhatinterpol - \ftrue$ that depend
% %% on the underlying input distributions.\\
% 
% 
% %% We can even observe in Figure \ref{fig:fig2a} that
% %% the shape of the bias curve with respect to $\beta$ is very similar
% %% for all studied input data distributions extending the inutions gained
% %% form our theoretical results.
% % This indicates that not just the lower bound from Theorem \ref{thm:main_thm} is ind to tight bounds on the bias. 
% 
% %% Furthermore, based on our results we expect that the bias increases step-wise as the degree of polynomials which we can approximate decrease with $\beta$.   
% %% Indeed, we can observe that phase transitions occur at around $\beta
% %% \sim 1/2$ for the degree-2 monomial $\fexp_1$ and at around $\beta \sim 1/3$
% %% and $ \beta \sim 1$ for the degree-3 monomial $\fexp_2$. For the
% %% latter, we want to note the flat region around $\beta \approx 0.5$
% %% which is due to the fact that the best degree-2 polynomial
% %% approximation of a degree-3 monomial around 0 is a linear
% %% function. Similar, holds for the degree-2 monomial where the best linear approximation around $0$ is a constant. Figure \ref{fig:fig2b} shows the 
% %% bias curve for differnt choices of $n$ and shows that we already enter the asymptotic regime for relatively low dataset sizes $n$. 
% %% Finally we want to note that the differences in the absolute values
% %% for the normalized bias among data models are due to the differences
% %% in the $\Ell_2(\prob_X)$ norms of $\fhatinterpol - \ftrue$ that depend
% %% on the underlying input distributions.\\
% 
% 
% 
% 
% %% a transition
% %% point, referred to as the approximation barrier $\beta \sim
% %% \frac{1}{k}$, the bias converges to the loss of 
% %% that only depends on the order $k$ of the polynomial
% %% and not on the specific distribution. When $\beta$ increases beyond
% %% $\frac{1}{k}$ 
% %observations and plot the risk for the minimum norm interpolator.
% %% The first experiments study the dependency of the bias on the parameter $\beta$. For each of the plots we draw $n = 5000$ samples
% %% from the specific distribution. Since this set of experiments studies the bias we can simply fit noiseless observations and plot the risk for
% %% the minimum norm interpolator. This is due to the linear dependency of the estimator $\fhatridge$ on the observations. 
% %% The plots in Figure ~\ref{fig:polymodels} show the empirical
% %% dependence of the bias on the hyperparameter $\beta$ and the ground
% %% truth.
% %% More specifically, for polynomials of degree $m$,
% %% Theorem~\ref{thm:main_thm} suggests that the risk should go to zero as
% %% $\beta$ decreases. Moreover, the transition should be independent of
% %% the distribution.
% 
% %% \fy{Honestly next
% %%   two sentences are a bit too complicated/detailed here without adding
% %%   much} Furthermore, we can see that the bias for the degree-3
% %% monomial $\fexp_2$ is constant around $\beta \approx 0.5$, which is
% %% exactly the phase transition for the degree-2 monomial $\fexp_1$. This
% %% agrees with our theory when noting that the best degree-2 polynomial
% %% approximation of $\fexp_2$ is a linear function.
% 
% 
% %% fact that the projection errors of
% %% the ground truth functions to the space of polynomials depend on the
% %% underlying probability distributions.
% 
% Figure \ref{fig:taudependence} illustrates how the bias depends on the scale
% parameter $\bw$ for different $\beta$ with $n=2000$.  We generate samples
% using Model 1 and the ground truth $\fexp_2$ and plot the
% bias of the minimum norm interpolator
% %% tackles the question whether the
% %% approximation barrier can be avoided by choosing a different scale
% %% parameter as a function of $n$.  For the ground truth $\fexp_2$
% %% sampled using Model 1, it shows how the bias depends on the scale
% %% parameter $\bw$ for different $\beta$ when $n=2000$,
% for the Laplace, Gaussian and exponential inner product kernel.
% %as in Section~\ref{sec:expnorm}.
% %% Gaussian (i.e. $\kernf(\xk,\xkd) = \exp(\frac{1}{\bw} \| \xk - \xkd
% %% \|_2^2)$) and exponential inner product (i.e. $\kernf(\xk,\xkd) =
% %% \exp(\frac{1}{\bw} \xk^T\xkd)$) kernels.
% We first note that for the Laplace and exponential inner product
% kernel, the minimum bias is achieved at the flat limit $\bw
% \to\infty$.  For the Gaussian kernel, the minimum seems to be obtained
% at $\bw = d$.  Given both that our lower bounds hold for both $\bw
% = d$ and $\bw \to\infty$ via Theorems~\ref{thm:main_thm} and
% \ref{thm:otherchoicesoftau}, these plots suggest that there
% might not exist a scale parameter in the intermediate regimes
% which can achieve consistency.
% %% We clearly observe a
% %% phase transition for all of the three plots occurring at $\bw =
% %% \effdim =d$. We use Model 1 to generate the data. We draw $n = 2000$
% %% input samples and interpolate the noiseless observations in order to
% %% estimate the bias. The ground truth function is set to $\fexp_2$ for
% %% all plots.
% 
% 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% feature selection %%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\subsection{Feature selection for high-dim. kernel learning}
\label{sec:expreal}
We now present experiments that demonstrate the U-shape of the bias
curve discussed in Section~\ref{sec:contributions} for synthetic and
real-world data. For a more complete picture, our experiments also
show that the risk curve preserves the U-shape even in the presence of
noise.
% 
% We now demonstrate the U-shape of the bias curve
% discussed in Section~\ref{sec:discussion} for
% synthetic and real-world data. For a more complete picture,
% our experiments actually show that even in the
% presence of noise, the risk curve preserves the U-shape.

\paragraph{Sparse functions}
For our synthetic experiments, we draw $n=500$ samples with inputs
from $\prob_1$ and noisy observations from a sparsely parameterized
function $y= 0.5\sum_{i=1}^4 \xel{2i+1}^2 - \sum_{i=1}^4 \xel{2i} +
\epsilon$ with uniform noise $\epsilon \sim \UU([-10,10])$.  We
increase $d$ by adding irrelevant dimensions and compute the bias and
variance of the minimum norm interpolator, estimated using $100$
independent draws for the observation noise. In
Figure~\ref{fig:biasvar}, we  observe that the  bias follows a
U-shape, the variance decreases with $d$ and the hence bias
dominates with increasing $d$ as asymptotics start to kick in. These
observations are in line with both our bias lower bounds and the upper
bounds on the variance in the literature (see e.g. \cite{Liang20b,
  Ghorbani20}), though a tighter analysis would be necessary to
rigorously show when the risk of the interpolator follows a U-shape as
opposed to a double descent curve. We leave this for future work.
%% specifically predict the U-shape instead 

\paragraph{Real-world data}
We further explore the outreach of our theory on real-world data that
does not necessarily follow the data distributions assumed in our
Theorem. For this purpose we checked out datasets with a large
number of features compared to the number of samples for which
classical methods can perform well (i.e. excluding images). 
In this section we show results on the regression dataset
\textit{residential housing} (RH) with $n=372$ and $d= 107$ to predict
sales prices from the UCI website \cite{Dua17}. Further datasets
can be found in \suppmat~\ref{sec:app_expreal}.  In addition, in order to
study the effect of noise, we generate an additional dataset (RH-2)
where we add synthetic i.i.d.  noise drawn from the uniform
distribution on $[-1/2,1/2]$ to the observations. The plots in
Figure \ref{fig:realworld} are then generated as follows.  We increase
the number of features using a greedy forward selection procedure. We
then plot the risk achieved by learning a kernel ridge and ridgeless
estimate using the Laplace kernel on the new subset of features.
See~\suppmat~\ref{sec:app_expreal} for further details.


Figure~\ref{fig:rh} that the risks of the minimum norm interpolator
and the ridge estimator are identical, indicating that the risk is
essentially equivalent to the bias. Hence our first conclusion is
that, similar to synthetic experiment, the bias follows a U-curve. For
the dataset RB-2 in Figure~\ref{fig:rh2}, we further observe that even
with additional observational noise, the U-shape of the risk persists
for both ridge and interpolation. This suggests that the
bias dominates in high dimensions, analogously to the synthetic
datasets.  We observe both trends in other high-dimensional datasets
discussed in~\suppmat~\ref{sec:app_expreal}. As a consequence, we can
conclude that at least for some datasets, feature selection is crucial
for kernel learning.  
 
Finally, we want to argue that the importance of feature selection for
the discussed real-world datasets when using kernel regression in high
dimensions does not necessarily contradict empirical work that
demonstrate good test performance of RBFs on other high-dimensional
data such as MNIST. In fact, the latter only suggests that linear or
polynomial fitting would do just as well which has indeed been
suggested in \cite{Ghorbani20}.

%% In order to reduce the enormous number of features
%% in the \textit{ALLAML} dataset with $d = 7129$ and $n=72$, we use the
%% feature selection algorithm in \cite{Chen17} to discard all except the
%% $100$ most relevant features.
%% Among the two target variables in
%% the \textit{Residential Housing} dataset we only consider the first
%% one (\textit{house prices}).
% We normalize both the features but normalize the observation vector using $\ell_1$ normalisation
% \fy{not clear its $\ell_1$ normalization}. \fy{this is confusing when
%   you first read it. why add noise and why only for residential
%   housing but not ALLAML?}  Every feature in both datasets is
% normalized to approximately satisfy the assumptions
% \Bdone-\Bdtwo. \fy{really don't get this, which model are you aiming
%   to approximately get?} \fy{some more comment on how distribution
%   relates to assumption} 
%

%% Even though this insight sounds
%% reminiscent of introductory machine learning courses, the reasoning
%% \emph{in high dimensions} is completely different to the
%% low-dimensional story: For fixed dimension, adding uninformative
%% dimensions enables overfitting to noise, leading to higher
%% variance. In high dimensions, it seems that additional dimensions
%% decrease the variance and degrade the bias. Even though prior work hints at this,


%% We first argue that for high-dimensional data with nontrivial
%% non-linear ground truth functions, it is often crucial to use kernel
%% regression only on a subset of features even for the noiseless case.
%% We want to emphasize that this does not stand in stark contrast to
%% high-dimensional tasks such as MNIST classification where kernel
%% methods using RBFs have been shown to work well \cite{Belkin18c} and
%% \cite{Geifman20} - it only suggests that linear or polynomial fitting
%% would do just as well (see \cite{Ghorbani20}).


%% \paragraph{Noiseless case}
%% We first note that without artificial noise, both datasets show
%% identical performance for the ridge estimate and interpolation.  We
%% hence conclude that the variance does not play a big role here.  and
%% the risk is essentially equivalent to the bias.  While in
%% fixed-dimensional theory, the bias curve decreases with model complexity,
%% the empirical results show unexpectedly, that the risk follows U-shaped
%% error curve with
%% no sign of a second descent even after $d>n$ \fy{sth for Vincent
%%   here}. In particular, in contrast to the double descent phenomenon,
%% after adding enough features to capture the signal of the data,
%% further increasing dimensionality only hurts the risk performance.

%% %% As a result,
%% we obtain the following datasets: \textit{ALLAML} with $n= 72$ and
%% $d=100$ and \textit{Residential Housing} with $n=372$ and $d= 107$.


%% Figure \ref{fig:realworld} shows the
%% cross validation classification error and risk obtained for the
%% Laplace kernel.
%We use cross validation to find the optimal scale and regularization
%parameters.
%for both kernel ridge regression and minimum norminterpolation. 

%% \paragraph{Noisy case}
%%  In order to study kernel learning in the presence of noise, we
%%  further take the \emph{Residential Housing} dataset and add synthetic
%%  i.i.d noise drawn from $\UU[-1/2,1/2]$. \fy{why not ALLAML}
%% %% in the presence of
%%  %% noise~\ref{fig:residentialhousing} and in low dimensions,

%% As expected, Figure~\ref{fig:residentialhousing} shows that ridge
%% regularization significantly improves the best test performance for a
%% low number of features. \fy{sasha?} Furthermore, even in the presence
%% of noise, the risk curve still follows a U-curve without a second
%% descent. This indicates that ...
%%  \fy{have to check what happens for even larger noise}
%% %% We conclude that in the presence
%% %% of noise and truly non-linear functions, regularization is indeed not
%% %% obsolete.

%% Together with Theorem~\ref{thm:main_thm} on the polynomial
%% approximation barrier which predicts that the bias increases with
%% ambient dimension, \fy{while variance is expected to decrease - variance
%%   bounds by others} the plots hence suggest that as
%% dimension increases, the effect of the bias starts to dominate.
%% This is in contrast to the usual bias variance tradeoff as a
%% function of model complexity where the variance increases with
%% complexity.





%% We make use of the $\alpha$-exponential kernel,
%% i.e. $k(\xk,\xkd) = \exp\left(- \frac{1}{ \tau^{\alpha/2}} \| \xk-\xkd
%% \|_2^{\alpha} \right)$, and the exponential inner product kernel,
%% i.e. $k(\xk,\xkd) = \exp\left(\frac{1}{\tau} \xk^\top
%% \xkd\right)$. Furthermore, we investigat the following two sparse
%% ground truth functions $\ftrue_2(\x) = 2 \xel{1}^2$ and $\ftrue_3(\x)
%% = 2 \xel{1}^3$.  In total $5000$ input data points \fy{passive: are
%%   used} for training and $25000$ for testing.

%% As a first step, we summarise our theoretical
%% predictions. Since Theorem \ref{thm:main_thm} does not depend on the
%% explicit structure of the covariance matrix $\inputcov$, we would
%% expect the two curves to look similar for both models. More precisely,
%% Theorem \ref{thm:main_thm} shows that the degree of the polynomial
%% decreases with respect to $\beta$ and hence, we would expect the bias
%% of $\ftrue_3$ to start to increase earlier than the one of
%% $\ftrue_2$. \\ For the experiment we draw $5000$ i.i.d input training
%% samples and set the observations to the ground truth value. Since the
%% estimator depends only linearily on the observations, we can write
%% \begin{equation}
%%     \Bias = \EE_x \left| \ftrue(\datamatrix)^\top (\kermat + \lambda \In)^{-1} \kstar(X) - \ftrue(X) \right|^2,
%% \end{equation}
%% which shows that the risk for noiseless observations equals exactly the bias of the estimator in the general case.
%% Furthermore, for this experiment it is sufficient to study the case where the estimator interpolates the data.

%% Figure \ref{fig:exp1_p1} shows the estimated bias for the ground truth
%% functions $\ftrue_2$ and $\ftrue_3$ where the input data is generated
%% by drawing $5000$ i.i.d random samples from the corresponding data
%% distribution specified in Model 1 and Model 2.  In addition, in order
%% to estimate the bias, we draw $25000$ i.i.d test samples drawn from
%% the same distribution. The bandwith is set to $\bw$ as in Theorem
%% \ref{thm:main_thm}. \\

%% As expected, we can observe that the bias
%% increases for both data models when increasing
%% $\beta$. Interestingely, we can see that the curves have a very
%% similar shape for both data models, however, the ratio between the
%% bias and the null estimator seems to differ significantly among the
%% data models. This indicates that there might exists

%% In the previous sections, we have already seen that both kernel ridge and "ridge-less" regression are not capable of approximating high degree polynomials. The question remains what the implications of our results for real world applications are. Both \citet{Belkin18c} and \citet{Geifman20} have shown that kernel methods can achieve good performance for high dimensional datasets, indicating that the effects described in Theorem \ref{thm:main_text} can be neglected. In contrast, we highlight that the degeneration of the estimator in high dimensions decreases the performance. In particular, we show real world tasks where feature selection, and thus the reduction of the dimensionality of the input data, is necessary in order to achieve good performance. \newline


==> sections/Sections_ICML/new_section5.tex <==

\section{Conclusion and future work}
\label{sec:discussion}

Kernel regression offers a
very elegant way to incorporate prior information of the specific problem by 
selecting the kernel. 
% induces a bias in the minimum norm regression problem in Equation \eqref{eq:krr},\eqref{eq:constraint_min_p}.
% One classical incentive to choose
% certain kernels to perform kernel regression lies in the
% inductive bias on the estimator via the specific induced Hilbert norm.
%% Kernel regression with  universal kernels imposes a strong
%% inductive bias on the estimator via the induced Hilbert norm, that
%% e.g. encourages smoothness.
Commonly used kernels in the literature are usually rotationally invariant and e.g. allow to incorporate prior information on smoothness (Gaussian) respectively spikiness (Laplace and small $\alpha$). Recent literature extends the line of results on consistency for such kernels by showing that this can be even achieved in high dimensional regimes.
% While such kernels seem most general in terms of approximation capacities, consistency is still unexpected since the
These results are surprising, since rotationally invariance means that exchanging any two input features does not affect the resulting estimator up to rotations of the input space, making these kernels a natural choice when
no prior information on the structure of the ground truth is available. 
% (as it treats all dimensions equally and independent) 
% seems most
%general in terms of approximation capacities, 
%\kd{This is a bit random:
%Previous works proved consistency of high-dimensional kernel learning
%for ridge and ridgeless estimators for different assumptions on the
%ground truth function and distributions.}

This paper presents a polynomial approximation barrier which puts previous 
results in perspective and shows that the induced bias in high dimensions enforces the estimator to reduce to a polynomial. 
% states that even though rotational symmetry is a natural choice when
% no prior information on the structure of the ground truth is available
% (as it treats all dimensions equally and independent) and seems most
% general in terms of approximation capacities, 
% the corresponding
% inductive bias in high dimensions is in fact restricting the average
% estimator to a polynomial.  
% As a result of our treatment of rotationally invariant kernels we prove this phenomenon for general distributions and scale
% parameters. %% how the inductive bias of rotationally invariant kernels
% %% degrades in the high-dimensional regime to encourage low-degree
%% polynomials.
Apart from novel and important technical insights that result from our
unified analysis (discussed in Sec.~\ref{sec:contributions}), our
result also opens up exciting new avenues for future research.

% \vspace{-0.2in}

\paragraph{Future work} 
% 
% \kd{In Section~\ref{sec:contributions}, we \fy{repeat: discussed} how the polynomial approximation barrier holds
% independent of the eigenvalue decay of the kernel.}
Since our polynomial approximation barrier holds
independent of the eigenvalue decay of the kernel, we conjecture
that in order to tackle challenging non polynomial problems in high dimensions, building the analysis upon the eigenvalue decay of the corresponding kernel could in fact lead to a
roadblock if the kernel is rotationally invariant.
In
particular, this includes recent results in the literature
studying the eigenvalue decay of fully connected NTK which have recently become
more popular in the deep learning theory literature \cite{Geifman20,Bietti21}.

% where the 
% underlying ground truth function goes beyond low degree polynomials,

%  studying their eigenvalue decay could in fact lead to a
% roadblock if the corresponding kernel is rotationally invariant.
% 
% 
% , in order to study well-performing highly parameterized functions
% in high dimensions when the ground truth is expected to be quite
% complex, \fy{reducing/simplifying..?} the function class to kernel
% regression and studying their eigenvalue decay could in fact lead to a
% roadblock if the corresponding kernel is rotationally invariant. 
% 
% In
% particular, this includes the treatment of neural networks by
% analyzing fully connected NTK that has recently become
% more popular in the deep learning theory literature.

Instead of primarily focusing on the eigenvalue
decay that helps to control variance, our lower bounds on the bias
suggest that for high-dimensional data, it is at least equally
important to understand how the specific function class, such as a
deep neural network, breaks the rotational symmetry of the kernel
function. Examples for such structural assumptions include sparse
parameterizations (i.e. dependence on few features) or compositional
structures (CNTK in \cite{Arora19} or \cite{Shankar20}).

Our real-world experiments in Section~\ref{sec:expreal} indeed confirm
this hypothesis for sparse functions and can be explained in
conjunction with fix-dimensional analysis. However, for more sophisticated
structures such as convolutions etc., it is not yet understood how the polynomial approximation barrier can be surpassed. Results in this direction would lead to important new insights for high-dimensional non-parametric learning.

\newpage
% believe 
% many apects are still not yet understood and can lead to important new insights for high-dimensional non-parametric learning.

%we believe a lot of analysis
%is still open and can lead to important new insights for
%high-dimensional non-parametric learning.

%% \paragraph{future work} For sparsity can use fix-dim.


%% Besides extending our results to arbitrary adaptive bandwidths,
%% showing consistency and tightening the barrier as a function of
%% $\beta$, 

%% Even though we have significantly extended previous results on
%% consistency to more general settings, consistency for these cases
%% still needs to be shown. In the process it would be necessary to show
%% a tight polynomial dependence as in \cite{Ghorbani20} and bound
%% the variance. 
%% %% When letting $\beta \to 0$ the bias bound vanishes for any
%% %% polynomial.
%% %% Hence, it remains to analyze the regime $\effdim \asymp
%% %% \log(n)$ in order to completely answer the question whether
%% %% for all high-dimensional regimes consistency can be guaranteed for general functions beyond
%% %% polynomials. Furthermore,
%% Furthermore, for even more sweeping inconsistency statements, it would
%% be crucial to complete our extensions to different $\bw$ scalings and
%% prove the lower bounds for arbitrary adaptive bandwidths as
%% \cite{Rakhlin18} for fixed dimensions.
%% % Furthermore, the current analysis does not cover the full spectrum of the bandwidth. In particular the case where $\bw/\effdim \to \infty$ is not yet fully understood. 
%% %% Besides, the degree $m$ in Theorem \ref{thm:main_thm} is not
%% %% necessarily tight and the variance is not included in the current
%% %% analysis.
%% Addressing these open questions would be an important step towards an
%% in-depth understanding of kernel methods in high dimensions. Other
%% interesting research avenues include further exploration of
%% consistency of more structured, e.g. compositional kernels and
%% whether the phenomenon persists for classification losses.
%% \fy{show flat limit for other kernels?}

%% Kernel regression with universal kernels such as the
%% $\alpha$-exponential kernels are commonly used to incorporate some
%% useful inductive bias towards e.g. smoother functions. Even though
%% this is indeed the case in the low-dimensional regime,
%% Theorem~\ref{thm:main_thm} implies that the inductive bias enforced by
%% the RKHS norm of rotationally invariant kernels becomes
%% problematic \emph{as $d$ increases} and high-dimensional asymptotic effects dominate
%% the estimator leading to a degeneration in the approximation capabilities limited to  polynomials of degree at most $m = 2\floor{2/\beta}$. 
%% %% In fixed dimension, $\alpha$-exponential kernels are e.g.
%% %% linked to increased smoothness of the kernel estimator.
%% \kd{remove, else it is too long:
%% Specifically, both the
%% ridge and minimum norm solution asymptotically become arbitrarily
%% close to an $m$-degree polynomial. In particular, the bigger $d$
%% compared to $n$, the \emph{smaller} the degree $m$.
%% Hence, in high dimensions, as $d$ (or $\beta$) increases,
%% the inductive bias enforces the estimator to degenerate and become vacuous.  
%% }

%% this quite defies against the low-dimensional
%% intuition that approximation capacity increases
%% with dimensionality and second 

%% Furthermore, we are also the first to prove that the polynomial
%% approximation barrier

%% persists beyond the usual scaling $\bw \asymp
%% \effdim$ in the literature, and in particular for the min-norm
%% interpolator in the flat limit $\frac{\bw}{\effdim} \to 0$.  Hence, we
%% provide a partial (negative) answer to the important question whether
%% increasing the bandwidth at a faster rate than $\effdim$ could
%% mitigate the inconsistency for nonpolynomials.

%% Our results explicitly highlight that the bias lower bound
%% holds for arbitrarily spiky kernels i.e. for $\alpha \to 0$ for
%% $\alpha$-exponential kernels. This insight is particularly interesting
%% in light of previous work that suggests that $\alpha \to 0$ could
%% improve generalization: \cite{Belkin19} prove minimax optimal rates
%% for the Nadaraya-Watson estimators with singular kernels for fixed
%% dimensions and empirical work by \cite{Wyner17} suggests that spikier
%% kernels have more favorable performances.
%% Based on our results, we can conclude that in high dimensions,
%% the effect of eigenvalue decay / spikiness is dominated by asymptotic
%% effects that are specific to rotation invariant kernels.

%% \paragraph{Breaking the barrier requires the right structural assumptions}
%% Our above statement on the polynomial inductive bias heavily uses the
%% the fact that the kernels are rotation invariant, which implies that
%% all dimensions are treated equally and independently and that the
%% kernel function is invariant against arbitrary arbitrary permutations.
%% While these minimalistic assumptions are useful when we don't have any
%% prior knowledge on the ground truth, our results indicate that without
%% imposing additional structural assumptions e.g. in the form of sparse
%% dependence on parameters \fy{ARD}, or e.g. convolutional structure as
%% in \cite{Arora19} \cite{Shankar20}, consistent learning of
%% non-polynomial functions is in fact not possible.

%% In Section~\ref{sec:exp}, we explore real-world and synthetic datasets
%% where we show in Figure~\ref{fig:realworld} that feature selection
%% indeed leads to a much lower MSE both in the noisy and noiseless case.




%% study the effect
%% of incorporating sparsity through feature selection in the next
%% experimental section and leave the rest for future work.

%% The advantage of rotationally invariant kernels is that they make
%% minimal assumptions on the rotational symmetries of the ground truth
%% functions. Breaking this invariance by using different kernels means
%% that we implicitly assume some underlying structure present in the
%% ground truth function. While it is evident that this can help to
%% improve performance, our results actually indicate that prior
%% knowledge on the rotational symmetries respectively non symmetries of
%% the ground truth function is necessary to consistently learn beyond
%% low degree polynomials in high dimensions.

%% The most straight forward way to obtain a non rotationally invariant
%% kernel to use some feature selection algorithm to obtain prior
%% knowledge on the relevant features. The resulting kernel depends then
%% only on a few features and is therefore clearly also no longer
%% rotationally invariant. Figure \ref{fig:realworld} shows that this is
%% indeed necessary for sparse non linear functions to achieve good
%% performance in high dimensions. However, the remarkable performances
%% on image data of non rotationally invariant kernels such as the
%% convolution NTK \cite{Arora19} and the compositional kernels
%% \cite{Shankar20} suggest that we can surpass the polynomial
%% approximation barrier in high dimensions even when with kernels which
%% make use of all features.  \kd{So what is the point here, I really
%%   want to say that we need to have some prior information on the
%%   structure of the ground truth function in order to learn
%%   consistently beyond polynomials (which are arguably simple
%%   functions) - the nice thing is that we can make bring this argument
%%   since our results apply to much more general settings than Ghorbani}





%% direction points at the study of
%% non-rotationally invariant kernel functions and analyses whether
%% similar statements to the polynomial barrier described in this paper
%% can be made. This type of research could lead to helpful intuitions
%% for the good performances of non rotationally invariant kernels like
%% compositional kernels \cite{Shankar20} on image data.

%% Finally, from a
%% non asymptotic view point it is not clear when we enter which
%% asymptotic regime. In fact, for given $n,d$ it is currently not
%% possible to determine whether we observe a behavior similar to the one
%% predicted for the asymptotic regime $\beta = \log(d)/\log(n)$ or for
%% the asymptotic regime $d = \gamma n$ with $\gamma = d/n$. Answering
%% this question is a key task in order to draw more refined conclusions
%% on the practical implications of our theory.



==> sections/old_sections/Section1.tex <==

\begin{abstract}
The abstract...
\end{abstract}


\section{Introduction}

\Comment{Need to rewrite completely} \\

Recent literature on high dimensional kernel ridge and in particular "ridge-less" regression suggests that inner product kernels show good approximation capabilities in certain regimes where the data is generated form a linear co variance model, $Z_i = \Sigma_d^{1/2} \tilde{Z_i}$ \cite{Liang20b,Rakhlin19,Liu20}. In particular, in \cite{Liang20b} the authors have shown that asymptotically consistency for $n,d \to \infty$ can be reached in regimes where $d \asymp n^{\beta}$ and $\beta <  1$. Furthermore, in \cite{Rakhlin19,Liu20}, the regime where $n \asymp d$ is studied including examples where a favourable choice of the covariance matrix $\Sigma_d$ can also lead to asymptotically consistent estimators.
Such results have strong similarities with results from the recent literature on linear regression \cite{Hastie20,Bartlett20}. For instance, it was shown in \cite{Bartlett20}
that the high dimensional linear "ridge-less" regression can reach asymptotically consistency under certain assumptions on $\Sigma_d$ and given that the ground truth is itself a linear function. 
\\\\





==> sections/old_sections/Section2.tex <==

\section{Background}
\subsection{Data Distribution}
 Let $n$ be the amount of training points and let $\tilde{\textbf{Z}} = \{\tilde{Z}_i\}_{i=1}^n$ be $d(n)$ dimensional vectors with entries $|\tilde{Z}_i[k]|$ consisting of i.i.d random variables of zero mean and unit variance. In order to make use of the strong concentration bounds for Lipschitz continuous functions of vectors of i.i.d. random variables, we additionally assume that $\tilde{Z}_i[k]$ is either a Gaussian random variable or bounded from both sides by some constant $c_Z$ independent of $n$. Let $\textbf{Z} = \{ Z_i \}_{i=1}^n$ be the input data generated from
 \begin{equation}
     \label{eq:data} 
     Z_i=  \Sigma_d^{1/2} \tilde{Z}_i 
 \end{equation} 
 with $\Sigma_d$ a positive semi definite co variance matrix. We assume that $||\Sigma_d||_2 = 1 $ and
 $\trace(\Sigma_d) \asymp n^{\beta}$
 with $\beta \in (0,1]$. As a consequence, we have that $\trace(\Sigma_d) \leq d(n)$. Besides this constraint, we do not make any further assumption on $d(n)$, meaning that $d(n)$ may be arbitrarily large. \\\\
In this paper, we are interested in studying kernel functions $k_{\tilde{\tau}}(Z_i,Z_j) = k(\tilde{\tau} Z_i, \tilde{\tau} Z_j)$ depending on a scale parameter $\tau$. It is therefore equivalent to analyse the algorithms with respect to the input data set $\textbf{X} = \{X_i\}_{i=1}^n$ where 
$$ X_i = \left(\sqrt{\trace(\Sigma_d)}\right)^{-1} Z_i$$
and $\tau = \sqrt{\trace(\Sigma_d)} \tau$.
The advantage of this formulation is that the random variable $X_i^T X_j$ has mean $\mathbb{E}~  X_i^TX_j = \delta_{i,j}$, where $\delta_{i,j}$ denotes the Kronecker-$\delta$ function, and variance
$$ \textrm{Var}(X_i^TX_j)  =\begin{cases}
    \trace(\Sigma_d)^{-2} \left(2\trace(\Sigma_d) + 3\mu_4 \trace(\Sigma_d \circ \Sigma_d) \right), & i=j.\\
  \trace(\Sigma_d)^{-1},  & i \neq j 
    \end{cases}$$
where $\mu_4$ is the fourth moment of the entries of $Z_i[k]$. We refer to \cite[Lemma~A.1]{el2010spectrum} for a proof of this fact. In fact we can show that 
\begin{lemma}
\label{lm:innerpr}
For any $\epsilon > 0$,
\label{lm:norm}
\begin{equation}
\label{eq:innerpreq}
    \max_{i,j }\left| X_i^T X_j- \delta_{i, j}\right| \leq n^{-\beta/2}log(n)^{1+\epsilon} ~~~ a.s.
\end{equation}
and
\begin{equation}
    \max_{i,j }\left|\lvert \lvert X_i -  X_j\rvert\rvert_2^2- 2(1-\delta_{i, j})\right| \leq n^{-\beta/2}log(n)^{1+\epsilon} ~~~ a.s.
\end{equation}
\end{lemma}
\begin{remark}
\label{rm:astoinp}
The almost sure condition is with respect to the sequence of data sets $\textbf{X}$ induced by $n \to\infty$. As may be seen in the proof of Lemma \ref{lm:innerpr}, we can replace the almost sure condition with an in probability condition. I.e for any $\epsilon>0$ there exists a constant $C>0$ such that for any $n$ sufficiently large, Equation \ref{eq:innerpreq} holds true with probability $\leq n \exp(-C \log(n)^{1+\epsilon})$ over the draws of $\textbf{X}$. 
\end{remark}
Finally, given a set of inputs $\textbf{X}$, we assume that we observe a vector of observations $Y$ with entries $Y_i$ independently drawn form the conditional distribution $Y_i \sim P_{Y \vert X}(.\vert X = X_i)$. Furthermore, let $f^*: \mathbb{R}^{d} \to \mathbb{R}$ be the mean of $P_{Y|X}(.|X)$, i.e. $\mathbb{E}_{y \sim P_{Y \vert X}(.\vert X)} y =  f^*(X)$. The function $f^*$ is usually referred to as the ground truth function. We assume that for ever $n$, $\vert f^* \vert$ is uniformly bounded by some constant $C_f$ independent of $n$.
\subsection{Kernel Ridge Regression}
 Let $k: \mathbb{R}^d \times \mathbb{R}^d \to \mathbb{R}$ be some positive definite kernel, i.e. where for any set of input vectors $\textbf{X}$ the empirical kernel matrix $K$ with entries $K_{i,j} = k(X_i,X_j)$ is positive semi definite. We assume that $k$ remains fixed for every $n$ and define $k_{\tau}(X,X') = k(\tau X, \tau X')$ to be the scale dependent kernel with scale parameter $\tau \in \mathbb{R}_+$ depending $n$. For every positive definite kernel and set $\mathcal{X} \subseteq \mathbb{R}^d$, there exists a unique corresponding reproducing kernel Hilbert space $\mathcal{H}$ (RKHS, see standard sources \cite{Wahba90,Berlinet04,Smola98}), consisting of functions mapping $\mathcal{X}$ to $\mathbb{R}$. We denote with $\langle.,.\rangle_{k}$ the corresponding inner product of the RKHS and by $\lvert\lvert . \rvert\rvert_{\mathcal{H}} := \sqrt{\langle.,.\rangle_{k}}$ the corresponding norm.\\
Given a set of data points $\textbf{X}$ and observations $Y$, the estimator of kernel ridge regression with ridge parameter $\lambda > 0$ is defined to be the solution of
\begin{equation}
\label{eq:krr}
    \hat{f}_{\lambda} = \underset{f \in \mathcal{H}}{\arg\min} ~~\sum_{i=1}^n \left(Y_i - f(X_i)\right)^2 + \lambda \lvert\lvert f \rvert\rvert_{\mathcal{H}} .
\end{equation}
and for $\lambda = 0$, $\hat{f}_{0} = \lim_{\lambda \to 0} \left[ \underset{f \in \mathcal{H}}{\arg\min} ~~\sum_{i=1}^n \left(Y_i - f(X_i)\right)^2 + \lambda \lvert\lvert f \rvert\rvert_{\mathcal{H}} \right]$.
 In the important special case where $\lambda = 0$, the estimator interpolates the data commonly referred. The resulting algorithm is commonly referred to as kernel "ridge-less" regression or kernel interpolation. In fact, one can see that when $\lambda =0$, the solution $\hat{f}_{\lambda}$ satisfies the following constraint minimisation problem 
 \begin{equation}
 \label{eq:constraint_min_p}
     \begin{split}
         \hat{f}_0 = \underset{f \in \mathcal{H}}{\arg\min} ~ \lvert\lvert f \rvert\rvert_{\mathcal{H}} ~~ \textrm{such that}~~ \forall i:~f(X_i) = Y_i 
     \end{split}
 \end{equation}
Surprisingly, the Representer Theorem \cite{Schoelkopf01} derived the following closed form expression for $\hat{f}_{\lambda}$: 
\begin{equation}
\label{eq:kernelridge}
    \hat{f}_{\lambda}(X^*) = Y^T (K(\textbf{X},\textbf{X})+ \lambda \textbf{I}_n)^{-1} K(\textbf{X},X^*) 
\end{equation}
where $K(\textbf{X},X^*) \in \mathbb{R}^{n}$ denotes the vector with entries $K(\textbf{X},X^*)_i = k_{\tau}(X_i, X^*)$. In this paper, we assume that $K$ is a strictly positive definite matrix and hence Equation \ref{eq:kernelridge} is well defined, which is guaranteed to be the case for universal kernels such as the Gaussian or Laplacian RBF kernels, given that the vectors in $\textbf{X}$ are distinct. For the brevity of notation, we write $K$ instead of $K(\textbf{X},\textbf{X})$ and $K^*$ instead of $K(\textbf{X},X^*)$.  \\
In this paper, we are interested in studying continuous rotational invariant kernels $k: \mathbb{R}^d \times \mathbb{R}^d \to \mathbb{R}$. More explicitly, for any $O \in \mathcal{O}(d(n))$, where $ \mathcal{O}(d(n))$ is the group of rotation matrices, and for any $X,X' \in \mathbb{R}^{d}$, we assume that $k(X,X') = k(O*X, O*X')$. \\
Given an estimator $\hat{f}_{\lambda}$, we are interested in studying the risk of the estimator, defined as
\begin{equation}
    \label{eq:risk}
    \mathbb{E}_{X^*,Y} ||\hat{f}_{\lambda}(X^*) - f^*(X^*)||^2 = \mathbb{E}_{X^*} || \mathbb{E}_{Y}\hat{f}_{\lambda}(X^*) - f^*(X^*)||^2 + \mathbb{E}_{X^*} || \mathbb{E}_{Y}\hat{f}_{\lambda}(X^*) - \hat{f}_{\lambda}(X^*)||^2 = \textbf{B} + \textbf{V}
\end{equation}
where the expectation is taken over the random variables $Y$ and $X^*$, where $X^*$ has the same distribution as the vectors of $\textbf{X}$. The decomposition of the risk into the terms $\textbf{B}+\textbf{V}$ is the well known \textit{Bias-Variance} decomposition with bias $\textbf{B}$ and variance $\textbf{V}$.





==> sections/old_sections/Section3.tex <==
\section{RKHS-Norm in High Dimensions}
\label{sec:norm}
The RKHS-norm $\lvert\lvert f^* \rvert\rvert_{\mathcal{H}}$ is an often used quantity for upper bounds on the infinity norm of $||f^* - \hat{f}_{\lambda}||_{L_{\infty}(\Omega)}$, which is itself an upper bound for the bias $\textbf{B}$ of the estimator. For an example we refer to \cite[Theorem~11.22]{Wendland04}. In fact, given that $d$ is constant, the bound from \cite[Theorem~11.22]{Wendland04} vanishes under additional assumptions on the ground truth $\hat{f}_{\lambda}^*$ and the distribution of $\mathbf{X}$ when $n \to \infty$. In contrast, this is usually wrong when $d(n) \to \infty$. The issue is that in order to achieve a that the bound in \cite[Theorem~11.22]{Wendland04} vanishes, the maximum fill distance of the data set $\textbf{X}$ must go to zero. Instead, \cite[Theorem~3]{Rakhlin19} derived a bound of the form 
$$ \textbf{B} \leq ||f^*||_{\mathcal{H}} ~C_1(\lambda_1(K),..., \lambda_n(K)) + C_2(n) $$
where $C_2(n) \to 0$ as $n \to \infty$ and $C_1(\lambda_1(K),..., \lambda_n(K))$ depends only on the eigenvalues of the empirical kernel matrix $K$. The advantage of this bound is that, under the assumption that $||f^*||_{\mathcal{H}}$ stays bounded by a constant for all $d(n)$, the bound vanishes whenever the Eigenvalues of $K$ decay sufficiently fast. In fact, in \cite[Example~4.3]{Rakhlin19}, we can see that this may even be the case when $\trace(\Sigma_d) \asymp n^{\beta}$ with $\beta >0$. \\
As a first result of this paper, we show that the assumption that $||f^*||_{\mathcal{H}}$ is bounded by some constant independently of $d(n)$ is generally not justified when $d(n) \to \infty$. As a result, we conclude that the dependency of $||f^*||_{\mathcal{H}}$ on $d$ must be taken into account when applying upper bounds on the bias of the form of \cite[Theorem~3]{Rakhlin19}.  \\
Unfortunately, the RKHS norm of commonly used kernels such as the Gaussian or the Laplacian kernel have very difficult expressions, especially when $\mathcal{X}$ is a compact domain. For instance, an expression for the Gaussian RKHS can be found in \cite[Theorem~4.22]{Steinwart08}. Instead,
in this paper, we give a simple example for a high dimensional RKHS where the RKHS norm of any sparse non constant function increases with $d$. The goal of this example is to highlight the dependency of RKHS norm on $d$. And in a next step, we empirically highlight the dependency on $d$ also for commonly used kernels such as the Gaussian and Laplacian kernels or the exponential inner product kernel studied in \cite{Rakhlin19}. 
\subsection{Example: Tensor Product Kernels}
 We construct a simple tensor product space RKHS with reproducing kernel $k$ of the form 
 \begin{equation}
     k:  [0,1]^d \times  [0,1]^d \to \mathbb{R}, (X,X') \to \left(\overset{d}{\tens{j = 1}} q^d \right)(X,X')
 \end{equation} 
 with $q^d : [0,1] \times [0,1] \to \mathbb{R}$,
$$ q^d(x,x') = \sum_{j=-\infty}^{\infty} q^d_j \exp\left(2\pi j i (x-x')\right) $$ 
where $i$ is the imaginary unit and $q^d_j \geq 0$ and $q^d_j = q^d_{-j}$. We remark that the conditions on $q^d_j$ are sufficient and necessary in order to guarantee that $q^d$ is a positive definite function. Furthermore, not that the coefficients $q_j^d$ explicitly depend on $d$. 
We refer to \cite[Proposition~12.31]{Wainwright19} for a proof of the fact that $k$ is again a positive definite kernel with induced inner product
$$\langle f,g\rangle_{k} = \prod_{j=1}^d \langle f_j,g_j\rangle_q $$
where $\langle f_j,g_j\rangle_q $ is the inner product induced by $q$ and  $f(X) = \prod_{j=1}^d f_j(X[j])$, where $X[j]$ is the $j$-th entry of the vector $X \in [0,1]^d$, and similar for $g$. We make the additional assumption that for all $x \in [0,1]$, $q(x,x) = 1$, which is equivalent to saying that for every $X \in [0,1]^d$, $k(X,X) = 1$. Hence, we require that $\sum_{i=-\infty}^{\infty}q_i = 1$. We can now show that for any choices of $q_i$ satisfying these assumptions, the RKHS norm of a sparse function goes to infinity as $d\to \infty$:
\begin{lemma}
\label{lm:rkhs}
Assume that $f$ is a non constant functions which has the form $f(X) = \prod_{j=1}^m f_j(X[j])$. Hence, $f$ is a sparse function depending only on the first $m$ dimensions. Then, for every sequence of coefficients $q_j^{d}$, 
$$ ||f||_{\mathcal{H}} := \sqrt{ \langle f,f\rangle_k}  \overset{d \to \infty}{\to} \infty $$
\end{lemma}
It is well known that the RKHS of the Guassian kernel is dense in $L_2(\mathcal{X})$ and thus is clearly much larger than the tensor product RKHS introduced in this sections. Nevertheless, we highlight that $\exp(-||X-X'||^{2}) = \prod_{i=1}^d\exp(-|X[i] - X'[i]|^2)$. Since the estimator of kernel ridge regression, given in Equation \ref{eq:kernelridge}, is only dependent on $k(X,X')$, we can see that the solution of kernel ridge regression with the Gaussian kernel results in the same estimator as when using the tensor product kernel with $q_d = \exp(-|X[i] - X'[i]|^2)$. Finally, because the solution of kernel ridge regression minimises Equation \ref{eq:krr}, we would expect both RKHS norms to behave similarly. 
\subsection{Experiments for RBF and Inner Product Kernels}
As we have already seen, the RKHS norm of any non constant function induced by the tensor product kernels defined in the last subsection growths to infinity with $d$ increasing. The purpose of this subsection is to empirically show that the phenomenon can also be observed for the popular Gaussian kernel $k(X,X') = \exp(-\tau ||X-X'||_2^2)$ and Laplace kernel $k(X,X') = \exp(-\sqrt{\tau} ||X-X'||_2)$. Furthermore, we can also observe this phenomenon also occurs for the exponential inner product kernel $k(X,X') = \exp(-\tau X^TX')$, studied in \cite{Rakhlin19}. We only study the case where $\tau = \frac{1}{d}$. This choice is commonly used in the literature \cite{ElKaroui10,Rakhlin19,Liu20,Ghorbani,Liang20b}. \\
Although the RKHS norm does often have not even a closed form solution, we remark that for any set of inputs $\textbf{X}$ and observations $Y$, we can compute the RKHS norm of the estimator $\hat{f}_{\lambda}$, which is given by 
\begin{equation}
    \lvert\lvert \hat{f}_{\lambda} \rvert\rvert_{\mathcal{H}} = Y^T (K +\lambda \textrm{I}_n)^{-1} K (K +\lambda \textrm{I}_n)^{-1} Y
\end{equation}
Choosing $\lambda = 0$ results in the case where $\hat{f}_{\lambda}$ interpolates the data and because $\hat{f}_{\lambda}$ is the solution of the minimisation problem from Equation \ref{eq:krr}, we know that $\hat{f}_{\lambda}$ is the function with minimum RKHS norm such that $f(X_i) = Y_i$. Hence, assuming that $Y_i = f^*(X_i)$ are noiseless observations, we get that $\lvert\lvert \hat{f}_0 \rvert\rvert_{\mathcal{H}} \leq \lvert\lvert \hat{f}^* \rvert\rvert_{\mathcal{H}}$.\\ As a result, Figure \ref{fig:rkhsnorm} shows that we can even observe diverging RKHS norms for the very simple function $f^*(X) = X[1]$. Furthermore, based on the previous discussion, we have that the estimates of the RKHS norms are simultaneously lower bounds. 
\\
\Comment{Conclusions are still missing..}
\begin{figure}
    \centering
    \includegraphics[height=4cm]{Plots/RKHSplot.png}
    \caption{RKHS Norm}{The first plot shows the the estimated RKHS norm of $f^*(X) = X[1]$. For the estimator, in total $7500$ input samples are drawn uniformly from $[0,1]^d$. Furthermore, the second plot shows the maximum distance of $\hat{f}_0$ and $f^*$ evaluated at $7500$ test samples drawn from the same distribution.}
    \label{fig:rkhsnorm}
\end{figure}

==> sections/old_sections/Section4.tex <==


\section{Main Result}
Assume that $\tau = \tau_0$ is some constant. Then, we can define $k'(X,X') = k(\tau_0 X,\tau_0 X')$ and instead analyse $k'_{\tau'}$ with $\tau' = 1$. Therefore, it is sufficient to distinct between the following three different choices of $\tau$:
\begin{center}
    \textbf{Case 1:} $\tau = 1 $, ~~~\textbf{Case 2:} $\tau \overset{n \to \infty}{\to} \infty$, ~~~ \textbf{Case 3:} $\tau \overset{n \to \infty}{\to} 0$\\
\end{center}
The main contribution of this paper is to study the first case where $\tau =1$ and therefore, $k_{\tau}(X,X') = k(X,X')$. We refer to the next section for a discussion for the other two cases. The advantage of this regime is that it allows a very general analysis of kernel methods due to the fact that, due to Lemma \ref{lm:innerpr}, the random variable $||\tau X_i||_2$ almost surely concentrates around $1$. Note that this stands in strong contrast with the other two cases, where $||\tau X_i||_2$ almost surely goes to zero respectively infinity. Besides, we highlight that this setting includes the one studied in the paper \cite{Liang20b}, where $d \asymp n^{\beta}$ and $k(X,X') = h(\frac{1}{d} X^TX')$. In addition, if $\trace(\Sigma_d) \asymp n$, this setting includes the ones studied in the papers \cite{ElKaroui10,Liang20,Liu20}. Finally, we remark that this regime is also relevant even if $\trace(\Sigma_d)$ is not known and $\textbf{Z}$ is assumed to be given as input data instead of $\textbf{X}$. In fact, let $\textbf{Z}$ and define $\hat{t} = \frac{1}{n} \sum_{i=1}^n Z_i^TZ_i$ be the estimator of $\trace(\Sigma_d)$. As a consequence of Lemma \ref{lm:consistent}, we can see that $\hat{c} = \frac{\sqrt{\trace(\Sigma_d)}}{\sqrt{\hat{t}}} \to 1 ~~a.s.$. 
\begin{remark}
Both \cite{Ghorbani,Ghorbani20} studied the regime where the input data is assumed to be uniformly distributed on a Hyper sphere, respectively uniformly distributed on the product of two Hyper spheres. However, we remark that any results directly imply corresponding results for the case where the input data $\textbf{S}$ is given with $S_i = X_i/\lvert\lvert X_i \rvert\rvert_2$. Note that this is a consequence of Lemma \ref{lm:innerpr}. As a consequence, we can partially extend the observations in \cite{Ghorbani,Ghorbani20} to to more general distributions on the sphere. We refer to the Appendix for a more detailed discussion on this topic. 
\end{remark}



\subsection{Assumptions}
It is well known from \cite{Schoenberg1988} that the restriction of a positive definite continuous rotational invariant kernel function $k$ on the hyper sphere $k|_{\mathcal{S}^{d-1} \times \mathcal{S}^{d-1}}(X,X')$ can be expressed in the form 
$$ k|_{\mathcal{S}^{d-1}\times \mathcal{S}^{d-1}}(X,X') = \sum_{j=0}^{\infty} c_j X^T X'$$
with constants $c_j$ in $\mathbb{R}$. Unfortunately, we are not aware of any extensions to the general case where $X \in \mathbb{R}^d$. However, note that due to Lemma \ref{lm:innerpr}, the data set $\textbf{X}$ closely concentrates around the unit Hyper Sphere. Furthermore, Corollary \ref{cr:testsample} shows that this is also the case for test samples $X^*$ drawn from the same distribution as $\textbf{X}$. Hence, it is sufficient to make regularity assumptions on $k$ in a neighbourhood of the unit Sphere. \\
Let $\delta \in (0,1)$ be some constant and define the compact set
\begin{equation}
\label{eq:omega}
\begin{split}
        \Omega := \lbrace ~ \{1+x\}\times \{1+y\} \times [-\sqrt{(1+x)(1+y)}, \sqrt{(1+x)(1+y)}]| x,y \in [-\delta, \delta] ~\rbrace \\
    \subset [1-\delta, 1+\delta]^2\times [-1-\delta, 1+\delta]
\end{split}
\end{equation}
\begin{remark}
\label{rm:remarkcont}
$\Omega$ is chosen such that for any $(x,y,z) \in\Omega$ and any $d(n)>1$, we can choose $X,X' \in \mathbb{R}^{d}$ such that $||X||_2^2 = x$, $||X'||_2^2 = y$ and $X^TX' = z$. This specific definition is necessary to have RBF kernels as a special case of our analysis. 
\end{remark}
Let $g: \Omega \to \mathbb{R}$ be some continuous function of the form
\begin{equation}
\label{eq:g}
g(x,y,z) = \sum_{i=0}^{\infty} z^i g_i(x,y)
\end{equation} 
with $g_i : [1-\delta, 1+\delta]^2 \to \mathbb{R}$, satisfying the following assumption. 
\begin{assumption} 
\label{ass:1}
\begin{enumerate}
    \item The restriction of $g$ on $\{(x,x,x)| x\in [1-\delta, 1+\delta]\} \subset \Omega$ is a Lipschitz continuous function.  
    \item Let $p = \floor{2/\beta}$. For any $i \leq p+1$, $g_i$ is $(p+1-i)$-times continuously differentiable on a closed ball of non zero radius around the point $(1,1)$.
\end{enumerate} 
\end{assumption}
We can now make the following regularity assumption on the kernel function $k$
\begin{assumption}
\label{ass:kernel}
There exists some $\delta >0$ and a function $g$ which satisfies Assumption \ref{ass:1}, such that for any $n$ and any $X,X' \in \mathbb{R}^{d(n)}$ with $(||X||_2^2, ||X'||_2^2)\in [1-\delta, 1+\delta]^2$,
\begin{equation}
    \label{eq:kernel}
    k(X,X') = g(||X||_2^2, ||X'||_2^2, X^T X')
\end{equation}
\end{assumption}
\begin{remark}
\label{rm:kalmostsureg}
For any $\delta>0$, we can choose $n$ sufficiently large such that $n^{-\beta/2} \log(n)^{1+\epsilon} \leq \delta$. Therefore, due to Lemma \ref{lm:innerpr},
\begin{equation}
    k(X_i,X_j) = g(||X_i||_2^2, ||X_j||_2^2, X_i^T X_j) ~~~~a.s
\end{equation}
\end{remark}
We highlight that Assumption \ref{ass:kernel} holds true for a very broad range of kernels. For example, any inner product kernel of the form $k(X,X') = \sum_{i=0}^{\infty} g_i (X^TX')^i $ satisfies the assumptions. The only non trivial point to show is that the the Lipschitz continuity from Assumption \ref{ass:1} holds true. For this, note that because $k$ exists for every $X,X' \in \mathbb{R}^d$, we can conclude that the power series $\sum_{i=0}^{\infty} g_i x^i$ converges absolutely for every $x \in \mathbb{R}$ and therefore also the derivative of it $\sum_{i=0}^{\infty}  g_{i+1} i! x^i$. Hence, we can conclude that the first point form Assumption \ref{ass:1} holds true. \\
Another example are the Neural Tangent Kernels \cite{Arora19,Jacot20} under weak additional assumptions on the activation function $\sigma$. In fact, as shown \ref{lm:ntk1}, this is the for the Relu-NTK of any depth and with activation $\sigma(x) = \max(0,x)$. Another example are RBF kernels of the form $k(X,X') = h(||X-X'||_2^2)$, given that $h$ is locally analytic around $2$ with Taylor series expansion converging at $0$. In order to see this, note that these assumptions imply that there exists $\delta >0$, such that for any $X,X' \in \mathbb{R}^{d(n)}$ with $||X||_2^2, ||X'||_2^2 \in [1-\delta, 1+\delta]$,
\begin{equation}
    k(X,X') = h(||X-X'||_2^2) = \sum_{i = 0}^{\infty} \frac{2^i h^i(2) }{i!} \left[(||X||_2^2-1) + (||X'||_2^2-1) -2X^TX' \right]^i
\end{equation}
Assumption \ref{ass:kernel} follows then trivially. We remark that the assumptions on $h$ are satisfied by many well known RBF kernels such as the Matern-RBF as described in \cite[Chapter~4]{Rasmussen03} kernels or the $\alpha$-Exponential RBF kernels of the form $h(x) = \exp(-\tau_0 x^{\alpha})$ with $\alpha \in (0,2]$. Finally, we remark that, in order to satisfy Assumption \ref{ass:kernel}, the kernel function $k$ does not necessarily have to be positive definite. For instance, the kernel $k(X,X') = \lvert\lvert X - X' \rvert\rvert_2^{\alpha}$ satisfies the assumptions as well for any $\alpha > -1$. 







\subsection{Minimum Eigenvalue of Kernel Matrix}
\label{sec:lowerboundofEV}
Before stating the main results of this paper, presented in the next subsection, we highlight an the important phenomenon that the Eigenvalues of the kernel matrix $K$ stay lower bounded by a positive constant independent of $n$. This observation is not novel and can also be made from \cite[Theorem~2.1\&2.2]{ElKaroui10} if $d \asymp \trace(\Sigma_d) \asymp n$ and the kernel $k$ is an inner product or RBF kernel. The contributions of this section are two folds. On the one hand, we extend the result to more general kernels including the NTK kernels, and on the other hand, we show that this phenomenon also occurs in the more general case where $\trace(\Sigma_d) \asymp n^{\beta}$ with $\beta \in (0,1]$. 
\begin{remark}
Note that the Eigenvalues of $K$ go to zero in \cite[Theorem~2.1\&2.2]{ElKaroui10} when choosing $\trace(\Sigma_d)/d \to 0$. This does not contradict our result since the choice of the scale parameter in \cite[Theorem~2.1\&2.2]{ElKaroui10} does only correspond to our setting when $\trace(\Sigma_d) \asymp d$. 
\end{remark}
We remark that this phenomenon of lower bounded Eigenvalues stands in strong contrast to classical regimes where $d$ is assumed to be constant. In fact, for these regimes, there exists many results connecting decay of the Eigenvalues of the kernel matrix $K$ with the Eigenvalue decay of the operator $\mathcal{T}: L^2_{\mu}(\mathcal{X}) \to L^2_{\mu}(\mathcal{X}), g \to \int_{\mathcal{X}} k(x,y) g(y) d\mu $. For instance, we refer to \cite[Theorem~2]{Belkin18a}, which shows that the Eigenvalues of the kernel matrix of the Gaussian kernel decay exponentially. \\
In order to lower bound the Eigenvalues, we require an asymptotic description of $K$, given in Proposition \ref{prop:elkarouiextension}. This result is inspired by \cite[Theorem~2.1\&2.2]{ElKaroui10}. Let, $\circ i$ denote the $i$-times Hadamard product and for any $ j\leq p+1,$ $ \alpha = (i_1,i_2)$, let $g_j^{(\mathbf{\alpha})}$ denote the partial derivatives $g_j^{(\mathbf{\alpha})}(x,y) = \frac{\partial^{|\alpha|}}{\partial t_1^{i_1} t_2^{i_2}} g_j(t_1,t_2)|_{x,y}$. Furthermore, let $\psi$ be the vector with entries $\psi_i = ||X_i||_2^2 - 1$. Then, 
\begin{prop}
\label{prop:elkarouiextension}
Given that Assumption \ref{ass:kernel} holds true, we have that
\begin{equation}
    ||K- M||_2 \to 0 ~~~ a.s.
\end{equation}  
with
\begin{equation}
\label{eq:elkarouiM}
\begin{split}
    M &= \textbf{I}_n\left(g(1,1,1)  - \sum_{i =0}^p g_i(1,1) \right) +  \sum_{i=0}^p (\textbf{X}^T\textbf{X})^{\circ i} \circ \left[
\sum_{m =0}^{p-i} \sum_{k = 0}^{m}  \frac{g_{i}^{(k,m-k)}(1,1)}{k!(m-k)!} \psi^{\circ k} (\psi^{\circ (m-k)})^T \right]
\end{split}
\end{equation}
\end{prop}
Proposition \ref{prop:elkarouiextension} provides an asymptotic description of the kernel matrix $K$ for a very broad class of kernel functions. We remark that the kernel function $k$ only needs to satisfy Assumption \ref{ass:kernel} but does not necessarily have to be positive definite. However, we are actually interested in order to obtain an asymptotic description of Equation \ref{eq:kernelridge}, we require that the Eigenvalues of $(\lambda \textbf{I}_n + K )$ do asymptotically not go to zero. Clearly, whenever $k$ is positive definite and $\lambda >0$ is constant, Proposition \ref{prop:elkarouiextension} implies that
\begin{equation}
\label{eq:lowerboundev}
     || (\lambda \textbf{I}_n + K )^{-1} - (\lambda \textbf{I}_n + M)^{-1}||_2 \to 0. 
\end{equation}
 For the choice $\lambda = 0$, this equation is only guaranteed if we can show that the minimum Eigenvalue of $K$, $\lambda_{min}(K)$ is asymptotically lower bounded by a positive nonzero constant $\lambda_{min}(K) \geq c_{\lambda_{min}}>0$ which is independent of $n$. Note that due to Proposition \ref{prop:elkarouiextension}, this statement is equivalent to showing that the Eigenvalues of $M$ are lower bounded. As a consequence, we obtain the following corollary of Proposition \ref{prop:elkarouiextension}. 
\begin{cor}
\label{cr:posdef}
Assume that for any $j$, $g_j$ is a positive definite function. In addition, assume that there exist $j \geq p+1$ such that $g_j(1,1) > 0$. Then, there exists some positive non zero constant $c_{\lambda_{min}}$ such that
\begin{equation}
\label{eq:lambdamin}
    \lambda_{min}(K) \geq c_{\lambda_{min}} >0 ~~~a.s.
\end{equation}
\end{cor}
First of all, note that when $k(X,X') = h(X^TX')$ is an inner product, the functions $g_i$ are all necessarily constants. Thus, the assumptions from Corollary \ref{cr:posdef} hold true for inner product kernels if $g_i \geq 0$ and if there exists $j \geq p+1$ such that $g_j >0$. These assumptions are analogous to the assumptions made on the kernel $k$ in \cite{Ghorbani20,Liang20b}. However, we highlight that Corollary \ref{cr:posdef} applies to a much broader class of kernel functions. For instance, we can show that Corollary \ref{cr:posdef} applies to the Relu-NTK \cite{Jacot20,Arora19} of any depth $L>0$. We refer to Corollary \ref{cr:ntk2} in the Appendix for a proof of this fact. Another example is the Gaussian kernel with constant scale parameter $\tau_0 > 0$, which can be seen when writing
\begin{equation}
    \exp(-\tau_0 ||X-X'||_2^2) =  \sum_{j=0}^{\infty} \frac{1}{j!} (X^TX')^j \left(\tau_0^j \exp(-\tau_0||X||_2^2)\exp(-\tau_0 ||X'||_2^2) \right), 
\end{equation}
and because $\tau_0^j \exp(-\tau_0||X||_2^2)\exp(-\tau_0 ||X'||_2^2) > 0$ is a positive definite kernel function. \\

Unfortunately, verifying that the assumptions in Corollary \ref{cr:posdef} holds true for more general RBF kernel functions is not trivial. Nevertheless, we can show that the phenomenon of lower bounded Eigenvalues of the kernel matrix applies also to the $\alpha$-exponential kernels:
\begin{lemma}
\label{lm:alphaexp}
Let $\alpha \in (0,2)$ and $\tau_0$ be some constant. Then, for the $\alpha$-Exponential kernel $k(X,X') = \exp(-\tau_0 ||X-X'||^{\alpha})$, the corresponding kernel matrix satisfies Equation \ref{eq:lambdamin} with $c_{\lambda_{min}}$ some non zero positive  constant.
\end{lemma}






\subsection{Lower Bound of the Bias}
\label{sec:biasbound}
We are now able to state the main result of this paper. For any $n$, let $X^* \in \mathbb{R}^{d(n)}$ be a random vector sampled from the same distribution as $\textbf{X}$. Furthermore, for any $\epsilon>0$, let $\mathcal{U}$ be the set of 
\begin{equation}
    \mathcal{U} = \left\{ X^* | \left|~||X^*||_2^2-1\right|  \leq n^-{\beta} \log(n)^{1+\epsilon}, ~ \max_{i} |X_i^T X^* |   \leq n^-{\beta} \log(n)^{1+\epsilon} \right\}.
\end{equation}
We know from Corollary \ref{cr:testsample} that for any $\epsilon>0$, there exists $C >0$, such that for $n$ sufficiently large, $\mathcal{U}$ has measure $P(\mathcal{U}) \geq 1 - n^2 \exp(-C \log(n)^{1+\epsilon}) \to 1$. Let $\psi^*$ be the vector with entries $\psi^*_i = ||X^*||_2^2 -1$. Then, 
\begin{theorem}
\label{th:main}
Assume that the minimum Eigenvalue of $(\lambda \textrm{I}_n + K)^{-1}$ is almost surely lower bounded by a non zero positive constant independent of $n$. Then, 
\begin{equation}
    \underset{X^* \in \mathcal{U}}{\max} ~ \lvert\lvert (\lambda \textrm{I}_n + K)^{-1} K^*  - (\lambda \textrm{I}_n + M)^{-1} M^*\rvert\rvert_1 \to 0 ~~~ a.s.
\end{equation} 
with $M$ from Proposition \ref{prop:elkarouiextension} and
\begin{equation}
    \label{eq:Mstar} 
     M^* =\sum_{i=0}^p (\textbf{X}^TX^*)^{\circ i} \circ \left[
\sum_{m =0}^{p-i} \sum_{k = 0}^{m}  \frac{g_{i}^{(k,m-k)}(1,1)}{k!(m-k)!} \psi^{\circ k}\circ (\psi^*)^{\circ (m-k)} \right]
\end{equation}
with $p = \floor{2/\beta}$.
\end{theorem}
Interestingly, $M^*$ depends on $X^*$ only by polynomials of $((X^*)^TX^*)^{p_1}(X_i^TX^*)^{p_2}$ with $p_1 + p_2 \leq p$. Hence, assuming that the entries of $Y$ are almost surely bounded by some constant independent of $n$, we have
\begin{equation}
    \underset{X^* \in  \mathcal{U}}{\max} |\hat{f}_{\lambda}(X^*)- Y^T(M + \lambda I_n)^{-1} M^*| \to 0 ~~a.s.. 
\end{equation}
Because $P(\mathcal{U}) \to 1$, we find that $\hat{f}_{\lambda}(X^*)$ looks asymptotically almost surely for almost all $X^*$ like a polynomial of degree at most $2p$. Unfortunately, the assumption that the entries of $Y$ are bounded by some constant is not satisfied for the important case where the observations are generated by adding an i.i.d. Gaussian noise term to the ground truth, i.e. $Y_i = f^*(X_i) + \epsilon_i$ and $\epsilon_i ~ \mathcal{N}(0, \sigma_{\epsilon}^2)$. However, recall that the Bias term is given by
\begin{equation}
    \mathbb{E}_{X^*} || \mathbb{E}_{Y}\hat{f}_{\lambda}(X^*) - f^*(X^*) ||^2 = \mathbb{E}_{X^*} || f^*(\textbf{X})^T (K + \lambda \textrm{I}_n)^{-1} K^* - f^*(X^*)||^2
\end{equation}
where $f^*(\textbf{X})$ is the vector with entries $f^*(\textbf{X})_{i} = f^*(X_i)$. As a result, we can see that the Bias term is only dependent on the mean of the observations $f^*$, which is much less restrictive to assume to be bounded. In fact, given that $f^*$ is a bounded function, Theorem \ref{th:main} implies that
\begin{equation}
    \underset{X^* \in  \mathcal{U}}{\max} |\mathbb{E}_{Y}\hat{f}_{\lambda}(X^*) - f^*(\textbf{X})^T(M + \lambda I_n)^{-1} M^*| \to 0 ~~a.s.
\end{equation}
This fact can now be used to lower bound the Bias. Let $\overline{P}_{l}(f^*)$ be the projection of $f^*$ onto the space of truncated polynomials of degree at most $l$, where the projection is such that
\begin{equation}
    \overline{P}_{l,C}(f^*) = \underset{p_l \in \overline{\mathcal{P}}_{l,C}}{\arg\min} \left[ \mathbb{E}_{X^*} \left( f^*(X^*) - \overline{p}_l(X^*)\right)^2 \right]
\end{equation}
with 
\begin{equation}
    \overline{\mathcal{P}}_{l,C} = \left\{\min \left(C, \sum_{j=0}^l\sum_{i=1}^{d} c_{j,i} X[i]^j\right)  \lvert c_{j,i} \in \mathbb{R}  \right\}
\end{equation} the space of truncated polynomials of degree at most $l$ and truncation parameter $C>0$. As a direct consequence of Theorem \ref{th:main} and the subsequent discussion, we obtain the following lower bound on the Bias term. 
\begin{cor}
\label{cr:biaslimit}
Assume that Theorem \ref{th:main} applies. Then, for any constant $C \geq \underset{d}{\sup}~ \lvert\lvert f^* \rvert\rvert_{\infty}$, any $\gamma>0$ and any $n$ sufficiently large,
\begin{equation}
    \textbf{B} - \gamma \geq \mathbb{E}_{X^*} \left[ f^*(X^*) - \overline{P}_{l,C}(f^*)\right]^2 ~~~ a.s.
\end{equation} 
with $l = 2p = 2 \floor{2/\beta}$.
\end{cor}
Note that this bound is clearly not thigh, however, the main purpose of this paper is to highlight that the Bias cannot vanish for sufficiently non linear ground truth functions $f^*$.

\Comment{Most important part is missing; the discussion of the results...}

==> sections/old_sections/Section5.tex <==
\section{Results for other Choices of $\tau$}
\label{sec:additionalresults}
The question which is now whether the lower bound of the Bias shown in Corollary \ref{cr:biaslimit} can be overcome when $\tau \to 0$ respectively $\tau \to \infty$. In fact, such settings occur for example in \cite{el2010spectrum,Rakhlin19,Liu20} when $\frac{\trace(\Sigma_d)}{d} \to 0$. Let $\tilde{X}_i = \tau X_i$. As a consequence of Lemma \ref{lm:innerpr}, we can see that $||\tilde{X}_i||_2^2 \to 0~~a.s.$ if $\tau \to 0$ and $||\tilde{X}_i||_2^2 \to \infty~~a.s.$ if $\tau \to \infty$. Thus, the behaviour of $\hat{f}$ is determined by the behaviour of the kernel function $k_{\tau}(X_i,X_j) = k(\tilde{X}_i, \tilde{X}_j)$ when $\tilde{X}_i,\tilde{X}_j$ approaches zero respectively infinity. Unlike the first case where $\tau = 1$, this behaviour can significantly differ among the distinct choices of $k$. For an example, compare the kernel functions $\exp(-||X-X'||_2^2)$ and $\exp(X^TX')$. \\
In this paper, we only study the special case where $k(X,X') = \exp(-||X-X'||^{\alpha})$ with $\alpha \in (0,2]$. For these kernel functions, we give two examples where $\tau \to 0$ respectively $\tau \to \infty$ and show that in both cases the lower bound from Corollary \ref{cr:biaslimit} still holds true. Although our analysis is restricted to two special examples, it clearly demonstrates that the issue of an non vanishing Bias does not only occur due to a bad choice of $\tau$. 
\subsection{Case 2: $\tau \to \infty$}
We know from Lemma \ref{lm:innerpr} that $||X_i - X_j||_2^2$ concentrate around $2 (1-\delta_{i,j})$. Therefore, we can see that when $\tau \to \infty$, $k_{\tau}(X_i,X_j) = \exp(-\tau||X_i - X_j||) \to \delta_{i,j}~~a.s.$. In fact, assuming that $\tau = n^{\theta}$ with $\theta >0$, we can see that 
\begin{equation}
    || K - \textrm{I}_n ||_2 \leq n ~ \max_{i \neq j} | \exp(-n^{\theta}||X_i - X_j||)| \to 0 ,
\end{equation}
and hence, for every $X^*$ such that $\underset{i}{\max}~\lvert\lvert X_i - X^*\lvert\lvert_2^2 \geq c >0$ with $c$ some positive constant independent of $n$ and any $\lambda \geq 0$,
\begin{equation}
    ||(K+\lambda \textrm{I}_n)^{-1} K^*||_1 \lesssim n ~ \max_{i} | \exp(-n^{\theta} c )| \to 0 . 
\end{equation}
Clearly, we can choose $c$ such that any $X^*$ satisfies the assumption that $\underset{i}{\max}\lvert\lvert X_i - X^*\lvert\lvert_2^2 \geq c >0$. Following the same reasoning as subsequent to Theorem \ref{th:main}, we can see that for any bounded set of observations $Y$, the estimator $\hat{f}$ looks almost everywhere asymptotically like the null estimator. Following again the same argumentation as in the proof of Corollary \ref{cr:biaslimit}, we get:
\begin{lemma}
\label{lm:biastautoinfty}
Assume that $k(X,X') = \exp(-||X-X'||^{\alpha})$, with $\alpha \in (0,2]$, and assume that $\tau = n^{\theta}$ with $\theta >0$. Then, for any $\gamma>0$,
\begin{equation}
    \textbf{B} - \gamma \geq \mathbb{E}_{X^*} f^*(X^*)^2 ~~~ a.s..
\end{equation} 
\end{lemma}
As a result, we note that this bound on the Bias is significantly stronger than Corollary \ref{cr:biaslimit}. 

\subsection{Case 3: $\tau \to 0$}
First of all, note that when assuming that $\tau = O(n^{-1})$, we can apply Lemma \ref{lm:innerpr} to show that
\begin{equation}
\label{eq:case3eqmat}
    || K - 11^T ||_2 \lesssim n ~ \max_{i \neq j} | \exp(-\frac{1}{n} ||X_i - X_j||) -1| \to 0 .
\end{equation}
As a result, we observe that the kernel matrix $K$ converges asymptotically to the rank one matrix $11^T$. We remark that such a phenomenon can also be observed in \cite[Theorem~2.1\&.2.2]{el2010spectrum} when $\trace(\Sigma_d)/d \to 0$. 
As a consequence, we observe that the Eigenvalues of $K^{-1}$ diverge as $n \to \infty$. We separate our analysis into the case where the ridge parameter $\lambda >0$ is some non zero constant and into the case where $\lambda = 0$. \\\\

\textbf{Non Zero Ridge Parameter $\lambda > 0$: } First the case where $\lambda > 0$. Trivially, the Eigenvalues of $(K +\lambda \textrm{I}_n)^{-1}$ are upper bounded by the constant $\frac{1}{\lambda}$. Thus, for every $X^*$ such that $\underset{i}{\max}~\lvert\lvert X_i - X^*\lvert\lvert_2^2 \leq c0$ with $c$ some positive constant independent of $n$,
\begin{equation}
    ||(K+\lambda \textrm{I}_n)^{-1} K^* - (11^T+\lambda \textrm{I}_n)^{-1} 1||_1 \lesssim n ~ \max_{i} | \exp(-n^{-1} c) -1| \to 0 . 
\end{equation}
where we have used that a similar result to Equation \ref{eq:case3eqmat} holds true for $K^*$. Following the same discussion as in the previous subsection, we can show that
\begin{lemma}
\label{lm:biastauto0}
Assume that $k(X,X') = \exp(-||X-X'||^{\alpha})$, with $\alpha \in (0,2]$, and assume that $\tau = O(n^{-1})$. Then, for any $\gamma>0$,
\begin{equation}
    \textbf{B} - \gamma \geq \mathbb{E}_{X^*} f^*(X^*)^2 ~~~ a.s..
\end{equation} 
\end{lemma}

\textbf{Zero Ridge Parameter $\lambda  =0$: } 
Surprisingly, the estimator $\hat{f}$ behaves substantially different in the case where $\lambda=0$. In fact, although the Eigenvalue of $K^{-1}$ diverge, we can still observe that $K^{-1}K^*$ remains stable, making this case significantly more difficult to analyse. In this subsection, we only analyse the extreme case where we obtain the flat limit solution. For any fixed $n,d$, the flat limit interpolator is defined  to be the interpolator $\hat{f}_{\textrm{fl}}$ obtained when taking the limit $\tau \to 0$: 
\begin{equation}
    \hat{f}_{\textrm{fl}}(X^*) = \lim_{\tau \to 0} \hat{f}(X^*) = \lim_{\tau \to 0} Y^T  K^{-1} K^*.
\end{equation}
In this section, we focus again on the case where  $k(X,X') = \exp(-\tau ||X-X'||^{\alpha})$, however, we restrict to $\alpha \in (0,2)$. Although the limit of $\lim_{\tau \to 0} K^{-1}$ does not exists, we can apply \cite[Theorem~3.12]{Lee2014} and \cite[Theorem~2.1]{Blumenthal60} to show that $\hat{f}_{\textrm{fl}}$ exists and has the form
\begin{equation}
    \hat{f}_{\textrm{fl}}(X^*) = \begin{pmatrix}Y \\ 0 \end{pmatrix} \begin{pmatrix} -D^{\alpha} & 1 \\ 1^T & 0 \end{pmatrix}^{-1} \begin{pmatrix} v^* \\ 1 \end{pmatrix},
\end{equation}
with $D^{\alpha}$ the $n\times n$ matrix with entries $D^{\alpha}_{i,j} = ||X_i-X_j||^{\alpha}$ and $v^*$ the vector with entries $v^*_i = ||X_i - X^*||^{\alpha}$. 
\begin{remark}
We remark that $D^{\alpha}$ is only almost surely invertible with respect to the draws of $\textbf{X}$, if $\alpha \in (0,2)$. On the other hand, when $d>n+1$, one can show that $D^2$ is singular for any choices of $\textbf{X}$. This is essentially the reason why the analysis in this section cannot be extended to the case where $\alpha = 2$. 
\end{remark}
\begin{remark}
The interpolator $\hat{f}_{\textrm{fl}}$ is called the \textit{Polyharmonic Spline} interpolator. In fact, \cite[Theorem~3.12]{Lee2014} applies to very general kernel functions. More detailed, we can see that the flat limit solution of any kernel of the form $k(X,X') = \phi(\lvert\lvert X-X' \rvert\rvert_2^2)$ with generalised Fourier transform asymptotically decaying at rate $x^{-d-\nu}$ is exactly the polyharmonic spline interpolator with $\alpha = \nu$. An other example is for instance the flat limit solution of the Matern RBF kernel with parameter $\nu \leq 2$. We refer to \cite[Chapter~4]{Rasmussen03} for a definition. 
\end{remark}
Interestingly, we can show a very similar result to Theorem \ref{th:main} holds true for the interpolator $\hat{f}_{\textrm{fl}}$. We refer to Theorem \ref{th:flatlimit} in the Appendix for an explicit statement of Theorem. Next, let $\textbf{B}_{\textrm{fl}}$ be the Bias term of the estimator $\hat{f}_{\textrm{fl}}$. Finally, we note that similarly to Theorem \ref{th:main}, as a consequence of Theorem \ref{th:flatlimit} we can show the following lower bound on the Bias of $\hat{f}_{\textrm{fl}}$:
\begin{cor}
\label{cr:biasflatlimit}
Assume that $\alpha \in (0,2)$. Then, for any $\gamma>0$ and any $n$ sufficiently large,
\begin{equation}
    \textbf{B}_{\textrm{fl}} - \gamma \geq \mathbb{E}_{X^*} \left[ f^*(X^*) - \overline{P}_{l,C}(f^*)\right]^2 ~~~ a.s.
\end{equation} 
with $l = 2p = 2 \floor{2/\beta}$.
\end{cor}









==> sections/old_sections/Section6.tex <==
\section{Experiments}
We now describe some numerical experiments that provide illustrative confirmations of the lower bound on the bias depending increasing with the parameter $\beta$. We study the following two different input data models:
\begin{itemize}
    \item \textbf{Model 1:} $\tilde{Z}_i[k] \sim \mathcal{N}(0,1)$; $d = \floor{n^{\beta}}$; $\Sigma_d = \textrm{I}_d$.
    \item \textbf{Model 2:} $\tilde{Z}_i[k] \sim \textrm{Uniform}(-C_U,C_U)$; $d = n$; $\Sigma_d$ is the diagonal matrix with entries $\Sigma_{d,i,i} = \lambda_i = (1 - ((i-1)/d)^{\kappa})^{1/\kappa}$ and $\kappa \geq 0$ such that $\trace(\Sigma_d) = \sum_{i=1}^n \lambda_i = n^{\beta}$.
\end{itemize}
We choose $C_U$ such that the variance of the random variable $Z_i[k]$ is one. Finally, for both models, we generate the input data $Z_i = \Sigma_d^{1/2} \tilde{Z}_i$ and normalise them to $X_i = \frac{1}{\sqrt{\trace(\Sigma_d)}}$. 
 We remark that the first model corresponds to the regimes studied in \cite{Liang20b} the second to the regimes studied in \cite{Rakhlin19}. For our analysis, we use the $\alpha$-exponential kernels of the form $k(X,X') = \exp\left(- \tau^{\alpha/2} \lvert\lvert X-X' \rvert\rvert_2^{\alpha} \right)$, and the exponential inner product kernel of the form $k(X,X') = \exp\left(\tau X^TX'\right)$. Furthermore, the ridge parameter $\lambda$ is well known to regulate the Bias-Variance trade off of the estimator $\hat{f}_{\lambda}$. Since we are primarily interested in the Bias term of the estimator, we only make experiments for the case where "ridge-less" case where $\lambda = 0$. 
 
 \subsection{Experiment 1}
 
 \begin{figure}
     \centering
     \minipage{0.24\textwidth}
  \includegraphics[width=\linewidth]{Plots/Breakpoint2_mdl1.png}
\endminipage\hfill
     \minipage{0.24\textwidth}
  \includegraphics[width=\linewidth]{Plots/Breakpoint2_mdl2.png}
\endminipage\hfill
     \minipage{0.24\textwidth}
  \includegraphics[width=\linewidth]{Plots/Breakpoint_mdl1.png}
\endminipage\hfill
     \minipage{0.24\textwidth}
  \includegraphics[width=\linewidth]{Plots/Breakpoint_mdl2.png}
\endminipage\hfill
\caption{ Bias with respect to $\beta$}{ The first two plots show the bias of $f^*_1$ for the first and second model and the other two figures show the same for the ground truth function $f^*_2$. In total $5000$ input data points are used for training and $25000$ for testing.}
\label{fig:exp1_p1}

 \end{figure}
 
 
 In a first experiment, we illustrate the Bias with respect to the parameter $\beta$ for the two sparse ground truth functions $f_1^*(X) = 2 Z[1]^2 = 2 \trace(\Sigma_d) X[1]^2 $ and $f_2^*(X) = 2 Z[1]^3 = 2 \trace(\Sigma_d)^{3/2} X[1]^3 $. Because the estimator $\hat{f}_{\lambda}$ depends only only linearly on the observations $Y$ ( recall Equation \ref{eq:kernelridge}, we can estimate the Bias term by computing the risk when using noise less observations for training, i.e. $Y_i = f^*(X_i)$. Figure \ref{fig:exp1_p1} shows the estimated bias for both models with respect to $\beta$. We can clearly observe for both input data sets, that the bias increases with respect to $\beta$. In particular, we observe that this happens similarly for all kernels, underlining the observation from our theoretical results that the lower bound of the Bias is independent of properties such as the Eigenvalue decay of the kernels. Finally, Corollary \ref{cr:biaslimit} separates the bias into different regimes of $\beta$. We can also make this observation in Figure \ref{fig:exp1_p1} when comparing the plots for $f^*_1$ and $f^*_2$. 
 \Comment{Missing: Make bridge to Linear Regression, i.e. the bias can not be overcome by making $\Sigma$ more spiky/less spiky. }
 
 \subsection{Experiment 2}
 The second experiment illustrates the dependency of the bias on $\tau$. \\
\Comment{Conclusion: Gaussian potentially diverges, for Laplacian, we can see that minimum bias is reached at $\tau -> 0$ (i.e. Flat limit)}
 
 
  \begin{figure}
     \centering
     \minipage{0.49\textwidth}
          \centering
  \includegraphics[height=4cm]{Plots/Tau_mdl1.png}
  \label{fig:awesome_image1}
\endminipage\hfill
     \minipage{0.49\textwidth}
          \centering
  \includegraphics[height=4cm]{Plots/Tau_mdl2.png}
\endminipage\hfill
\caption{Dependency of the bias on $\tau$}{ The bias is plotted with respect to $\tau$ for different choices of $\beta$ and for the Laplacian ($\alpha = 1$) and Gaussian ($\alpha =2$) kernels. 
The first plot shows the case where the data is generated from the first model and the second from the second model. In total $5000$ input data points are used for training and $25000$ for testing. In addition, we perform $100$ iterations each to estimate bias. The variance is then computed by taking the difference of the mean of the risk and the bias. The ground truth function is $f^*_3$.}
\label{fig:exp2}
 \end{figure}
 
 
 
\subsection{Experiment 3}
For this experiment, we generate the observations from $Y_i = f_2^*(X_i) + \epsilon_i$, with $\epsilon_i \sim \textrm{Uniform}(-10,10)$. Figure \ref{fig:exp2} shows the Bias-Variance decomposition of the risk.  
 \Comment{As a last experiment, we are interested in studying the Bias-Variance decomposition. => Future research, study dependency of variance on structure of Sigma. Here, we can mention Rakhlin and make the point that his bounds on the variance diverges when $\trace(\Sigma_d) /d \to 0$. }
 \begin{figure}
     \centering
     \minipage{0.49\textwidth}
          \centering
  \includegraphics[height=4cm]{Plots/Breakpoint_mse.png}
  \label{fig:awesome_image1}
\endminipage\hfill
     \minipage{0.49\textwidth}
          \centering
  \includegraphics[height=4cm]{Plots/Breakpoint2_mse.png}
\endminipage\hfill
\caption{Bias-Variance decomposition of risk with respect to $\beta$}{ The risk, bias and variance are plotted for the case where $\alpha=1$. The first plot shows the case where the data is generated from the first model and the second from the second model. In total $5000$ input data points are used for training and $25000$ for testing. In addition, we perform $100$ iterations each to estimate bias. The variance is then computed by taking the difference of the mean of the risk and the bias.}
\label{fig:exp2}
 \end{figure}
 \subsection{Experiment 4}
 Real world experiment.

==> sections/old_sections/outline_proof.tex <==

\subsection{Outline of the Proof}
\label{sec:outlineofproof}
\Comment{Needs to be updated again due to changes} \newline
In essence, both Corollary \ref{cr:EVlowerbound} and \ref{th:main_text} are a consequence of the concentration of Lipschitz continuous functions of i.i.d random vectors. For brevity of the notation, we write $\z = \tau \x$. As a result of our choice of the scale parameter, we can show that the rescaled samples $\z_i$ concentrate around the unit hyper sphere
implying Lemma \ref{lm:innerpr}. 
\begin{lemma}[Consequence of Lemma A.2 \cite{el2010spectrum}]
For any $\epsilon > 0$,
\label{lm:innerpr}
\begin{equation}
\label{eq:innerpreq}
    \max_{i,j }\left| \z_i^T \z_j- \delta_{i, j}\right| \leq n^{-\beta/2}log(n)^{1+\epsilon} ~~~ a.s.
\end{equation}
and
\begin{equation}
    \max_{i,j }\left|\lvert \lvert \z_i -  \z_j\rvert\rvert_2^2- 2(1-\delta_{i, j})\right| \leq n^{-\beta/2}log(n)^{1+\epsilon} ~~~ a.s..
\end{equation}
\end{lemma}
As a result, we can see that 
\begin{equation}
    k_{\tau}(\x_i,\x_j) = k(\z_i,\z_j) = g(\lvert\lvert \z_i \rvert\rvert_2^2, \lvert\lvert \z_j \rvert\rvert_2^2, \z_i^T\z_j). 
\end{equation}
Inspired by \cite[Theorem~2.1\&2.2]{el2010spectrum}, we can then make use of the power series of $g$ from Equation \ref{eq:kerneldefg} in order to find the asymptotic spectrum of the kernel matrix $K$. We separate the analysis into the diagonal and off diagonal parts of $K$. The diagonal matrix can be controlled using the Lipschitz continuity from Assumption (A.6). Furthermore, the off diagonal matrix can be controlled using the Talyor series approximation of $g_i$, for which we use the differentiability assumptions in Assumption (A.5), and the Frobenius norm, which is an upper bound for the spectral norm. As a result, we can show Proposition \ref{prop:elkarouiextension}.
\begin{prop}
\label{prop:elkarouiextension}
Assume that the Assumptions A.1-A.6 hold ture. Then, we have that
\begin{equation}
    \lvert\lvert K- M \rvert\rvert_2 \to 0 ~~~ a.s.
\end{equation}  
with
\begin{equation}
\label{eq:elkarouiM}
\begin{split}
    M &= \textbf{I}_n\left(k(e_1,e_1)  - \sum_{i =0}^p g_i(1,1) \right) +  \sum_{i=0}^p (\textbf{X}^T\textbf{X})^{\circ i} \circ \left[
\sum_{m =0}^{p-i} \sum_{k = 0}^{m}  \frac{g_{i}^{(k,m-k)}(1,1)}{k!(m-k)!} \psi^{\circ k} (\psi^{\circ (m-k)})^T \right]
\end{split}
\end{equation}
\end{prop}
Here,  $\lvert\lvert . \rvert\rvert_2$ denotes the operator norm of the matrix and $\circ i$ denotes the $i$-times Hadamard product. In addition, for any $ j\leq p+1,$ $ \alpha = (i_1,i_2)$ and denote $g_j^{(\mathbf{\alpha})}$  the partial derivatives $g_j^{(\mathbf{\alpha})}(x,y) = \frac{\partial^{|\alpha|}}{\partial t_1^{i_1} t_2^{i_2}} g_j(t_1,t_2)|_{x,y}$ and $\psi$ is the vector with entries $\psi_i = ||X_i||_2^2 - 1$. As a consequence, we can see that $M$ and $K$ have asymptotically the same Eigenvalues, from which Corollary \ref{cr:EVlowerbound} follows. \newline
Next, using the fact that $(K + \lambda \textrm{I}_n)$ has lower bounded Eigenvalues and following a similar argument for $K^*$ as used for Proposition \ref{prop:elkarouiextension}, we can then derive Theorem \ref{th:main} in the Appendix. As a consequence, we will see that for any $n$, there exits a polynomial $p$ of degree at most $2 \floor{2/\beta}$ such that with high probability over the draws of $\x^*$, we have that
\begin{equation}
\label{eq:fhatpoly}
 |\fhat_{\textrm{ns},\lambda}(\x^*)- p(\x^*)| \to 0 ~~a.s.,
\end{equation}
where we make use of the fact that $\fstar$ is bounded. In fact, we will see that the convergence happens uniformly, which allows us to use it in order to bound the Bias depending on the projection error of polynomials. Finally, we require the truncated expression of the polynomials used for the definition of $\overline{B}_{\leq m,C}$ in order to control the effect of the probability regions of $\xstar$ for which Equation \ref{eq:fhatpoly} does not hold true. As a result, we can then show Theorem \ref{th:main_text}.


==> sections/old_sections_v2/new_Section6.tex <==
\newpage

\section{Experiments}
\label{sec:6}
We now describe some numerical experiments that provide illustrative confirmations of the lower bound on the bias depending increasing with the parameter $\beta$. We study the following two different input data models:
\begin{itemize}
    \item \textbf{Model 1:} $\tilde{Z}_i[k] \sim \mathcal{N}(0,1)$; $d = \floor{n^{\beta}}$; $\Sigma_d = \textrm{I}_d$.
    \item \textbf{Model 2:} $\tilde{Z}_i[k] \sim \textrm{Uniform}(-C_U,C_U)$; $d = n$; $\Sigma_d$ is the diagonal matrix with entries $\Sigma_{d,i,i} = \lambda_i = (1 - ((i-1)/d)^{\kappa})^{1/\kappa}$ and $\kappa \geq 0$ such that $\trace(\Sigma_d) = \sum_{i=1}^n \lambda_i = n^{\beta}$.
\end{itemize}
We choose $C_U$ such that the variance of the random variable $Z_i[k]$ is one. Finally, for both models, we generate the input data $Z_i = \Sigma_d^{1/2} \tilde{Z}_i$ and normalise them to $X_i = \frac{1}{\sqrt{\trace(\Sigma_d)}}$. 
 We remark that the first model corresponds to the regimes studied in \cite{Liang20b} the second to the regimes studied in \cite{Rakhlin19}. For our analysis, we use the $\alpha$-exponential kernels of the form $k(X,X') = \exp\left(- \tau^{\alpha/2} \lvert\lvert X-X' \rvert\rvert_2^{\alpha} \right)$, and the exponential inner product kernel of the form $k(X,X') = \exp\left(\tau X^TX'\right)$. Furthermore, the ridge parameter $\lambda$ is well known to regulate the Bias-Variance trade off of the estimator $\hat{f}_{\lambda}$. Since we are primarily interested in the Bias term of the estimator, we only make experiments for the case where "ridge-less" case where $\lambda = 0$. 
 
 \subsection{Experiment 1}
 
 \begin{figure}
     \centering
     \minipage{0.24\textwidth}
  \includegraphics[width=\linewidth]{Plots/Breakpoint2_mdl1.png}
\endminipage\hfill
     \minipage{0.24\textwidth}
  \includegraphics[width=\linewidth]{Plots/Breakpoint2_mdl2.png}
\endminipage\hfill
     \minipage{0.24\textwidth}
  \includegraphics[width=\linewidth]{Plots/Breakpoint_mdl1.png}
\endminipage\hfill
     \minipage{0.24\textwidth}
  \includegraphics[width=\linewidth]{Plots/Breakpoint_mdl2.png}
\endminipage\hfill
\caption{ Bias with respect to $\beta$}{ The first two plots show the bias of $f^*_1$ for the first and second model and the other two figures show the same for the ground truth function $f^*_2$. In total $5000$ input data points are used for training and $25000$ for testing.}
\label{fig:exp1_p1}

 \end{figure}
 
 
 In a first experiment, we illustrate the Bias with respect to the parameter $\beta$ for the two sparse ground truth functions $f_1^*(X) = 2 Z[1]^2 = 2 \trace(\Sigma_d) X[1]^2 $ and $f_2^*(X) = 2 Z[1]^3 = 2 \trace(\Sigma_d)^{3/2} X[1]^3 $. Because the estimator $\hat{f}_{\lambda}$ depends only only linearly on the observations $Y$ ( recall Equation \ref{eq:kernelridge}, we can estimate the Bias term by computing the risk when using noise less observations for training, i.e. $Y_i = f^*(X_i)$. Figure \ref{fig:exp1_p1} shows the estimated bias for both models with respect to $\beta$. We can clearly observe for both input data sets, that the bias increases with respect to $\beta$. In particular, we observe that this happens similarly for all kernels, underlining the observation from our theoretical results that the lower bound of the Bias is independent of properties such as the Eigenvalue decay of the kernels. Finally, Corollary \ref{cr:biaslimit} separates the bias into different regimes of $\beta$. We can also make this observation in Figure \ref{fig:exp1_p1} when comparing the plots for $f^*_1$ and $f^*_2$. 
 \Comment{Missing: Make bridge to Linear Regression, i.e. the bias can not be overcome by making $\Sigma$ more spiky/less spiky. }
 
 \subsection{Experiment 2}
 The second experiment illustrates the dependency of the bias on $\tau$. \\
\Comment{Conclusion: Gaussian potentially diverges, for Laplacian, we can see that minimum bias is reached at $\tau -> 0$ (i.e. Flat limit)}
 
 
  \begin{figure}
     \centering
     \minipage{0.49\textwidth}
          \centering
  \includegraphics[height=4cm]{Plots/Tau_mdl1.png}
  \label{fig:awesome_image1}
\endminipage\hfill
     \minipage{0.49\textwidth}
          \centering
  \includegraphics[height=4cm]{Plots/Tau_mdl2.png}
\endminipage\hfill
\caption{Dependency of the bias on $\tau$}{ The bias is plotted with respect to $\tau$ for different choices of $\beta$ and for the Laplacian ($\alpha = 1$) and Gaussian ($\alpha =2$) kernels. 
The first plot shows the case where the data is generated from the first model and the second from the second model. In total $5000$ input data points are used for training and $25000$ for testing. In addition, we perform $100$ iterations each to estimate bias. The variance is then computed by taking the difference of the mean of the risk and the bias. The ground truth function is $f^*_3$.}
\label{fig:exp2}
 \end{figure}
 
 
 
\subsection{Experiment 3}
For this experiment, we generate the observations from $Y_i = f_2^*(X_i) + \epsilon_i$, with $\epsilon_i \sim \textrm{Uniform}(-10,10)$. Figure \ref{fig:exp2} shows the Bias-Variance decomposition of the risk.  
 \Comment{As a last experiment, we are interested in studying the Bias-Variance decomposition. => Future research, study dependency of variance on structure of Sigma. Here, we can mention Rakhlin and make the point that his bounds on the variance diverges when $\trace(\Sigma_d) /d \to 0$. }
 \begin{figure}
     \centering
     \minipage{0.49\textwidth}
          \centering
  \includegraphics[height=4cm]{Plots/Breakpoint_mse.png}
  \label{fig:awesome_image1}
\endminipage\hfill
     \minipage{0.49\textwidth}
          \centering
  \includegraphics[height=4cm]{Plots/Breakpoint2_mse.png}
\endminipage\hfill
\caption{Bias-Variance decomposition of risk with respect to $\beta$}{ The risk, bias and variance are plotted for the case where $\alpha=1$. The first plot shows the case where the data is generated from the first model and the second from the second model. In total $5000$ input data points are used for training and $25000$ for testing. In addition, we perform $100$ iterations each to estimate bias. The variance is then computed by taking the difference of the mean of the risk and the bias.}
\label{fig:exp2}
 \end{figure}
 \subsection{Experiment 4}
 Real world experiment.

==> sections/old_sections_v2/new_section1.tex <==

\section{Introduction}
Kernel methods offer a great amount of flexibility with the ability to interpolate even noisy features. While this allows the models to approximate highly non linear functions well, according to conventional wisdom explicit regularisation should be added to the least-squares objective in order to prevent "overfitting" \cite{Golub79,Wahba90,Smola98,Shawe04,Evgeniou00,Devito05,Alvarez11}. One very popular variant of regularised kernel methods is the kernel ridge regression algorithm which is consistent for a large set of different kernel functions, given that the dimension of the input data does not change with respect to the size of the data set \cite{Christmann07}. In fact, \citet{Rakhlin18} explicitly shows that for the case where the kernel function is the Laplace kernel, regularisation is necessary for kernel regression to achieve consistency when observation noise is present.\newline\newline
While the classical literature largely agrees on the importance of regularisation for highly flexible models, Over-parameterised deep neural networks are capable of interpolating even noisy training data while still generalising well \cite{Zhang16}. This has led to a surge of works analysing interpolating linear and kernelised estimators. In particular, recent work studying kernel "ridge-less" regression, i.e. the solution obtained when letting the ridge regularisation parameter go to zero and thus interpolating the data, demonstrates both from an empirical perspective using real world data sets \cite{Belkin18c,Geifman20} as well as from a theoretical perspective \cite{Liang20a,Liang20b} that kernel "ridge-less" regression works well for high dimensional data sets. These results hold true even when observation noise is present and thus question the classical wisdom of the necessity of regularisation for good generalisation performances. \newline \newline
Both works \cite{Liang20b,Liang20a} study linear covariance data models for which the authors claim that kernel "ridge-less" regression can achieve consistency in certain high dimensional regimes where the dimension of the input data $d$ increases with the data set size $n$. 
Especially the assumptions used for the results by \citet{Liang20b} hold true for a broad class of ground truth function, implying that consistency is not limited to very specific ground truth functions. \citet{Ghorbani19,Ghorbani20} take a different approach and the setting where the input data is generated by drawing i.i.d samples from the unfirom distribution on the hyper sphere, respectively on the product of two hyper sphere of different radii. In contrast to the work arguing that kernel interpolation works well in high dimensions,  \citet{Ghorbani19,Ghorbani20} show that consistency can be reached at most for polynomial ground truth functions of a certain order. \newline \newline
In this paper, we highlight the discrepancy in the current literature on the set of functions for which consistency can be reached, and ask for the limitations of kernel ridge and particularly "ridge-less" regression in high dimensional settings. As a first contribution in our paper, we empirically and theoretically underline that the \textit{Reproducing Kernel Hilbert Space} (RKHS) norm of even very simple ground truth functions increases when raising the dimension of the input space. As a result, we question the applicability of the upper bound on the bias presented by \citet{Liang20a} which relies on the assumption that the RKHS norm of the ground truth function stays bounded for any dimension of the input data. The second and main contribution of this paper is to theoretically derive a novel lower bound on the bias term for kernel ridge and "ridge-less" regression in high dimensional regimes. We only study the case where the kernel function is rotationally symmetric which holds true for a large amount of different kernels used in the literature \cite{Ghorbani19,Ghorbani20,Liang20a,Liang20b,Belkin18c,Geifman20}. Our results apply for the case where the data is generated from a linear covariance model but can also be adapted to the case where the data is normalised and thus lives on a hyper sphere. As a result of our study, we can see that our presented lower bound can only vanish if the ground truth function is almost everywhere a polynomial. This stands in agreement with the intuitions gained from the papers \cite{Ghorbani19,Ghorbani20}. In particular, we show that the maximum order of the polynomial only depends on the trace of the covariance matrix of the data but no on the explicit structure. 
Finally, we we empirically verify our theoretical results using both synthetic and real world data sets. 
\newline \newline
Our results clearly limit the set of ground truth functions for which consistency can be reached, and thus questions the generalisation capabilities of kernel interpolation in high dimensional regimes. As a consequence, our research puts the claim that regularisation can be avoided in high dimensional settings into perspective. Instead, our observations indicate rather the opposite, namely that both kernel ridge and "ride-less" regression are not capable of approximating highly non-linear ground truth function well in high dimensions. In order to reach consistency, the data must be projected onto a lower dimensional subspace, where classical wisdom applies and hence regularisation is known to be important for good generalisation. This intuition can also be empirically observed for real world data sets, highlighting the fact that these issues should also be taken into consideration for real world applications.
\newline\newline 
Besides these general consequences, we  discuss in the paper several special cases of kernels for which the assumptions used for the statements apply. For instance, our theorems apply to a broad range of inner product kernels which put the results from the papers \cite{Liang20b,Liang20a} into perspective. Another example are the $\alpha$-Exponential kernel functions, which are well known to cover a broad spectrum of different Eigenvalue decays. As a consequence, we can observe that the non vanishing bias issue is not limited to certain Eigenvalue decays of the kernel operators. Finally, we mention that our results also apply to the Neural Tangent Kernels (NTK) of any depth with a broad range of distinct activation functions including the popular Relu activation. Hence, we can see that when increasing the depth of the NTK kernel the lower bound on the bias does not improve. This clearly limits the benefit of higher depths for NTK kernels, especially when the bias is the dominant term in the risk. 
\newline\newline
The reminder of the paper is structured as follows. In Section \ref{sec:2}, we provide background on RKHS and kernel ridge and "rige-less" regression. Section \ref{sec:3} presents a discussion on the dependency of the RKHS norm on the dimension $d$, followed by the statement of the main results in Section \ref{sec:4}. While our main results require a specific choice of the scale parameter of the kernel, in Section \ref{sec:5} examples for other choices of the scale parameter are discussed. Finally, in Section \ref{sec:6} we provide simulations and real world experiments to underline our theoretical insights. 
\newline


==> sections/old_sections_v2/new_section2.tex <==

\section{Background}
\label{sec:2}

\subsection{Kernel Ridge Regression}
 Let $\mathcal{X}$ be some non empty subset of $\mathbb{R}^d$ and define $k: \mathcal{X} \times \mathcal{X} \to \mathbb{R}$ to be some positive definite kernel, i.e. where for any set of input vectors $\textbf{X} = \{x_1, \cdots,x_n\}$ in $\mathcal{X}$, the empirical kernel matrix $K$ with entries $K_{i,j} = k(x_i,x_j)$ is positive semi definite. For every positive definite kernel, there exists a unique corresponding reproducing kernel Hilbert space $\mathcal{H}$ (RKHS, see standard sources \cite{Wahba90,Berlinet04,Smola98}), consisting of functions mapping $\mathcal{X}$ to $\mathbb{R}$. We denote with $\langle.,.\rangle_{k}$ the corresponding inner product of the RKHS and by $\lvert\lvert . \rvert\rvert_{\mathcal{H}} := \sqrt{\langle.,.\rangle_{k}}$ the corresponding norm.\\
In addition to the input vectors $\textbf{X}$, assume that we observe a vector $\y \in \mathbb{R}^n$ of response variables, where every entry $y_i$ is the response of the system for the corresponding input vector $x_i$. Based on these input output pairs, kernel ridge regression estimates the ground truth function of the underlying system by solving the following minimisation problem
\begin{equation}
\label{eq:krr}
    \hat{f}_{\lambda} = \underset{f \in \mathcal{H}}{\arg\min} ~~\sum_{i=1}^n \left(y_i - f(x_i)\right)^2 + \lambda \lvert\lvert f \rvert\rvert_{\mathcal{H}},
\end{equation}
where $\lambda>0$ is the ridge parameter. An important extension, which is also studied in this paper, is the kernel "ridgeless" estimator. This estimator is defined to be the limit when letting $\lambda \to 0$:
\begin{equation}
    \hat{f}_{0} := \lim_{\lambda \to 0} \left[ \underset{f \in \mathcal{H}}{\arg\min} ~~\sum_{i=1}^n \left(y_i - f(x_i)\right)^2 + \lambda \lvert\lvert f \rvert\rvert_{\mathcal{H}} \right].
\end{equation}
We refer to this estimator as the solution of kernel ridged regression when choosing $\lambda = 0$. Interestingly, in this case, the estimator interpolates the data. This can be seen best when noting that the the solution solution of kernel "ridgeless" regression satisfies the following constraint minimisation problem 
 \begin{equation}
 \label{eq:constraint_min_p}
     \begin{split}
         \hat{f}_0 = \underset{f \in \mathcal{H}}{\arg\min} ~ \lvert\lvert f \rvert\rvert_{\mathcal{H}} ~~ \textrm{such that}~~ \forall i:~f(\x_i) = \y_i 
     \end{split}
 \end{equation}
 

\subsection{Risk of an Estimator}
Assuming that the data set is generated by drawing i.i.d. samples from a joint distribution $(x_i, y_i)_{i=1}^n \sim P_{X,Y}$, we can ask for the risk of an estimator, which is defined to be
\begin{equation}
    \label{eq:risk}
    \textbf{R}(\fhat_{\lambda}) := \mathbb{E}_{Y|X} \mathbb{E}_{X}\lvert \fhat_{\lambda}(\Xrv) - \fstar{\lambda}(\Xrv) \rvert^2,
\end{equation}
where $f^*(x^*)$ is called the ground truth function which is defined to be the mean of $y$ given $x^*$, i.e. $f^* := \mathbb{E}_{y\sim P_{Y|X}} y$.
Furthermore, the expectation $\mathbb{E}_{Y|X}$ is taken with respect to the distribution $P_{Y|X=\textbf{X}}$, which is the conditional distribution of the observations given the input samples $\textbf{X}$. In addition, the expectation $\mathbb{E}_{X}$ is with respect to the marginal distribution $P_{X}$. When analysing the risk of an estimator, it is often convenient to decompose the risks into two terms called the \textit{Bias} $\textbf{B}(\hat{f}_{\lambda})$ and \textit{Variance} $\textbf{V}(\hat{f}_{\lambda})$ of the estimator:
\begin{equation}
    \label{eq:biasvariance}
        \textbf{R}(\hat{f}_{\lambda}) := \underbrace{\mathbb{E}_{X} \lvert \mathbb{E}_{Y} \hat{f}_{\lambda}(\Xrv) - \fstar(\Xrv) \rvert^2 }_{=: \textbf{B}}+ \underbrace{\mathbb{E}_{X} \lvert \mathbb{E}_{Y}\fhat_{\lambda}(\Xrv) - \fhat_{\lambda}(\Xrv) \rvert^2}_{=: \textbf{V}}.
\end{equation}
 This decomposition of the risk is the well known \textit{Bias-Variance}. 



























==> sections/old_sections_v2/new_section3.tex <==
\section{RKHS-Norm in High Dimensions}
\label{sec:norm}
\label{sec:3}
\citet{Liang20a} derive a bound for the risk for kernel "ridge-less" regression in high dimensional settings based on the bias-variance decomposition. While the bound of the Variance \cite[Theorem~2]{Liang20a} only applies to the specific setting used in the paper, the authors highlight that their bound on the bias \cite[Theorem~3]{Liang20a} does only make very few assumptions and thus can be applied to much more general settings. Informally stating, the bound has the form 
\begin{equation}
\label{eq:rakhlinbound}
    \textbf{B} \leq \lvert\lvert f^* \rvert\rvert_{\mathcal{H}} ~C_1(\lambda_1(K),..., \lambda_n(K)) + C_2(n),
\end{equation} 
where $C_2(n) \to 0$ as $n \to \infty$ and $C_1(\lambda_1(K),..., \lambda_n(K))$ depends only on the eigenvalues of the empirical kernel matrix $K$. In particular, under the assumption that the RKHS norm $\lvert\lvert f^* \rvert\rvert_{\mathcal{H}}$ stays bounded for any d, \citet{Liang20a} shows that the Bias can vanish even in high dimensional regimes. Unfortunately, this assumption is not further discussed in the paper and simply assumed to be true. \\
As a first step in this paper, we highlight that the RKSH norm $\lvert\lvert f^* \rvert\rvert_{\mathcal{H}}$ can go to infinity as $d \to \infty$ even for very simple ground truth functions $f^*$. Therefore, we can conclude that although $C_1\to 0$ from Equation ~\ref{eq:rakhlinbound}, we can not conclude that the Bias vanishes for general ground truth functions. In fact, we will see that our observations hold true for very simple functions, and therefore, as a conclusion we question whether the assumption that the RKHS norm $\lvert\lvert f^* \rvert\rvert_{\mathcal{H}}$ is bounded holds true for any function of practical interests. \\
In the following subsection we empirically analyse the dependency of the RKHS norm for the popular Gaussian, Laplacian and exponential inner product kernel. We remark that the exponential inner product kernel has been used for the experiments in the paper \cite{Liang20a}. Furthermore, in a the subsequent subsection, we introduce an example for an RKHS where we can explicitly study the dependency of the RKHS norm on the dimension $d$. The purpose of this theoretical example is to give an intuition on the dependency of the RKHS norm on $d$ and in particular why the norm should increase with respect to $d$.

\subsection{Experiments for RBF and Inner Product Kernels}
In this subsection, we empirically study the RKHS norm on the space $[0,1]^d$ of the popular Gaussian kernel $k(\xk,\xkd) = \exp(-\tau \lvert\lvert \xk-\xkd \rvert\rvert_2^2)$ and Laplace kernel $k(\xk,\xkd) = \exp(-\sqrt{\tau} \lvert\lvert \xk-\xkd \rvert\rvert_2)$. Furthermore, we study the exponential inner product kernel $k(\xk, \xkd) = \exp(-\tau \xk^T\xkd)$, which is used for the examples in the paper \cite{Liang20a}. The goal of this section is to highlight our observation that the RKHS norm increases with respect to the dimension $d$ even for very simple functions. \\
For our experiments, we choose $\tau = \frac{1}{d}$, which is commonly used in the high dimensional kernel literature \cite{ElKaroui10,Liang20a,Liu20,Ghorbani19,Liang20b}. 
Although the RKHS norm does in many cases not have a closed form solution, we remark that for any set of inputs $\Xs$ and observations $y$, we can compute the RKHS norm of the estimator $\fhat_{\lambda}$, which is given by 
\begin{equation}
    \lvert\lvert \fhat_{\lambda} \rvert\rvert_{\mathcal{H}} = y^T (K +\lambda \textrm{I}_n)^{-1} K (K +\lambda \textrm{I}_n)^{-1} y
\end{equation}
Choosing $\lambda = 0$ results in the case where $\hat{f}_{\lambda}$ interpolates the data and because $\fhat_{\lambda}$ is the solution of the minimisation problem from Equation ~\ref{eq:krr}, we know that $\fhat_{\lambda}$ is the function with minimum RKHS norm such that $f(\x_i) = y_i$. Hence, assuming that $y_i = f^*(\x_i)$ are noiseless observations, we get that $\lvert\lvert \fhat_0 \rvert\rvert_{\mathcal{H}} \leq \lvert\lvert \hat{f}^* \rvert\rvert_{\mathcal{H}}$. This allows us to get an estimate of the lower bound for the RKHS norm. \\
In order to estimate the RKSH norm of the function $\fstar(\xstar) = \xstar_{(1)}$, i.e. the linear function of the first dimension, we draw $7500$ i.i.d random samples $\Xs$ from the uniform distribution over $[0,1]^d$ and set the observations $y_i$ to the ground truth values $y_i = \fstar(\x_i) = \x_{i,(1)}$. In addition, we use $7500$ random test samples to estimate the maximum test error. The amount of training data points is then chosen such that we can ensure that the maximum train error is below $0.1$ in order to guarantee that $\fhat_0$ approximates $\fstar$ well. Figure ~\ref{fig:rkhsnorm} shows the approximated RKHS norm when increasing the dimension $d$. We can clearly see that the assumption that the RKHS norm is bounded, is not justified for any of the analysed kernels. Although we only show the single case where the function is a simple sparse linear function, we expect a similar behaviour for other functions of interests. 




\begin{figure}
    \centering
    \includegraphics[height=4cm]{Plots/RKHSplot.png}
    \caption{RKHS Norm}{Figure ~\ref{fig:rkhsnorm} plots the RKHS norm on the space $[0,1]^d$ of the function $f\star(\xs) = \xs_1$, showing that the norm increases with respect to the dimension $d$ on the. The plot shows the curve for the Laplacian, Guasian and inner product exponential kernel. }
    \label{fig:rkhsnorm}
\end{figure}







\subsection{Example: Tensor Product Kernels}
In this subsection, we further highlight the dependency of the RKHS norm on the dimension $d$ by construction an explicit example for an RKHS norm which we can then study more detailed. We construct a simple tensor product space RKHS with reproducing kernel $k: [-\frac{1}{2},\frac{1}{2}]^d \times   [-\frac{1}{2},\frac{1}{2}]^d \to \mathbb{R}$ of the form 
 \begin{equation}
   k(\xk ,\xkd) = \prod_{j=1}^d q^d(\xk_j, \xkd_j),
 \end{equation} 
with translation invariant kernels $q^d: [-\frac{1}{2},\frac{1}{2}] \times  [-\frac{1}{2},\frac{1}{2}] \to \mathbb{R}$ defined using the Eigenfunctions of the Fourier series :
\begin{equation}
\label{eq:sec3fourier}
    q^d(\xk,\xkd) = \sum_{j=-\infty}^{\infty} q^d_j \exp\left(2\pi j i (\xk-\xkd)\right) .
\end{equation}
 Here, $i$ is the imaginary unit and $q^d_j$ are the Fourier coefficients satisfying $q^d_j \geq 0$ and $q^d_j = q^d_{-j}$. We remark that the assumption that the sum from Equation ~\ref{eq:sec3fourier} converges together with the conditions on $q^d_j$ is sufficient and necessary in order to guarantee that $q^d$ is a positive definite function. Furthermore, we highlight that the kernel function $q^d$ depends on the dimension $d$, meaning that $k$ can change with the dimension $d$. This assumption is usually given, when for example analysing kernels which depend on a scale parameter changing with $d$. In order to guarantee that the kernel $k$ behaves well when increasing the dimension $d$, we make the additional assumption that for any $d$ and for every $\xk \in [-\frac{1}{2},\frac{1}{2}]^d$, $k(\xk,\xk) = 1$.   
Note that this is equivalent to saying that for any $\xk \in [-\frac{1}{2},\frac{1}{2}]$, $q^d(x,x) = 1$, which is implies that $\sum_{i=-\infty}^{\infty}q_i = 1$. 
 \\
Although our constructed class of kernels does not include popular kernels such as the Gaussian kernel as special cases, we remark that there exists a connection between our studied kernels and the Gaussian kernel. We refer to \cite[Example~12.24\&25]{Wainwright19} for further details. Furthermore, we remark that our constructed kernels cover a very broad spectrum of different Eigenvalue decays, and hence, our analysis gives also good intuitions for kernels with non exponential decays like for example the Laplacian kernel. 
\\
Interestingly, we can see from \cite[Proposition~12.31]{Wainwright19} that the induced RKHS norm has a simple expression for product typed functions of the form $f(\xk) = \prod_{j=1}^d f_j(\xk_j)$, given by
\begin{equation}
\label{eq:sec3closeform}
\lvert\lvert f \rvert\rvert^2_{\mathcal{H}_k} = \prod_{j=1}^d \lvert\lvert f_j\rvert\rvert^2_{\mathcal{H}_{q}}
\end{equation}
where $\lvert\lvert f_j\rvert\rvert_{\mathcal{H}_{q}} $ is the RKHS norm induced by $q^d$. Although the RKHS contains much more functions than only product functions, we remark that we have only access to a closed form expression of the RKHS norm for product functions. We can now state Lemma ~\ref{lm:rkhs}:
\begin{lemma}
\label{lm:rkhs}
Assume that $f$ is a non constant sparse product function $f(\xk) = \prod_{j=1}^m f_j(\xk_j)$. Then, for every sequence of coefficients $q_j^{d}$, 
$$ ||f||_{\mathcal{H}_k}  \overset{d \to \infty}{\to} \infty $$
\end{lemma}
 Lemma ~\ref{lm:rkhs} shows that for any sparse non constant product function, there exits no sequence of kernels $q^d$, such that the tensor product RKHS norm stay bounded when $d\to\infty$. In fact, this holds true for any Eigenvalue decay. While a similar result can also be stated for the case where the product function $f$ is non sparse, this would require additional notation which is why we omit the extension. Finally, due to the triangular inequality, we would expect this to be also the case for arbitrary functions in the RKHS. As a consequence, we can conclude that Lemma ~\ref{lm:rkhs} clearly demonstrates the dependency of RKHS norms on the dimension $d$ and highlight of divergence with respect to $d \to \infty$ occurs for any Eigenvalue decay of the kernel. While it is well known that kernel with similar Eigenvalue decays have similar RKHS \textbf{(Cite this)}, we expect to observe the described phenomenon also for more general kernels. 
\Comment{Not sure how much more I should say at this point....}





==> sections/old_sections_v2/new_section4.tex <==

\section{Main Result}
\label{sec:4}

While there exists multiple paper on kernel ridge and especially "ridge-less" regression claiming that consistency can be reached for rotationally symmetric kernels in high dimensional regimes \cite{Liang20a,Liang20b,Liu20,Ghorbani19,Ghorbani20}, we highlight that the current literature is unclear about the set of ground truth functions for which this is true. On the one hand, \citet{Ghorbani19,Ghorbani20} showed that we can at most approximate polynomials of a certain degree when assuming that the input data sets are drawn from the uniform distribution on the hyper sphere, respectively on the product of two hyper spheres of different radii. In contrast, on the other hand, in the papers \cite{Liang20a,Liang20b,Liu20} linear covariance data models are studied, where less restrictive assumptions on the ground truth function are imposed. In particular, these results do not limit the ground truth function to polynomials. In the last section, we have already questioned the applicability of the bias bound from \cite[Theorem~3]{Liang20a}. Still, it is yet unclear how the discrepancy in the results for the linear covariance data models \cite{Liang20b,Liu20} with the ones for spherical input data \cite{Ghorbani19,Ghorbani20} can be reached can be explained. 
\newline
In this paper we take a different approach  and show that the estimator of kernel ridge and "ridge-less" regression looks asymptotically almost everywhere like a polynomial. As a result, we can conclude that consistency can be only reached for a limited set of ground truth functions. Our results therefore build upon the intuitions gained from the papers \cite{Ghorbani19,Ghorbani20} and extend them to a much broader class of data distributions.\newline \Comment{Not sure how much more we need to say here- i feel it becomes a bit repetitive. } \newline
\Comment{Say something like in a first step of this section blabla}\newline


\subsection{Setting and Assumptions}

We impose the following assumptions on the distribution of the data:
\begin{itemize}
\item[(A.1)] \textit{Data-Distribution}: Assume that $x_i = \Sigma_d^{1/2} \xtilde_i $ with $\xtilde_i \in \mathbb{R}^d$ random vectors with i.i.d entries $\xtilde_{i,j}$ of zero mean and unit variance. In addition, we assume that either $\xtilde_{i,j}$ is normally distributed or $|\xtilde_{i,j}| \leq C_{\xtilde} ~a.s.$ with $C_{\xtilde}>0$ some constant. Finally, we assume that $\lvert\lvert \Sigma_d \rvert\rvert_2 = 1$. 
\item[(A.2)] \textit{High Dimensionality of the Problem}: $d_{\textrm{eff}} := \trace(\Sigma_d) \asymp n^{\beta}$ with $\beta \in (0,1]$.  
\item[(A.3)] \textit{Ground Truth Function}: The absolute value of the ground truth function $\lvert f^* \rvert \leq C_{f^*}$ is almost surely bounded by some constant $C_{f^*} >0$ for any $n$. 
\end{itemize}
Let $k^* \in \mathbb{R}^{n}$ be the vector with entries $k^* = k_{\tau}(x_i, x^*)$. In order to be able to make use of closed form expression of $\fhat_{\lambda}$,
\begin{equation}
\label{eq:kernelridge}
    \hat{f}_{\lambda}(\xstar) = \y^T (K+ \lambda \textbf{I}_n)^{-1}k^*,
\end{equation}
which is due to the well known Representer Theorem shown by \citet{Schoelkopf01}, we assume that the kernel matrix $K$ is almost surely invertible with respect to the draws over the data sets $\Xs$. We remark that this assumption is guaranteed to be the case for any universal kernels such as the Gaussian or Laplacian RBF kernels. We remark that as a consequence, we can write the bias $\textbf{B}(\hat{f}_{\lambda})$ as
\begin{equation}
\label{eq:biassimplified}
   \textbf{B}(\hat{f}_{\lambda}) = \mathbb{E}_{X} \lvert f^*(\Xs)^T (K + \lambda \textrm{I}_n)^{-1} k^*(X) - f^*(X) \rvert^2, 
\end{equation}
where $\fstar(\textbf{\x})$ is the vector with entries $\fstar(\Xs)_i = \fstar(\x_i)$ and $k^*(X)$ is the vector with entries $k^*_i = k_{\tau}(x_i, X)$. \newline
 In this paper we study scale dependent kernels $k_{\tau}$ with $k_{\tau}(x,x') = k(\tau x, \tau x')$ and $k$ is some fixed positive definite kernel. For the main results of this paper we assume that the scale parameter is set to $\tau = d_{\textrm{eff}}^{-1/2}$. We refer to the Subsection ~\ref{sec:discussionofass} for a further discussion on the choice of the scale parameter $\tau$. 
 In addition, in this paper, we limit our study to kernels which only depend on the squared Euclidean norm of $\xk$ and $\xkd$ and the inner product $\xk^T\xkd$. This constraint is satisfied by a broad spectrum of commonly used kernels including any RBF kernel and any inner product kernel, but also for instance the Neural Tangent Kernels (NTK) \cite{Jacot20,Arora19}. As a consequence, the kernels $k$ are rotationally symmetric. Hence, we can use the well known result by \citet{Schoenberg1988}, showing that the restriction onto the sphere $k|_{\mathcal{S}^{d-1} \times \mathcal{S}^{d-1}}(\xk,\xkd)$ can be expressed as a power series of the form $      k|_{\mathcal{S}^{d-1}\times \mathcal{S}^{d-1}}(\xk,\xkd) = \sum_{j=0}^{\infty} c_j \xk^T \xkd$
with constants $c_j$ in $\mathbb{R}$. \newline
Based on this fact, we can now introduce Definition ~\ref{def:regrotsym}, which extends the power series expression to parts of the neighbourhood of the hyper sphere in a way such that the kernel $k$ only depends on the norm and the inner product.  
\begin{definition}
\label{def:regrotsym}
We say that a kernel function $k$ has a locally rotational symmetric power series expansion, if we can find $\delta>0,\delta'>0$ such that there exists functions $g_i: \to \mathbb{R}$ such that for any $(x,x') \in \mathbb{R}^d \times \mathbb{R}^d$, with $(||\xk||_2^2, ||\xkd||_2^2) \in  [1-\delta, 1+\delta] \times [1-\delta, 1+\delta]$ and $\xk^T \xkd \in  [-\delta',\delta']$, 
\begin{equation}
    \label{eq:kerneldefg}
    k(x,x') =  \sum_{i=0}^{\infty} (x^Tx')^i g_i(||x||_2^2,||x'||_2^2) =: g(||x||_2^2, ||x'||_2^2, x^T x')
\end{equation}
\end{definition}
Using Definition ~\ref{def:regrotsym}, we can now specify the regularity assumptions needed for the kernel function $k$:
\begin{itemize}
\item[(A.4)] \textit{Rotational Symmetry of the Kernel}: The kernel function $k$ has a \textit{locally rotational symmetric power series expansion }(Definition ~\ref{def:regrotsym}) with the additional regularity assumption that $g$ is continuous and for any $i \leq \floor{2/\beta}+1$, $g_i$ is $(\floor{2/\beta}+1-i)$-times continuously differentiable in an neighbourhood of $(1,1)$.
\item[(A.5)] \textit{Restricted Lipschitz Continuity:}The restriction of $k$  on $\{(x,x)| x \in \mathbb{R}^d, \lvert \lvert x \rvert\rvert_2^2 \in [1-\delta_L, 1+\delta_L]\}$ is a Lipschitz continuous function for some $\delta_L>0$ is from Definition ~\ref{def:regrotsym}. 
\end{itemize}

We remark that the Assumptions (A.4) and (A.5) apply to a very broad range of kernels including RBF, inner product and NTK kernels. More specific, any inner product kernel $k(\xk,\xkd) = h(\xk^T\xkd)$ with $h$ locally analytic around zero satisfies the assumptions. This fact follows trivially from the local Taylor expansion around zero, $h(\xk^T\xkd) = \sum_{j=0}^{\infty} h_i ~ (\xk^T \xkd)^j$. Similarly, the Assumptions hold true for any RBF kernels $k(\xk,\xkd) = h(\lvert\lvert \xk - \xkd \rvert\rvert_2^2)$ which is locally analytic around $2$. We refer to Lemma ~\ref{lm:RBFass} for a proof. Finally, Proposition ~\ref{prop:ntkass} shows that the Assumptions also hold true for the NTK kernels of any depth and a broad range of different activation functions. 



\subsection{Statement of the Main Results}

We can now state the main result of this paper, where we remark that the almost surely conditions, abbreviated with $a.s.$, refers to the sequence of input data sets $\Xs$ induced by $n$ when $n \to \infty$. However, we point out that the almost surely statement can also be replace with an in probability statement. We refer to Remark ~\ref{rm:astoinp} for further details. Let $\mathcal{P}_{\leq m}$ be the space of polynomials of degree at most $m$, 
$ \mathcal{P}_{\leq m} = \left\{ \sum_{j = 1}^{l} c_{j} \prod_{i=1}^d (x_{(i)}^*)^{\alpha_{j}^i} \lvert l \in \mathbb{N}, c^l_{j} \in \mathbb{R}, \alpha_{j}^i \in \mathbb{N}, \sum_{i=1}^d \alpha_{j}^i \leq m \right\} $, 
where $x^*_{(i)}$ is the $i$-th entry of the vector $x^*$. Furthermore, for any $C>0$, define $\overline{\mathcal{P}}_{\leq m,C}$ to be the space of truncated polynomials with elements $\overline{p}(x^*) = \max\left( -C, \min \left(C, p(x^*) \right)\right)$. We have:
\begin{theorem}
\label{th:main_text}
Assume that the Assumptions A.1-A.5 are satisfied. Furthermore, assume that the minimum Eigenvalues of $(\lambda \textrm{I}_n + K)^{-1}$ are almost surely lower bounded by a non zero positive constant. Then, for any $C\geq C_{f^*}$, any $\gamma >0$ and any $n$, the bias can be lower bounded by 
\begin{equation}
    \textbf{B}(\hat{f}_{\lambda})  \geq  \underset{\overline{p} \in \overline{\mathcal{P}}_{\leq m,C}}{\inf} \mathbb{E}_{X} \left| f^*(X) - \overline{p}(X)\right|^2  - \gamma ~~~a.s.
\end{equation}
with $m = 2 \floor{2/\beta}$, meaning that the bias can be lower bounded by the minimum projection error of $f^*$ onto the set of truncated polynomials of degree at most $m$.
\end{theorem}








Surprisingly, we find that bound from Theorem ~\ref{th:main_text} depends only on the growth rate of the trace $\trace(\Sigma_d)$ with respect to $n$, but not on the explicit structure of the covariance matrix $\Sigma_d$. Hence, given that $\beta$ is some constant, we find that the Bias $\textbf{B}(\hat{f}_{\lambda})$ never vanishes if the ground truth is sufficiently non linear. In fact, our results do not depend on the sparsity of the ground truth function, meaning that the issue also holds true for arbitrarily sparse ground truth functions. As a consequence, we can see that we can never reach consistency given that the ground truth function is not a polynomial of degree at most $2\floor{2/\beta}$ . Our results specify the intuition gained from the paper \cite{Ghorbani20}, where the authors show for an explicit example that spiked data models do not help to overcome the bias in high dimensions. Finally, we mention \cite[Theorem~4]{Bartlett20},  where it was shown that for the linear regression the explicit structure of the data covraiance matrix plays an important role to determine whether consistency can be reached. While this result leads to the question whether the explicit structure of the covariance matrix also determine consistency for kernel regression, our analysis clearly shows that this is not true for general non linear functions. 
\newline
\Comment{Interestingly, we can furthermore show that...}
\begin{cor}
\label{cr:poly}
Assume that the assumptions from Theorem ~\ref{th:main_text} hold true and in addition, assume that the observations $\y_i$ remain bounded for any $n$. 
Then, for any $\epsilon>0$ and any $n$ sufficiently large, there exists a polynomial $p \in \mathcal{P}_{\leq m}$, with $m =2 \floor{2/\beta}$ such that  with probability $\geq 1- \exp(-C \log(n)^{1+\epsilon'})$ over the draws of  $\xstar$,
\begin{equation}
\label{eq:degenratedf}
    \left| \hat{f}_{\lambda}(\xstar) - p(\xstar) \right| \leq \epsilon ~~ a.s.,
\end{equation}
with $\epsilon'>0, C>0$ some positive constants.
\end{cor}
 We argue that the assumption that the observations $\y_i$ remain bounded is usually justified for practical applications. Hence, if the setting is sufficiently high dimensional, such that we can assume that we have already entered the asymptotic regime, we can see that the estimator $\hat{f}_{\lambda}$ looks almost everywhere like a polynomial of degree at most $2 \floor{2/\beta}$. \newline
 

\subsection{Discussion}
\label{sec:discussionofass}
In this section, we discuss some of the assumptions imposed for the main results and the consequences of our results for various kernels. 
\subsubsection{Data Distribution}
Although our assumptions on the distribution of $\xtilde_i$ are more restrictive than the ones from the papers \cite{ElKaroui10,Liang20b,Liang20a,Liu20}, we remark that instead we allow much greater flexibility in the choice of $d$ and the covariance matrix $\Sigma_d$. The only restriction which we impose on the dimension $d$ is that $\trace(\Sigma_d) \leq d$, which is a consequence of the fact that $\lvert\lvert \Sigma_d \rvert\rvert_2 = 1$. The assumption that $\trace(\Sigma_d) \asymp n^{\beta}$ is not very restrictive and allows us to categorise high dimensional settings. Besides, we do not make any further assumptions on the covariance matrix. In fact, we remark that we obtain the setting studied in the papers \cite{ElKaroui10,Liang20a,Liu20} when $d \asymp n$ and the one studied in the paper \cite{Liang20b} when $d \asymp n^{\beta}$ and $\Sigma_d = \textrm{I}_d$. \\
While our main results are for the linear covariance model, we remark that our analysis implies similar results for the case where $x_i$ is normalised, and hence lives on the unit hyper sphere. As a result, we can see that our analysis also extends the results from \citet{Ghorbani19,Ghorbani20}, where it is assumed that the input data points $x_i$ are drawn form the uniform distribution on the hyper-sphere, respectively from the uniform distribution from the product of two hyper-spheres of different radii. We refer to the Appendix ~\ref{sec:sphere} for a discussion of this case and a comparison with the results from \citet{Ghorbani19,Ghorbani20}.
\newline
\subsubsection{Choice of the Scale Parameter}
The assumption that the kernel function depends on a scale parameter which changes with respect to $d$ is common practice in the literature \cite{Ghorbani19,Ghorbani20,ElKaroui10,Liang20a,Liang20b,Liu20}, where all cited papers choose $\tau = d^{-1/2}$. We remark that the dependency of $\tau$ on $d$ is required in order to adapt to the changing square norm of the vectors $x_i$, given by 
\begin{equation}
    \mathbb{E}~ \lvert\lvert \x \rvert\rvert_2^2  = \mathbb{E}~  \x^T \x = \trace(\mathbb{E} \x \x^T) = \trace(\Sigma_d) = d_{\textrm{eff}}
\end{equation}
 The motivation for our choice of the scale parameter $\tau = d_{\textrm{eff}}^{-1}$ is that the re-scaled inputs have squared mean $\mathbb{E} \lvert\lvert \tau x_i \rvert\rvert_2^2 =1$. This consequence is particularly important for NTK kernels, where the correspondence with infinitely wide Neural Network only holds true when the data set is carefully re-scaled \cite{Arora19,Jacot20}. 
 As a consequence, our choice of the scale parameter only agrees with the one from the mentioned paper if $d_{\textrm{eff}} = d$. While this is the case for the paper \cite{Liang20b} and also for the paper \cite{Ghorbani19} when projecting onto the hyper sphere, we remark that this is only the case for the papers \cite{ElKaroui10,Liang20a,Liu20} if $\trace(\Sigma_d) \asymp d$. We refer to the next section for a discussion of cases where $\tau$ is chosen differently. 
\newline
\subsubsection{Lower Bounded Eigenvalues}
Clearly, whenever $\lambda$ does not go to zero but instead is lower bounded by some positive constant, the Eigenvalues of $K + \lambda \In$ are also lower bounded. Furthermore, we can show that for a broad range of kernels, the kernel matrix $K$ has itself positive non zero lower bounded Eigenvalues. We already know from \cite[Theorem~2.1\&2.2]{ElKaroui10} that this is true for the RBF and inner product kernels when $\trace(\Sigma_d) \asymp d \asymp n$. We can extend these results and show that under additional assumptions on $k$, Corollary ~\ref{cr:EVlowerbound} guarantees the non zero lower bound of the Eigenvalues for a broad spectrum of kernels and distributions. 
\begin{cor}[Corollary of Proposition ~\ref{prop:elkarouiextension}]
\label{cr:EVlowerbound}
Assume that Assumption A.1-A.5 hold true. In addition, assume that that for any $j$, $g_j$ is a positive definite kernel function. Then, we have that for any $\gamma >0$, 
\begin{equation}
\label{eq:lambdamin}
    \lambda_{min}(K) \geq k(e_1,e_1) - \sum_{j = 1}^{\floor{2/\beta}} g_j(1,1) - \gamma ~~~a.s.
\end{equation}
with $e_1 = (1,0, \cdots,0)$. 
Furthermore, under the assumption that the definition of $g$ can be extended such that $k(e_1,e_1) = \sum_{i=0}^{\infty} g_j(1,1)$ holds true, we can see that the Eigenvalues of $K$ are lower bounded by a positive non zero constant if there exists $j > \floor{2/\beta}$ such that $g_j(1,1) > 0$. 
\end{cor}
We can now show various examples for which Corollary ~\ref{cr:EVlowerbound} holds true. For instance, any inner product kernel of the form $k(\xk,\xkd) = \sum_{j=0}^{\infty} h_j ~ (\xk^T\xkd)^j$ with $h_j \geq 0$ and given that there exists $\hat{j} \geq \floor{2/\beta}$ such that $h_{\hat{j}}>0$ satisfies the assumption in Corollary ~\ref{cr:EVlowerbound}. Another example are the NTK kernels of any depth. We refer to Proposition ~\ref{prop:ntkass} for a proof. Unfortunately, it is unclear whether general RBF kernel satisfy the additional assumptions in Corollary ~\ref{cr:EVlowerbound}. However, we can show that it holds true for the special case when $k(\xk, \xkd) = \exp(-\tau_0 \lvert\lvert \xk - \xkd \rvert\rvert_2^2)$ is the Guassian kernel, which follows immediately from $\exp(-\lvert\lvert \xk - \xkd \rvert\rvert_2^2) =\sum_{j=0}^{\infty} \frac{2}{j!}(\xk^T\xkd)^j \exp(-\lvert\lvert \xk \rvert\rvert_2^2)\exp(-\lvert\lvert \xkd \rvert\rvert_2^2) $. Furthermore, using a different proof technique, Proposition ~\ref{prop:alphaexp} from the appendix shows that the Eigenvalues of $K$ can also be lower bounded away from zero when $k$ is the $\alpha$-exponential kernel with $k(\xk, \xkd) = \exp(-\tau_0 \lvert\lvert \xk - \xkd \rvert\rvert_2^{\alpha})$ and $\alpha \in (0,2)$. \newline
Finally, we remark that the phenomenon of lower bounded Eigenvalues is a consequence of the high dimensionality of the input data. In contrast, in classical regimes where the dimension $d$ is constant there exists many results connecting the decay of the Eigenvalues of the kernel matrix $K$ with the Eigenvalue decay of the operator $\mathcal{T}: L^2_{\mu}(\mathcal{X}) \to L^2_{\mu}(\mathcal{X}), g \to \int_{\mathcal{X}} k(x,y) g(y) d\mu $. For instance, we refer to \cite[Theorem~2]{Belkin18} for a statement of this type. 
\subsubsection{Implications for Various Kernels}
\label{sec:variouskernels}
We can now discuss the implications of Theorem ~\ref{th:main_text} for various kernels. First of all, we note that whenever $\lambda$ dos not go to zero, based on the previous discussion, the Theorem ~\ref{th:main_text} applies for a very broad range of kernels. For the more interesting case where $\lambda = 0$ or $\lambda \to 0$, we shown in the above discussion several important examples for which Theorem ~\ref{th:main} still holds true. In this section, we are going to discuss the implication of our results for these kernels.  \newline
\textbf{Inner Product Kernels:} 
The inner product kernels are widely used in the literature \cite{Liang20b,Liu20,Liang20a,Ghorbani19,Ghorbani20,ElKaroui10}, allowing a good comparison with the existing results. In particular, \citet{Liang20b} claims that the risk vanishes in regimes where $d \asymp n^{\beta}$ with $\beta \in (0,1)$ and $\Sigma_d = \textrm{I}_d$. While it is not exactly clear which ground functions satisfy the assumption in the paper \cite{Liang20b}, as a consequence of our results, we can clearly show that this is not true given that the ground truth function $f^*$ is not a polynomial of degree at most $\floor{2/\beta}$. \newline
\textbf{$\alpha$-Exponential RBF kernels:} The second example of kernels for which we can show that Theorem ~\ref{th:main_text} applies are the $\alpha$-Exponential RBF kernels of the form $k(\xk,\xkd) = \exp(-\lvert\lvert \xk - \xkd \rvert\rvert_2^{\alpha})$ with special cases including the Laplace kernel ($\alpha =1$) and the Gaussian kernel ($\alpha = 2$). These kernels have shown strong performance on multiple high dimensional data sets as shown in the paper\cite{Geifman20}. In addition, we can see from \cite[Theorem~2.1]{Blumenthal60} that these kernels cover a broad spectrum of different Eigenvalue decays, including both exponential decay, i.e. when $\alpha =2$, and a broad range of polynomial decays, i.e. when $\alpha <2$. As a consequence, we can conclude that the phenomenon described in Theorem ~\ref{th:main_text} and Corollary ~\ref{cr:poly} appears to be independent of the Eigenvalue decay of the kernels. \newline
\textbf{Neural Tangent Kernels:} 
\newline
\Comment{Thanks to Parnians hint, our statements hold for many more activation functions than just Relu :)}
\newline
As a last example, we discuss the Neural Tangent Kernels (NTK) with activation function. Interestingly, from the above discussion, we know that the NTK of any depth satisfies the assumptions in Corollary ~\ref{cr:EVlowerbound} and thus also in Theorem ~\ref{th:main_text}. These results extend the observations for NTK's on the Hyper sphere by \citet{Ghorbani19,Ghorbani20}. Furthermore, we remark that the benefits of the depth for NTK kernels has also been questioned in the paper \cite{Bietti20}. However, our results are orthogonal to the results of \citet{Bietti20}, because their main argument is that the NTK of any depth has the same Eigenvalue decay. Since our results do not depend on the Eigenvalue decay, we highlight that our observation that the depth does not help to overcome the bias bound from Theorem ~\ref{th:main_text} is not a consequence of the results form the paper \cite{Bietti20}. \newline
\Comment{Make the point with CNTK and compositional kernels ?}


\subsection{Results for other Choices of the scale parameter $\tau$}

\label{sec:additionalresults}
This subsection studies different cases where $\tau$ is not equal to $\frac{1}{d_{\textrm{eff}}}$. For instance, this is the case for the settings in the papers \cite{ElKaroui10,Liang20a,Liu20} when $\frac{\trace(\Sigma_d)}{d} \to 0$. In this section, we study the case where $\tau = \tilde{\tau}/d_{\textrm{eff}}$ for different choices of $\tilde{\tau}$. Firs of all, we remark that the case where $\tilde{\tau}$ follows immediately from the previous section. For the other two cases, we can see form Lemma ~\ref{lm:innerpr} that $\lvert\lvert \tau \x_i \rvert\rvert_2^2 \to 0~~a.s.$ if $\tilde{\tau} \to 0$ and $\lvert\lvert \tau \x_i \rvert\rvert_2^2 \to \infty~~a.s.$ when $\tilde{\tau} \to \infty$. As a result, we can see that the behaviour of the estimator $\hat{f}_{\lambda}$ strongly depends on the behaviour of the kernel $k$ when the input data goes to zero respectively infinity. We remark that this behaviour can significantly differ even among the kernels of interests in this paper
For an example, compare the kernel functions $\exp(-\lvert\lvert \xk-\xkd \rvert\rvert_2^2)$ and $\exp(\xk^T\xkd)$. Furthermore, NTK are only the infinitely wide limit of Neural Networks if the input data is scaled appropriately \cite{Jacot20,Arora19}. Hence, the analysis for other choices of $\tilde{\tau}$ is only of limited interests for the NTK kernels. 
\\
In this paper, we only study the special case where $k(\xk,\xkd) = \exp(-\lvert\lvert \xk-\xkd \lvert\lvert_2^{\alpha})$ with $\alpha \in (0,2]$. The main purpose of this section is not to give a general statement for any choices of the parameter $\tilde{\tau}$ but rather to highlight that the phenomenon from Theorem ~\ref{th:main_text} and Corollary ~\ref{cr:poly} are not limited to an unfavourable choice of the scale parameter $\tau$. \newline
The cases where $\tilde{\tau}\overset{n\to \infty}{\to} \infty$ and $\tilde{\tau}\overset{n\to \infty}{\to} 0$, but with $\lambda$ lower bounded, can be both straightforwardly analysed given that $\tilde{\tau}$ increases respectively decays sufficiently fast. In the "ridge-less" case, where $\lambda = 0$ and $\tilde{\tau} \overset{n\to \infty}{\to} 0$ the analysis turns out to be significantly more challenging. Here, we only study the extreme case where we analyse the flat limit, i.e. the solution obtained when for any fixed $n,d$ taking the limit of $\tilde{\tau} \to 0$,
\begin{equation}
    \forall n,d ~\textrm{constant}: ~~ \fhat_{\textrm{PS}}(\xstar) := \lim_{\tilde{\tau} \to 0} \fhat(\xstar) = \lim_{\tilde{\tau} \to 0} y^T  K^{-1} k^*.
\end{equation}
In general, it is not clear whether this solution exists. However, we can apply \cite[Theorem~3.12]{Lee2014} and \cite[Theorem~2.1]{Blumenthal60} to show that for any $\alpha \in (0,2)$, $\hat{f}_{\textrm{PS}}$ exists and exactly the \textit{Polyharmonic Spline Interpolator} introduced by \citet{Wahba90} with the closed form expression:
\begin{equation}
    \fhat_{\textrm{PS}}(\xstar) = \begin{pmatrix}y \\ 0 \end{pmatrix}^T \begin{pmatrix} -D^{\alpha} & 1 \\ 1^T & 0 \end{pmatrix}^{-1} \begin{pmatrix} d^{\alpha,*} \\ 1 \end{pmatrix}.
\end{equation}
Here $D^{\alpha}$ is $n\times n$ matrix with entries $D^{\alpha}_{i,j} = \lvert\lvert \z_i-\z_j \rvert\rvert_2^{\alpha}$ and $d^{\alpha,*}$ is the vector with entries $d^{\alpha,*}_i = \lvert\lvert \z_i - \z^* \rvert\rvert_2^{\alpha}$ and with $\z_i = \tau \x_i$ and $\z^* = \tau \x^*$. We can now state the main theorem of this section. 
\begin{theorem}
\label{th:otherchoicesoftau}
Assume that the Assumptions A.1-A.3 hold true. Let $k(\xk,\xkd) = \exp(-\lvert\lvert \xk-\xkd \lvert\lvert_2^{\alpha})$ be the $\alpha$-exponential kernel with $\alpha \in (0,2]$. For any $\gamma>0$ and any $n$ sufficiently large, we have that:
\begin{enumerate}
    \item Given $\lambda = \Theta(1)$ and $\tilde{\tau} = o(n^{-1})$ or given $\tilde{\tau} = \Omega(n^{\theta})$ with $\theta>0$,
    \begin{equation}
    \textbf{B}\geq \mathbb{E}_{\Xrv} \left|\fstar(\Xrv)\right|^2 - \gamma  ~~~ a.s..
\end{equation} 
\item Given that $\alpha \in (0,2)$, 
\begin{equation}
    \textbf{B}_{\textrm{PS}} \geq  \underset{\overline{p} \in \overline{\mathcal{P}}_{\leq m,C}}{\inf} \mathbb{E}_{\Xrv} \left| \fstar(\Xrv) - \overline{p}(\Xrv)\right|^2  - \gamma ~~~a.s.
\end{equation} 
where $\textbf{B}_{\textrm{PS}}$ is the bias of the estimator $\fhat_{\textrm{PS}}$. 
\end{enumerate}
\end{theorem}
Theorem ~\ref{th:otherchoicesoftau} shows that the bound on the bias from Theorem ~\ref{th:main_text} cannot be overcome in any of the three studied cases. Surprisingly, we can see that the kernel "ridge-less" regression differs significantly from the kernel ridge regression with a constant non zero ridge parameter when $\tilde{\tau} \to 0$. Finally, we mention that \citet{Lee2014} showed that the polyharmonic spline interplator $\fhat_{\textrm{PS}}$ is the flat limit of a much broad range of different kernel functions, which implies that our results can be extended to a much broader class of kernel functions. 


==> sections/old_sections_v2/new_section5.tex <==

\section{Regularisation for Highly Non-Linear Functions}
\label{sec:5}
In this section, we discuss the relevance of regularisation in a broader perspective and incorporate our results with the literature on classical low dimensional settings. Our discussion concentrates again on the setting described by the Assumptions A.1 and A.3, however, we do not necessarily require that the regime is high dimensional, i.e. Assumption A.2. Furthermore, in order to be able to apply the classical results guaranteeing consistency, we require that the support of $X$ is compact. 
\newline
We call a kernel on a compact space $\mathcal{X}$ \textit{universal} if its corresponding RKHS is dense in the set of continuous functions $C(\mathcal{X})$ with respect to the infinity norm \cite[Definition~11]{Christmann07}. This definition applys to a braod range of popular kernel functions including the Laplace kernel as shown in \cite[Example~1]{Sriperumbudur11}. We can now summarise the positive results on consistency of kernel ridge regression from \cite[Thoerem~12]{Christmann07} and the negative results for the special case of the Lapalace kernel by \citet{Rakhlin18} in the following corollary:
\begin{cor}[Corollary of Theorem~12 ~\citet{Christmann07} \& Theorem~2.1 ~\citet{Rakhlin18}]
\label{cr:lowdimcons}
Assume that the data is distributed according to Assumptions A.1 and A.3. In addition, assume that the support of $X$ is compact and the dimension $d$ is constant. Then, under a suitable choice of the ridge parameter, kernel ridge regression for any universal kernel is consistent. In particular, this holds true for the Laplace kernel. \newline
In contrast, assume that the observations are generated by adding $i.i.d$ Rademacher noise $\xi_i$ to the ground truth function, i.e. $\y_i = \fstar(\x_i) + \xi_i$ with $P(\xi_i = 1) = P(\xi_i = -1) = 1/2$. Then, the kernel "rigde-less" regression for the Laplace kernel is never consistent. 
\end{cor}
As a result of this corollary, we can see that regularisation is explicitly required for the Laplace kernel to be consistent in fixed dimensions $d$. Furthermore, as a result of our research, we can conlcude:
\begin{cor}[Corollary of Theorem \ref{th:main_text} \& \ref{th:otherchoicesoftau}]
\label{cr:highdimcons}
Assume that the Assumptions A.1-A.3 hold true and furthermore assume that the scale parameter $\tau$ is chosen as described in Theorem \ref{th:main_text} or Theorem \ref{th:otherchoicesoftau}. Then, both kernel ridge and "ridge-less" regression for the Laplace kernel can only be consistent if for any $C>C_{\fstar}$, 
\begin{equation}
\label{eq:polyrestriction}
    \underset{\overline{p} \in \overline{\mathcal{P}}_{\leq m,C}}{\inf} \mathbb{E}_{X} \left| f^*(X) - \overline{p}(X)\right|^2 \to 0
\end{equation}
with $m = 2\floor{2/\beta}$.
\end{cor}
As a result, we can conclude that the bias does never vanish when $\fstar$ is a highly non linear function. For instance, choosing $\fstar(\xstar) = \sin(\xstar_{(1)})$ would satisfy our assumptions and hence can never be consistently learned in the described high dimensional regimes. As a consequence of Corollary \ref{cr:lowdimcons} and Corollary \ref{cr:highdimcons}, we can conclude that sufficiently non polynomial functions in the sense that Equation \ref{eq:polyrestriction} does not vanish can only be learned if the input dimension is constant and regularisation is used. 

==> sections/section2vB.tex <==

\section{Problem setting}
\label{sec:2}

In this section we define the data model and estimators we analyze in
our main results \fy{or for which we show...} and compare it with the models in the existing
literature that study kernel regression. First, we start by shortly
defining kernel regression estimators in reproducing kernel
Hilbert spaces. We then introduce our assumptions on the kernel, data
distribution and choice of asymptotic regime and compare them to
the assumptions made in related papers.

\subsection{Kernel Ridge Regression}
We consider nonparametric regression in a \emph{reproducing
  kernel Hilbert space} (RKHS) with functions on the domain $\XX \subset \R^d$ induced by a positive semidefinite kernel $\kerfunc: \XX \times \XX
\to \R$. That is, for any set of input vectors $\{\xind{1}, \cdots,\xind{n}\}$ in $\XX$, the empirical kernel matrix
$\kermat$ with entries $\kermat_{i,j} = \kerfunc{\xind{i},\xind{j}}$
is positive semi-definite. 
We denote with $\langle.,.\rangle_{k}$ the
corresponding inner product of the RKHS and by $\|
. \|_{\Hilbertspace} := \sqrt{\langle.,.\rangle_{k}}$ the
corresponding norm. \fy{for more background see ...cite...}

%% For every positive definite kernel, there
%% exists a unique corresponding reproducing kernel Hilbert space
%% $\Hilbertspace$ (RKHS, see standard sources
%% \cite{Wahba90,Berlinet04,Smola98}), consisting of functions mapping
%% $\XX$ to $\RR$.

%% that are aggregated to the data matrix $\datamatrix \in \XX^{n\times d}$ with rows $x_i$ and response vector $y\in\R^n$. 

We observe tuples of input vectors and response variables $(x,y) $ with $x \in \XX$ and $y \in \R$.
%% assume that we observe a vector $\y \in \RR^n$ of response variables,
%% where every entry $y_i$ is the response of the system for the
%% corresponding input vector $\xind{i}$. 
%% Based on these input output
%% pairs,
Given the $\numobs$ samples the ridge regression estimator %% the ground truth function of
%% the underlying system by solving the following minimisation problem
minimizes the penalized square loss
\begin{equation}
\label{eq:krr}
    \fhatridge = \underset{f \in \Hilbertspace}{\arg\min} ~~\sum_{i=1}^n \left(\y_i - f(\xind{i})\right)^2 + \lambda \| f \|_{\Hilbertspace},
\end{equation} 
where $\lambda>0$ is the ridge parameter. For consistency of ridge
regression as $n\to\infty$, $\lambda$ is usually chosen as a
sequence that vanishes which is also the setting that we
study in this paper. On the other hand if the sequence
is bounded a by a constant, inconsistency is not \fy{galopp: worth a story}.
%%  An important extension, which is also studied in this paper, is the kernel "ridgeless" estimator. This estimator is defined to be the limit when letting $\lambda \to 0$:
%% \begin{equation}
%%     \fhatinterpol := \lim_{\lambda \to 0} \left[ \underset{f \in \Hilbertspace}{\arg\min} ~~\sum_{i=1}^n \left(y_i - f(\xind{i})\right)^2 + \lambda \| f \|_{\Hilbertspace} \right].
%% \end{equation}
%% We refer to this estimator as the solution of kernel ridged regression
%% when choosing $\lambda = 0$. Interestingly, in this case, the
%% estimator interpolates the data. This can be seen best when noting
%% that the
Recently interpolants with zero training loss have also attracted
attention from the theoretical community due to curiously good
generalization properties of neural networks with zero training error.
In particular, recent papers \fy{cite} analyze the kernel "ridgeless"
estimate, or equivalently, the \emph{minimum norm interpolant}
 \begin{equation}
 \label{eq:constraint_min_p}
     \begin{split}
         \hat{f}_0 = \underset{f \in \Hilbertspace}{\arg\min} ~ \| f \|_{\Hilbertspace} ~~ \textrm{such that}~~ \forall i:~f(\xind{i}) = \y_i 
     \end{split}
 \end{equation}
Note that this is equivalent to taking $\lambda\to 0$ (for fixed $n$) for the ridge estimate in~\eqref{eq:krr}.
Our results hold for both ridge regression and the minimum norm interpolant.
 
For evaluation, we assume the observations are i.i.d. samples from
a joint distribution $(\xind{i}, y_i)_{i=1}^n \sim \jointp{X}{Y}$,
and we denote $\ftrue$ as the ground truth function that minimizes the
population square loss $\EE (Y-f(X)^2$ and can be expressed as
$\ftrue(x) := \EE [y \mid X= x]$.  We evaluate the estimator using the
population risk conditioned on the input data $\datamatrix$, defined
by
\begin{align}
    \label{eq:biasvariance}
    \Risk(\fhatridge) &\define \EE (\fhatridge(\Xrv) - \ftrue(\Xrv) )^2= \underbrace{\EE_{\Xrv} ( \EEobs \fhatridge(\Xrv) - \ftrue(\Xrv) )^2 }_{=: \text{ Bias }\Bias}+ \underbrace{\EE_{\Xrv} ( \EEobs \fhatridge(\Xrv) - \fhatridge(\Xrv))^2}_{=: \text{ Variance } \Var}. \nonumber
\end{align}
where $\EEobs$ is the
expectation taken with respect to $P_{Y|X=\datamatrix}$ and
$\EE_{\Xrv}$ is with respect to the
distribution of a test sample $X$ independent from the data.
In this paper we examine the bias which is required to vanish
in order to achieve consistency that is $\fhatridge \to \ftrue$.

%%  $\Bias$ is called the bias and $\Var$
%% %% , which is the conditional distribution of the
%% %% observations given the input samples $\datamatrix$.
%% In addition, the expectation $\EE_{\Xrv}$ is with respect to the
%% marginal distribution $P_{X}$. When analysing the risk of an
%% estimator, it is often convenient to decompose the risks into two
%% terms called the \textit{Bias} $\Bias(\fhatridge)$ and
%% \textit{Variance} $\Var(\fhatridge)$ of the estimator:
%% \begin{equation}
%%     \label{eq:biasvariance}
%%         \Risk(\fhatridge) := \underbrace{\EE_{\Xrv} \| \EE_y \fhatridge(\Xrv) - \ftrue(\Xrv) \|^2 }_{=: \Bias}+ \underbrace{\EE_{\Xrv} \| \EE_y\fhatridge(\Xrv) - \fhatridge(\Xrv) \|^2}_{=: \Var}.
%% \end{equation}
%%  This decomposition of the risk is the well known \textit{Bias-Variance}.

\subsection{Prior work on consistency of kernel regression}



\begin{figure}
    \centering
    \includegraphics[height=5cm]{Plots/RKHSNorm.png}
    \caption{RKHS Norm}{Figure ~\ref{fig:rkhsnorm} plots the RKHS norm on the space $[0,1]^d$ of the function $f\star(\xs) = \xs_1$, showing that the norm increases with respect to the dimension $d$ on the. The plot shows the curve for the Laplacian, Guasian and inner product exponential kernel. Details on the experimental setting are given in \ref{sec:rkhsexp}}
    \label{fig:rkhsnorm}
\end{figure}









\label{sec:priorkernelwork}

For ridge regression estimates in RKHS, a rich literature exists on
consistency and rate optimality for some sequence $\lambda \to 0$ as
$\numobs \to \infty$ both in the non-asymptotic
(e.g. \cite{Caponnetto07} \fy{Yun}) and asymptotic setting
\fy{check?}.  Most of them require the ground truth function to have
bounded RKHS norm or source condition parameter $r$ bounded away from
$0$. \fy{ToDO:to be fair, Rosasco/Smale source condition type stuff
  doesn't really require that... their bound depends on how ``far''
  they are from being in RKHS, as I noted before. Even considering
  this factor, it should also blow up for our examples. But then need
  to show this :/} Motivated by interpolating predictors in the deep
learning literature, some recent papers also prove consistency for minimum
norm interpolants in the high-dimensional regime \cite{Liang20a,
  Liang20b, Liu20} \fy{more, does multiple descent paper now actually prove rates?}.

In the high-dimensional setting however, it is rarely discussed how
the space of feasible, Hilbert norm bounded functions \fy{or constant $r$ for source condition}, looks like.
After all, the RKHS changes with $\dim$, in a way that depends on the
kernel. In particular, innocuous functions might have exploding RKHS
norm. For example, for common kernels such as the Gaussian, Laplacian
or expoenntial inner product kernel, the RKHS norm empirically seems
to diverge for $f_1 (x) = e_1^\top x$ \fy{add plot here}. In
Appendix~\ref{sec:norm}, we show provide a rigorous example: 
for tensor kernels of the form $\kerfunc{\xk}{\xkd} = \prod_{j=1}^d
q(x_j,x_j')$, any sparse product function of the form $\ftrue(x) =
\prod_{j=1}^d f_j(x_j)$ will have an RKHS norm that diverges,
i.e. $\|\ftrue\|_\Hilbertspace \to \infty$ as $d\to\infty$.

Can we really not learn $f_1$ consistently or is it an artefact of the
analysis?  A recent line of work Ghorbani et al.~\cite{Ghorbani19,
  Ghorbani20} provides a partial asymptotic answer when restricting
the data on the sphere without requiring bounded Hilbert norm of
$\ftrue $ to be bounded for all $\numobs$. In particular, they prove
for two distributions on the sphere (uniform and a \fy{product of two
  hyperspheres}), that ridge regression estimates and minimum norm
interpolants can consistently learn polynomials of degree at most $\frac{\log \numobs}{\log \effdim}$. \fy{check again if their results
  really also holds for non-decreasing $\lambda$ .. can't be}

Given the literature, our paper extends the analysis to a broader
set of input distributions and asymptotic regime to take a further step towards answering the question

\begin{center}
  \emph{Q: Can we consistently learn functions beyond polynomials with kernels in high dimensions?}
  \end{center}

\fy{not sure yet if it belongs here}
%% \citet{Liang20a} derive a bound for the risk
%% for kernel "ridge-less" regression in high dimensional settings based
%% on the bias-variance decomposition. While the bound of the Variance
%% \cite[Theorem~2]{Liang20a} only applies to the specific setting used
%% in the paper, the authors highlight that their bound on the bias
%% \cite[Theorem~3]{Liang20a} does only make very few assumptions and
%% thus can be applied to much more general settings. Informally stating,
%% the bound has the form
%% \begin{equation}
%% \label{eq:rakhlinbound}
%%     \Bias \leq \| \ftrue \|_{\Hilbertspace} ~C_1(\lambda_1(\kermat),..., \lambda_n(\kermat)) + C_2(n),
%% \end{equation} 
%% where $C_2(n) \to 0$ as $n \to \infty$ and $C_1(\lambda_1(\kermat),..., \lambda_n(\kermat))$ depends only on the eigenvalues of the empirical kernel matrix $\kermat$. In particular, under the assumption that the RKHS norm $\| \ftrue \|_{\Hilbertspace}$ stays bounded for any d, \citet{Liang20a} shows that the Bias can vanish even in high dimensional regimes. Unfortunately, this assumption is not further discussed in the paper and simply assumed to be true. \\
%% As a first step in this paper, we highlight that the RKSH norm $\| \ftrue \|_{\Hilbertspace}$ can go to infinity as $d \to \infty$ even for very simple ground truth functions $\ftrue$. Therefore, we can conclude that although $C_1\to 0$ from Equation ~\ref{eq:rakhlinbound}, we can not conclude that the Bias vanishes for general ground truth functions. In fact, we will see that our observations hold true for very simple functions, and therefore, as a conclusion we question whether the assumption that the RKHS norm $\| \ftrue \|_{\Hilbertspace}$ is bounded holds true for any function of practical interests.


\subsection{Our problem setting}

We now introduce our model with all the relevant assumptions on the
kernel and the data distribution.
\fy{change macro of sphere to take $d$ as argument}

\paragraph{Kernels}
%% Assuming that the input data is spherical, it is sufficient for our analysis to impose the following assumptions for the kernel $k_{\Sphere}: \Sphere^{d-1} \times \Sphere^{d-1} \to \RR$: 
%% \begin{itemize}
%%     \item[(B.1)] The kernel $k_{\Sphere}$ is positive definite, continuous and rotationally symmetric. 
%% \end{itemize}
%% For the more general case where the input data is not spherical but
%% lives in $\RR^d$

%% A well-known result by Schoenberg \cite{Schoenberg1988} then implies
%% that the restriction of $\kernf$ onto the sphere can be expressed as
%% an inner product kernel $\kressphere(\xk,\xkd) = \rotkerfunc(\xk^\top
%% \xkd)$ where $\rotkerfunc$ is a sum of Gegenbauer polynomials. When 
%%  $\rotkerfunc$ is locally analytic around $0$ we can write
%% \begin{equation}
%% \label{eq:Scheonbergseries}
%%     \rotkerfunc(\xk^\top \xkd) = \sum_{j=0}^{\infty} \rotkerfunccoeff (\xk^\top \xkd)^j
%% \end{equation}
%% with constants $\rotkerfunccoeff$ in $\RR$. \fy{RBF not included anymore?}
%% When the data lies on the sphere $\XX \subset \Sphere{d-1}$, our main
%% results are relatively easy to show using the series
%% expansion~\eqref{eq:Scheonbergseries}.  For data distributions on more
%% general $\XX \subset \R^d$ we require a few additional assumptions on the kernel function.
In this paper, we focus on continuous rotationally invariant kernels.
First, we assume that $\kernf$ only depends on the squared Euclidean
norm of $\xk$ and $\xkd$ and the inner product $\xk^\top\xkd$,
i.e. there is a function $\rotkerfunc: \R \to \R$ such that
$\kerfunc{\xk}{\xkd} = \rotkerfunc(\|\xk\|_2^2, \|\xkd\|_2^2, \xk^\top
\xkd)$.  This is satisfied by many commonly used kernels including any
radial basis function (RBF) and any inner product kernel, but also for instance the
Neural Tangent Kernels (NTK) \cite{Jacot20,Arora19}. We then require
the following assumptions to hold for the kernel function $\kernf$
locally around the sphere where the data concentrates in high
dimensions.

%%  Based on the decomposition we get form
%% Schoenberg's theorem \cite{Schoenberg1988}, we  extend the power
%% series to also include terms depending on the squared euclidean norm
%% of $\xk$ and $\xkd$:
%% Where $g_i: \R\times \R \to \R$ are some
%% functions depending only on the squared Euclidean norm of $\xk$ and
%% $\xkd$. Assuming that this power series converges for any $\xk,\xkd
%% \in \RR^d$ would be overly restrictive. In fact, we only
%% require that it converges in certain neighbourhoods of the hyper
%% sphere. More detailed, we assume that the kernel function $k:
%% \RR^d\times \RR^d \to \RR$ satisfies the
%% following assupmtions.




\begin{itemize}
\item[(A.1)] \textit{Kernel has a local power expansion}:
  Define the neighborhood $\convergeset{\delta}{\delta'} \subset \R^d \times \R^d$  as
  \begin{equation*}
    \convergeset{\delta}{\delta'} := \{(\xk,\xkd) \in  \R^d \times \R^d \mid (\|\xk\|_2^2, \|\xkd\|_2^2) \in [1-\delta, 1+\delta] \times
  [1-\delta, 1+\delta]\}.
  \end{equation*}
  
  A kernel $\kernf$ has a local power expansion if $\rotkerfunc$ can be expanded as a power series
  \begin{equation}
    \label{eq:kerneldefg}
    \kerfunc{\xk}{\xkd}= \rotkerfunc(\|\xk\|_2^2, \|\xkd\|_2^2, \xk^\top \xkd) = \sum_{j=0}^{\infty} \rotkerfunccoeffj{j}(\|\xk\|_2^2,\|\xkd\|_2^2) (\xk^\top \xkd)^j 
   \end{equation}
   that converges in a neighborhood $\convergeset{\delta,\delta'}$ of the sphere for some $\delta, \delta'>0$ and where $g_i$ is
  $(\floor{2/\beta}+1-i)$-times continuously differentiable in an
  neighbourhood of $(1,1)$. In addition, we assume that there exists $\jthresh > \floor{2/\beta}$ such that $\rotkerfunc_{\jthresh}(1,1) >0$.
  %%   In  particular, there exists a power series as described in Equation
  %% \ref{eq:kerneldefg}, for which we can find $\delta>0,\delta'>0$ such
  %% that for any
  %% $(x,x') \in \RR^d \times \RR^d$, with
  %% $(||\xk||_2^2, ||\xkd||_2^2) \in [1-\delta, 1+\delta] \times
  %% [1-\delta, 1+\delta]$ and $\xk^\top \xkd \in [-\delta',\delta']$, the
  %% power series converges and equals $k(\xk,\xkd)$.  In particular, we
  %% assume that the function $g$ from Equation \ref{eq:kerneldefg} is
  %% continuous and for any $i \leq \floor{2/\beta}+1$, $g_i$ is
  %% $(\floor{2/\beta}+1-i)$-times continuously differentiable in an
  %% neighbourhood of $(1,1)$.
\item[(A.2)] \textit{Positive Definiteness:} Any function $g_i$ from Assumption A.1 is a positive definite kernel function.
\item[(A.3)] \textit{Restricted Lipschitz
  Continuity:} The restriction of $k$ on $\{(x,x)| x \in \R^d,
  \| x \|_2^2 \in [1-\delta_L, 1+\delta_L]\}$ is
  a Lipschitz continuous function for some constant $\delta_L>0$.
\end{itemize}


The assumption A.1 guarantees that the kernel function $k$ is sufficiently smooth around the unit sphere. We will make heavily use of the power series representation given in Equation \ref{eq:kerneldefg}. The additional assumption that there exists $\jthresh > \floor{2/\beta}$ such that $\rotkerfunc_{\jthresh}(1,1) >0$ is needed in order to lower bound the Eigenvalues of the kernel matrix.  Assumption A.2 is a stronger statement than positive definiteness and plays also an important role in the proof of the main Theorem when lower bounding the Eigenvalues of the kernel matrix. Note that this assumption is trivially guaranteed if $k$ is an inner product kernel and $\rotkerfunc_i \geq 0$. We point out that similar assumptions to A.1-A.2 have been made in \cite{Ghorbani20,Liang20b} where only inner product kernels are studied. Finally, assumption A.3 will be needed in the proofs to control the diagonal that the diagonal of the kernel matrix $\kermat$. 
We remark that the Assumptions A.1-A.3 apply to a very broad
range of kernels including RBF, inner product and NTK kernels. More
generally, any inner product kernel $\kerfunc{\xk}{\xkd} =
\rotkerfunc(\xk^\top \xkd)$ with $\rotkerfunc$ locally analytic around
zero satisfies the assumptions given that the Taylor series has only non negative coefficients and at least one non zero coefficient of order higher than $\floor{2/\beta}$. 
%% This fact
%% follows  trivially  from  the  local  Taylor  expansion  around  zero,
%% $h(\xk^\top\xkd) = \sum_{j=0}^{\infty} h_i  ~ (\xk^\top \xkd)^j$.
In addition,
Proposition ~\ref{prop:ntkass}  shows that  the Assumptions  also hold
true for the NTK  kernels of any depth and a broad range of different
activation functions. Among the RBF kernels, we can show that the Gaussian kernel $k(\xk,\xkd)$ satisfies the assumptions, which can be seen from $\exp(- \| \xk - \xkd \|_2^2) = \sum_{j=0}^{\infty} \frac{2^j}{j!} (\xk^\top\xkd)^j \exp(\|\xk|\_2^2 + \| \xkd \|_2^2)$. Yet, it is not exactly which other RBF kernel functions satisfy the Assumption B.3. We refer to the Section \ref{sec:AppendixRBF} for a more detailed treatment of RBF kernels. 
\newline
While the mentioned kernels are all defined for input data on $\mathbb{R}^d$, we will also study the case where the input data lives on the hyper sphere $\Sphere{d}$. As a result, for this case it is sufficient to require that the assumptions A.1 and A.2 hold true for the restriction of the kernel function onto the hyper sphere $ \kernfuncressphere{d}$. In fact, assumption A.2 holds trivially true since any inputs $\x$ has norm $1$ by assumptions. Furthermore, we know from \citet{Schoenberg1988} that any continuous rotational symmetric function on the hyper sphere can be written as an inner product kernel, i.e. $\kernfuncressphere{d}(\xk,\xkd) = \rotkerfunc(\xk^\top \xkd)$, which we know from the previous discussion satisfies assumption A.1-A.3 under weak assumptions. 
\paragraph{Data Distribution and scale parameter}
In this paper we consider a standard covariance model and its
projection onto the sphere. The asymptotic regime is then defined
using the trace of the covariance in both cases.

\fy{can be automated
  to have this format. with some alpha notation} 

\begin{itemize}
\item[(B.1)] \textit{Covariance model}: The random input vectors $X
  \sim \prob_X$ have mean $0$ and covariance $\Sigma$. They are
  defined as $X = \inputcov^{1/2} \standardrv $ where 
  $\standardrv \in \R^d$ has i.i.d. entries of zero mean and unit
  variance. In addition, we assume that either each entry is normally
  distributed or bounded a.s.  by a constant $c>0$. %Finally, we
  assume wlog that $\| \inputcov \|_2 = 1$.
\item[(B.2)] \textit{High Dimensional regime}:
  We assume that the trace of $\inputcov$ grows with the sample size $\numobs$ as $\frac{\trace(\inputcov)}{\|\inputcov\|_2} \asymp n^{\beta}$ with $\beta \in (0,1]$. In the sequel we assume w.l.o.g. $\|\inputcov\|_2 = 1$ for simplicity.

\end{itemize}

%% More generally, our high-dimensional regime covers
%% $\frac{\trace(\inputcov)}{\|\inputcov\|_2} \asymp n^\beta$
%% Note that
%% the only restriction which we impose on the dimension $d$ of the input
%% data $d$ is that $\trace(\inputcov) \leq d$, which is a consequence of
%% the fact that $\| \inputcov \|_2 = 1$. Together with the assumption
%% that $\trace(\inputcov) \asymp n^{\beta}$, we cover a very broad range
%% of settings including the ones studied in
%% \cite{ElKaroui10,Liang20a,Liang20b}.
%% \newline Furthermore, we study the case where the data
%% is obtained by normalising $\xi{i}$, i.e.
%% \begin{equation}
%%     \s_i =\xind{i}/ \|\xind{i} \|_2^2
%% \end{equation}
%% This results in the case where the data is distributed on the hyper sphere. As a consequence, our results can be extended to cover the settings studied by \citet{Ghorbani19,Ghorbani20}.


In our analysis, the kernel function $\rotkerfunc$ \fy{not sure how to
  call it} itself stays constant for any $d$. However as
$\trace(\inputcov), n\to\infty$ we need to adjust the scaling of the
input since the norm concentrates around $\EE~ \| \x \|_2^2 =
\trace(\inputcov)$. 
Hence, as $\numobs \to\infty$, we consider the sequence of scale
dependent kernels
\begin{equation}
  \label{eq:scalekernel}
  \sckerfunc{\bw}{x}{x'} = \rotkerfunc\left(\frac{\|\xk\|_2^2}{\bw},
  \frac{\|\xkd\|_2^2}{\bw}, \frac{ \xk^\top \xkd}{\bw}\right)
\end{equation}
where $\bw$ can vary with sample size $\numobs$. For RBF $\bw$ is
simply the bandwidth, for inner product kernels and NTKs, it's usually
set to $\bw=d$
\cite{Ghorbani19,Ghorbani20,ElKaroui10,Liang20a,Liang20b,Liu20}. The
scaling is especially crucial for NTK, where the
correspondence with infinitely wide Neural Network can, to the best of
our knowledge, only be shown for test samples $\bw \Xrv$ on the hyper
sphere \cite[Theorem~3.2]{Arora19}.  In Section~\ref{sec:tauconst} we
consider the standard scaling $\bw = \effdim$ before analyzing
$\frac{\bw}{\effdim} \to 0$ and $\to\infty$ respectively in
Section~\ref{sec:otherbw}.

%respectively $\kernfsphere$ \fy{this is
%  not true, the $\kerfunc$ changes domain so can't stay the same}
%% remain the same for any $d$. To react on the change of the dimension
%% $d$, we study scale dependent kernels $k_{\bw}$ with
%% $\sckerfunc{\bw}{x}{x'} = \rotkerfunc(\frac{\|\xk\|_2^2}{\bw},
%% \frac{\|\xkd\|_2^2}{\bw}, \frac{ \xk^\top \xkd}{\bw}) $. 
%% The
%% assumption that the kernel function depends on a scale parameter which
%% changes with respect to $d$ is common practice in the literature
%% \cite{Ghorbani19,Ghorbani20,ElKaroui10,Liang20a,Liang20b,Liu20}, where
%% all cited papers choose $\bw = d$.
%% We remark that in the asymptotic setting, some dependence of
%% $\bw$ on $d$ is required in order to adapt to the changing
%% norm of the vectors $\xind{i}$.
%% More, generally, the expected norm depends on the effective dimension
%% \begin{equation}
%%   \label{eq:effdim}
%%     \effdim \define \EE~ \| \x \|_2^2  = \trace(\EE \x \x^\top) = \trace(\inputcov) 
%% \end{equation}
%% Most of the discussion in this paper will focus on the choice of
%% $ \bw = \effdim$. We also provide ...


%%%%%%%%%% Relating setting to previous works %%%%%%%%%%
\paragraph{Generality of our setting}
Our setting and assumptions cover a very broad range of
settings. First of all, we directly recover the setting studied in the
papers \cite{ElKaroui10,Liang20a,Liu20} when $d \asymp n$ and
$\trace{\inputcov} \asymp d$ and the one studied in the paper
\cite{Liang20b} when $d \asymp n^{\beta}$ and $\inputcov =
\idmat_d$. Note that we also cover the case
$\frac{\trace{\inputcov}}{d}\to 0$ if $d\gg \numobs^\beta$. In
\cite{Liang20a}, they choose $\bw = d$ and hence
$\frac{\bw}{\effdim}\to \infty$, a case we \kd{discuss instead of cover ?}cover in
Section~\ref{sec:otherbw} \fy{sth like that..?} Furthermore we recover
\cite{Ghorbani19, Ghorbani20}, by choosing $\inputcov = \idmat_d$
respective $\inputcov = (r^2-1)UU^\top + I$ (using notation as in
\cite{Ghorbani20} Sec 2.1.) and projecting the data onto the
sphere. The following table summarizes our setting vs. the ones
in the literature.
\fy{insert sth like the table here}

%% The motivation for our choice of the
%% scale parameter is that the re-scaled inputs have squared mean
%% $\EE \| \bw \xind{i} \|_2^2 =1$.

%% \fy{completely rewrite}
%%  We remark that our choice of
%% the scale parameter only agrees with the one from the mentioned paper
%% if $\effdim = d$. While this is the case for the paper
%% \cite{Liang20b} and also for the paper \cite{Ghorbani19} when
%% projecting onto the hyper sphere, we remark that this is only the case
%% for the papers \cite{ElKaroui10,Liang20a,Liu20} if $\trace(\inputcov)
%% \asymp d$.


%% \paragraph{Kernel regression}

%% Don't see how we need this
%% As a consequence, we can see that
%% the bias $\Bias(\fhatridge)$ can be expressed as
%% \begin{equation}
%% \label{eq:biassimplified}
%%    \Bias(\fhatridge) = \EE_{X} \| \EE_y \fhatridge(X) - \ftrue(X) \|^2, 
%% \end{equation}
%% where $\ftrue(\textbf{\x})$ is the vector with entries $\ftrue(\datamatrix)_i
%% = \ftrue(\xi{i})$ and $\kstar(X)$ is the vector with entries $\kstar_i =
%% k_{\tau}(\xind{i}, X)$. Finally, the same applies for the spherical input
%% data, where for some random input $\Srv$ on the hyper sphere
%% $\Sphere$, we write $\kstar_{\Sphere}$ instead of $\kstar(X)$,
%% $\kermat_{\Sphere}$ instead of $\kermat$ and $\ftrue(\Ss)$ instead of
%% $\ftrue(Xs)$.










==> sections/section3vB.tex <==





\section{Main Results}
\label{sec:4}


\kd{This paragraph needs to be completely rewritten} While there
exists multiple paper on kernel ridge and especially "ridge-less"
regression claiming that consistency can be reached for rotationally
symmetric kernels in high dimensional regimes
\cite{Liang20a,Liang20b,Liu20,Ghorbani19,Ghorbani20}, we highlight
that the current literature is unclear about the set of ground truth
functions for which this is true. On the one hand,
\citet{Ghorbani19,Ghorbani20} showed that we can at most approximate
polynomials of a certain degree when assuming that the input data sets
are drawn from the uniform distribution on the hyper sphere,
respectively on the product of two hyper spheres of different
radii. In contrast, on the other hand, in the papers
\cite{Liang20a,Liang20b,Liu20} linear covariance data models are
studied, where less restrictive assumptions on the ground truth
function are imposed. In particular, these results do not limit the
ground truth function to polynomials. In the last section, we have
already questioned the applicability of the bias bound from
\cite[Theorem~3]{Liang20a}. Still, it is yet unclear how the
discrepancy in the results for the linear covariance data models
\cite{Liang20b,Liu20} with the ones for spherical input data
\cite{Ghorbani19,Ghorbani20} can be reached can be explained.

In this paper we take a different approach and show that the estimator
of kernel ridge and "ridge-less" regression looks asymptotically
almost everywhere like a polynomial. As a result, we can conclude that
consistency can be only reached for a limited set of ground truth
functions. Our results therefore build upon the intuitions gained from
the papers \cite{Ghorbani19,Ghorbani20} and extend them to a much
broader class of data distributions. \kd{Not sure how
  much more we need to say here- i feel it becomes a bit
  repetitive. }  \kd{Say something like in a first step
  of this section blabla}



\begin{figure}[t!]
    \centering
    \includegraphics[width=0.3\textwidth]{Plots/sin_curve_1.png}
    \includegraphics[width=0.3\textwidth]{Plots/sin_curve_5.png}
    \includegraphics[width=0.3\textwidth]{Plots/sin_curve_40.png}

    \caption{Toy Example}{blabla}
    \label{fig:rkhsnorm}
\end{figure}


\subsection{Consistency for kernel regression}
\label{sec:tauconst}
We can now state the main result of this paper. Let $\polyspace{m}$ be
the space of polynomials of degree at most $m$. Throughout this section, the results in this section
hold for the scaling $\bw \asymp \effdim$ as defined in ~\eqref{eq:effdim}. 

%%%%%%%%%%%%%%%%%%%%5%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% Theorem: Poly approx %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{theorem}[Consistency for polynomials]
  \label{thm:main_thm}
  Assume that the kernel function $\kernf$, respectively its restriction onto the unit hyper sphere $\kernfuncressphere{d}$, satisfies the Assumptions A.1-A.3. Let $X$ be some random variable drawn form the data distribution and define $m$ as:
\begin{enumerate}
    \item  For $X$ drawn form a distribution that satisfies
  Assumptions B.1-B.2 we define $m = 2
      \floor{2/\beta}$. 
      \item For $X = \frac{Z}{\|Z\|}$ with $Z$ drawn from a
      distribution that satisfies
      Assumptions B.1-B.2 we define $m = \floor{2/\beta}$. 
\end{enumerate}
Then, the following result holds for any ground truth that is bounded $|\ftrue| \leq \ubfunc$
  almost surely for some $\ubfunc > 0$. The bias of the kernel ridge and ridgeless estimators
  $\fhatridge$ is asymptotically lower bounded for any $\gamma > 0$ as
  $n\to \infty$,
  \begin{equation}
    \label{eq:biaslb}
    \Bias(\fhatridge) \geq \underset{\polyf \in
      \polyspace{m}}{\inf} \EE_{X} \left| \ftrue(\Xrv) -
    \polyf(\Xrv)\right|^2 - \gamma ~~~a.s..
  \end{equation}
  Furthermore, there exists constants $\epsd >0$ and $\Cgenprob{\epsd}$ such that with probability $\geq 1- \exp(-\Cgenprob{\epsd}
  \log(n)^{1+\epsd})$ over the draws of a test sample $\Xrv$, for any
  $\eps$ there exists a polynomial $\polyf \in \polyspace{m}$ so that
  \begin{equation}
    \label{eq:polyapprox}
    \left| \EEobs \fhatridge(\Xrv) - \polyf(\Xrv) \right| \leq \epsilon
    ~~ a.s.,
  \end{equation}
  where $\EEobs \fhatridge(\Xrv)$ is the estimator with expectation
  taken over the observation noise.
  
  

  %%   The results hold trivially for $\lambda \geq c > 0$ and for decaying
  %% $\lambda \to 0$ and $\lambda = 0$ (the minimum norm interpolator
  %%   $\fhatinterpol$ in~\eqref{eq:constraint_min_p}) if the
  %%   eigenvalues of $\kermat$ are lower bounded by a positive constant for all $n$.   
\end{theorem}

% Now we can mention the kernels again which satisfiy the assumptions A.1-A.3 in words. 

As already discussed in the previous section, a broad spectrum of different practically relevant kernels such as the inner product kernels, the NTK kernels and the Gaussian kernel satisfies the Assumptions in the Theorem \ref{thm:main_text}. Furthermore, we can weaken the Assumption A.1-A.2 such that we can also show that they include general RBF kernels. However, in order to show guarantee that Theorem \ref{thm:main_thm} still applies, we now require that the Eigenvalues of the kernel matrix $\kermat$ can be lower bounded by a non zero positive constant. We refer to Corollary \ref{cr:RBFmain_thm} for the precise statement. As a consequence, we can show that the results from Theorem \ref{thm:main_thm} also applies to the $\alpha$-Exponential kernels for general $\alpha$. 
\kd{We can merge it with the main theorem, but i find this quite elegant.}
\begin{prop}
The results form Theorem \ref{thm:main_thm} also apply for the $\alpha$-Exponential kernel when $\alpha <2$.
\end{prop}






%% Assume that the Assumption A.1-A.3 hold true and the assumption
%% B.1-B.2 for the kernel $k$, respectively the Assumption
%% $\tilde{\textrm{B}}$.1 for the kernel $\kerns$.  Furthermore, assume
%% that the minimum Eigenvalues of $(\lambda \textrm{I}_n + \kermat)$,
%% respectively $(\lambda \textrm{I}_n + \Ks)$ are almost surely lower
%% bounded by a non zero positive constant. Let $m =\floor{2/\beta}$. We
%% have that:
%% \begin{enumerate}
%% \item
%% For any $\epsilon>0$ and any $n$ sufficiently large, there exists a polynomial $p \in \mathcal{P}_{\leq 2m}$, such that  with probability $\geq 1- \exp(-C \log(n)^{1+\epsd})$ over the draws of  $X$,
%% \begin{equation}
%% \label{eq:degenratedf}
%%     \left| f^*(\datamatrix)^\top (K + \lambda \textrm{I}_n)^{-1} \kstar(\Xrv) - p(\Xrv) \right| \leq \epsilon ~~ a.s.,
%% \end{equation}
%% and similarly there exists a polynomial $p_{\mathcal{S}} \in \mathcal{P}_{\leq m, \mathcal{S}}$ such that with probability $\geq 1- \exp(-C \log(n)^{1+\epsd})$ over the draws of  $S$,
%% \begin{equation}
%% \label{eq:degenratedf}
%%     \left| f^*(\Ss)^\top (\Ks + \lambda \textrm{I}_n)^{-1} \kstars(\Srv) - p_{\mathcal{S}}(\Srv) \right| \leq \epsilon ~~ a.s.,
%% \end{equation}
%% with $\epsd>0, C>0$ some positive constants.
%% \item
%% For any $C\geq C_{f^*}$, any $\gamma >0$ and any $n$, the bias can be lower bounded by 
%% \begin{equation}
%%     \textbf{B}(\hat{f}_{\lambda})  \geq  \underset{\overline{p} \in \overline{\mathcal{P}}_{\leq 2 m,C}}{\inf} \mathbb{E}_{X} \left| f^*(X) - \overline{p}(X)\right|^2  - \gamma ~~~a.s,
%% \end{equation}
%% and similarly, 
%% \begin{equation}
%%         \textbf{B}(\hat{f}_{\lambda,\mathcal{S}})  \geq  \underset{\overline{p_{\mathcal{S}}} \in \overline{\mathcal{P}}_{\leq m,C, \mathcal{S}}}{\inf} \mathbb{E}_{\Srv} \left| \ftrue(\Srv) - \overline{p}_{\mathcal{S}}(\Srv)\right|^2  - \gamma ~~~a.s.
%% \end{equation}
%% \end{enumerate}
%% \end{theorem}




\paragraph{Proof sketch}
 For the brevity of the notation, we call $\zind{i} = \sqrt{\bw}\xind{i}$ and $\Zrv = \sqrt{\bw} \Xrv$ where $\Xrv$ is a random variable independently drawn form the same distribution as $\xind{i}$. Essentially, any of the presented results are a consequence the strong concentration of Lipschitz continuous functions of vectors of i.i.d random variables \cite[Corollary~4.10]{Ledoux2001}. As a consequence, we will show in Corollary \ref{cr:testsample} that for any $\eps >0$, with high probability over the draws of $\Zrv$,
\begin{equation}
\label{eq:oultineproof}
    \underset{i}{\max}\left| \zind{i}^\top \Zrv \right| \leq n^{-\beta/2}(\log n)^{1+\epsilon}
\end{equation}
Here, we only provide the main intuition for the proof of Theorem \ref{thm:main_text} for the case where the kernel function $k$ is an inner product kernel. This is offers the simplest way to gain an intuition for the phenomenon causing the bias to be bounded. As a consequence of the concentraiton inequality from Equation \ref{eq:oultineproof}, we can show that we can discard the higher order term of the Taylor series approximation:
\begin{equation}
    \kernf(\zind{i},\Zrv) = \sum_{j=0}^{m} g_j ~ (\zind{i}^\top\Zrv)^j + O\left(n^{-(m+1)\beta/2} (\log n)^{(m+1)(1+\epsilon} \right) ~~a.s..
\end{equation}
Since we choose $m = \floor{\beta/2}$, we can see that $n \left(n^{-(m+1)\beta/2} (\log n)^{(m+1)(1+\epsilon}\right) \to 0$. As a result, the kernel function $k$ looks like a polynomial of degree at most $m$ plus an error term which vanishes at rate $o(n^{-1})$ with high probability over the draws of $\Zrv$ and almost surely over the draws of $\Z = \{\z_1,...,\z_n\}$ .


The proof hinges on the closed-form expression of the ridge(less)
estimate.  For some $x\in \X$, let $\kerx{x} \in \R^n$ be the
vector with entries $\kerx{x} = k_{\bw}(\xi{i}, x)$. For any $\lambda
>0$ we can write obtain
\begin{equation}
\label{eq:kernelridge}
    \fhatridge(x) = \y^\top (\kermat + \lambda \idmat_n)^{-1}\kerx{x}.
\end{equation}
As a next step, we show that
\begin{equation}
\label{eq:sec4outlinproof}
   \EE_Y \fhatridge(X) = \ftrue(\Xrv)^\top (\kermat + \lambda \In)^{-1}\kerx{\Xrv} = \sum_{i=0}^n \sum_{j=0}^{m} g_j ~ (\zind{i}^\top\Zrv)^j + o(1)~~a.s.,
\end{equation}
holds true with high probability over the draws of $\Xrv$. Here, we use the assumption that the Eigenvalues of $\kermat+ \lambda \In$ are lower bounded. The rest of the proof is then just a straight forward application of this fact. \qed


For decreasing risk estimates and the minimum norm interpolator
Theorem~\ref{thm:main_thm} requires that the $\kermat+ \lambda \In$ is
asymptotically lower bounded by a positive constant. The following
proposition characterizes for which kernels this condition is satisfied.
%% which is due to the well known Representer Theorem, \fy{schoelkopf
%%   didn't invent representer theorem, too standard to cite}
%% For interpolation, 
%% we assume
%% that the kernel matrix $K$ is almost surely invertible with respect to
%% the draws over the data sets $\datamatrix$. We remark that this assumption is
%% guaranteed to be the case for any universal kernels such as the
%% Gaussian or Laplacian RBF kernels.

%% Clearly, whenever $\lambda$ does not go to zero but
%% instead is lower bounded by some positive constant, the Eigenvalues of
%% $ \lambda \In + K$ are also lower bounded and therefore Theorem
%% \ref{thm:main_text} applies for any of the kernels satisfying the
%% Assumptions B.1 and
%% $\tilde{\textrm{B}}$.4-$\tilde{\textrm{B}}$.5. \fy{see it would be better to be able to reference so that you don't have undefined references} Unfortunately, this is
%% not guaranteed for the minimum norm interpolant when the ridge parameter $\lambda\to 0$.  Showing that this holds true for different kernels is the main
%% technical challenge of this paper. In fact, we can show that:
\fy{mention that we need at least universality}
\kd{No, we just need that the kernel matrix $\kermat$ is almost surely invertible}
%%%%%%%%%%%%%%%%%%%%5%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% Proposition lower bounded EV %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% \kd{changed the proposition}

% \begin{prop}[Lower bounded kernel eigenvalues]
%   \label{prop:kernelslowerboundev}
%   The eigenvalues of the kernel
%   matrix $\kermat$ can be almost surely lower bounded by a non zero
%   positive constant $c>0$ for any $n$, 
% \begin{enumerate}

% \item in the case when $\Xrv$ is drawn from a distribution that satisfies Assumptions
%   A.1-A.2, for the following kernel functions:
%   \begin{enumerate}
%   \item Any inner product kernel with Taylor expansion
%     $\kerfunc{\xk}{\xkd} = \rotkerfunc(\xk^\top \xkd) =
%     \sum_{j=0}^{\infty} \rotkerfunccoeff ~(\xk^\top \xkd)^j$ with
%     $\rotkerfunccoeff \geq 0$ and $\jthresh > \floor{2/\beta}$ such
%     that $\rotkerfunccoeffj{\jthresh} > 0$.
%   \item The $\alpha$-exponential kernel $k(\xk,\xkd) =
%     \exp(-\| \xk- \xkd \|_2^{\alpha})$ with
%     $\alpha \in (0,2)$.
%   \item Any neural tangent with a homogeneous activation function and Hermit polynomial extension with coefficients $\hermitcoeff \in \RR$ and $\jthresh > \floor{2/\beta}$ such that $\hermitcoeffj{\jthresh}$. In particular, this holds true for the Relu activation function $\actfun{\xk} = \max(0,\xk)$. \kd{This is a bit long - but i do not want to introduce homogenity and Hermit poly extension here}
%   \end{enumerate}
  
% \item in the case when $\Xrv = \frac{Z}{\|Z\|}$ with $Z$ drawn from a
%   distribution that satisfies Assumptions A.1-A.2, for all of the
%   above kernels and more generally, any kernel $k$ where the restriction on the unit hyper sphere $\kernfuncressphere{d}$ satisfies the assumptions from (1.a).  
% \end{enumerate}
% \end{prop}



% \begin{prop}[Lower bounded kernel eigenvalues]
%   \label{prop:kernelslowerboundev}
%   The eigenvalues of the kernel
%   matrix $\kermat$ can be almost surely lower bounded by a non zero
%   positive constant $c>0$ for any $n$, 
% \begin{enumerate}

% \item in the case when $\Xrv$ is drawn from a distribution that satisfies Assumptions
%   A.1-A.2, for the following kernel functions:
%   \begin{enumerate}
%   \item Any inner product kernel with Taylor expansion
%     $\kerfunc{\xk}{\xkd} = \rotkerfunc(\xk^\top \xkd) =
%     \sum_{j=0}^{\infty} \rotkerfunccoeff ~(\xk^\top \xkd)^j$ with
%     $\rotkerfunccoeff \geq 0$ and $\jthresh > \floor{2/\beta}$ such
%     that $\rotkerfunccoeffj{\jthresh} > 0$.
%   \item The $\alpha$-exponential kernel $k(\xk,\xkd) =
%     \exp(-\| \xk- \xkd \|_2^{\alpha})$ with
%     $\alpha \in (0,2)$.
%   \item Any neural tangent with a homogeneous activation function and Hermit polynomial extension with coefficients $\hermitcoeff \in \RR$ and $\jthresh > \floor{2/\beta}$ such that $\hermitcoeffj{\jthresh}$. In particular, this holds true for the Relu activation function $\actfun{\xk} = \max(0,\xk)$. \kd{This is a bit long - but i do not want to introduce homogenity and Hermit poly extension here}
%   \end{enumerate}
  
% \item in the case when $\Xrv = \frac{Z}{\|Z\|}$ with $Z$ drawn from a
%   distribution that satisfies Assumptions A.1-A.2, for all of the
%   above kernels and more generally for any rotation invariant kernel
%   for which the series expansion $\kerfunc{\xk}{\xkd} =
%   \sum_{j=0}^{\infty} \rotkerfunccoeff ~(\xk^\top \xkd)^j$ as in
%   Equation~\eqref{eq:Scheonbergseries} only has non-negative
%   coefficients $\rotkerfunccoeff \geq 0$, and there exists $\jthresh >
%   \floor{2/\beta}$ such that $\rotkerfunccoeffj{\jthresh} > 0$.
% \end{enumerate}
% \end{prop}

In fact, we can show a much more general result for the case where the
input data is $\datamatrix$ than the one presented in Proposition
\ref{prop:kernelslowerboundev}. However, we remark that it is not
trivial to verify that these assumptions hold true for arbitrary
kernels. We refer to Proposition \ref{prop:Evlowerbound} in the
Appendix for the statement and a discussion on the applicability of
this proposition.



\fy{significantly cut and probably move parts before proof sketch}

Surprisingly, we find that bound from Theorem ~\ref{thm:main_text}
depends only on the growth rate of the trace $\trace(\inputcov)$ with
respect to $n$, but not on the explicit structure of the covariance
matrix $\inputcov$. Hence, given that $\beta$ is some constant, we find
that the Bias $\textbf{B}(\hat{f}_{\lambda})$ never vanishes if the
ground truth is sufficiently non linear. In fact, our results do not
depend on the sparsity of the ground truth function, meaning that the
issue also holds true for arbitrarily sparse ground truth
functions. As a consequence, we prove the intuitions gained from
\cite{Ghorbani19} who shows a stronger version of Theorem
\ref{thm:main_text} for the uniform distribution on the hyper sphere.
As a result, we can see that we can never reach consistency if the
projection error of the ground truth function onto the space of
truncated polynomials is not vanishing, respectively zero. Finally, we
mention \cite[Theorem~4]{Bartlett20}, where it was shown that for the
linear regression the explicit structure of the data covraiance matrix
plays an important role to determine whether consistency can be
reached. While this result leads to the question whether the explicit
structure of the covariance matrix also determine consistency for
kernel regression, our analysis clearly shows that this is not true
for general non linear functions. \newline Interestingly, our proof
does not just only imply that the bias does not vanish, but also that
the noiseless estimator looks asymptotically almost everywhere like a
polynomial. This clearly demonstrates that both kernel ridge and
"ridge-less" regression have an implicit bias towards simple models in
high dimensions, which is also responsible for the non vanishing bias
if the ground truth function is sufficiently non polynomial. Finally,
we remark that Proposition \ref{prop:poly} can also applies for the
estimator $\hat{f}_{\lambda}$ even when noise is present under the
assumption that the observation noise is bounded. \newline We will now
discuss the implications for the three explicit examples of kernels
mentioned in Proposition \ref{prop:kernelslowerboundev}.

\textbf{Inner Product Kernels:} 
\kd{ Need to rewrite:}
The inner product kernels are widely used in the literature \cite{Liang20b,Liu20,Liang20a,Ghorbani19,Ghorbani20,ElKaroui10} which allows a good comparison with the existing results. In particular, \citet{Liang20b} claims that the risk vanishes in regimes where $d \asymp n^{\beta}$ with $\beta \in (0,1)$ and $\inputcov = \textrm{I}_d$. While it is not exactly clear which ground functions satisfy the assumption in the paper \cite{Liang20b}, as a consequence of our results, we can clearly show that this is not true given that the ground truth function $f^*$ is not a polynomial of degree at most $\floor{2/\beta}$.

\textbf{The role of eigenvalue decay} The second example of kernels
for which we can show that Theorem ~\ref{thm:main_text} applies are the
$\alpha$-Exponential RBF kernels of the form $k(\xk,\xkd) =
\exp(-\| \xk - \xkd \|_2^{\alpha})$ with special
cases including the Laplace kernel ($\alpha =1$) and the Gaussian
kernel ($\alpha = 2$). These kernels have shown strong performance on
multiple high dimensional data sets as shown in the papers
\cite{Geifman20,Belkin18a}. In addition, we can see from
\cite[Theorem~2.1]{Blumenthal60} that these kernels cover a broad
spectrum of different Eigenvalue decays, including both exponential
decay, i.e. when $\alpha =2$, and a broad range of polynomial decays,
i.e. when $\alpha <2$. As a consequence, we can conclude that the
phenomenon described in Theorem ~\ref{thm:main_text} and Corollary
~\ref{prop:poly} appears to be independent of the Eigenvalue decay of
the kernels. Furthermore, our results indicate that the strong
performance observed in \cite{Geifman20}

\textbf{Neural Tangent Kernels:} 

\kd{Thanks to Parnians hint, our statements hold for many more activation functions than just Relu :)}

As a last example, we discuss the Neural Tangent Kernels (NTK) with
activation function. Interestingly, from the above discussion, we know
that the NTK of any depth satisfies the assumptions in Corollary
~\ref{prop:Evlowerbound} and thus also in Theorem
~\ref{thm:main_text}. These results extend the observations for NTK's
on the Hyper sphere by \citet{Ghorbani19,Ghorbani20}. Furthermore, we
remark that the benefits of the depth for NTK kernels has also been
questioned in the paper \cite{Bietti20}. However, our results are
orthogonal to the results of \citet{Bietti20}, because their main
argument is that the NTK of any depth has the same Eigenvalue
decay. Since our results do not depend on the Eigenvalue decay, we
highlight that our observation that the depth does not help to
overcome the bias bound from Theorem ~\ref{thm:main_text} is not a
consequence of the results form the paper \cite{Bietti20}.


\subsection{Alternative choices of the scale parameter $\bw$}
\label{sec:otherbw}


\fy{I have to say I find it nicer to think about normalization constants (i.e. use BW vs $\bw$ and then ratios of constants, rather than have $\bw \effdim$. You then don't need to do acrobatics in your head each time :D}
  \begin{figure}
     \centering
     \minipage{0.49\textwidth}
          \centering
  \includegraphics[height=4cm]{Plots/taudependencyNew.png}
  \label{fig:awesome_image1}
\endminipage\hfill

\caption{Dependency of the bias on $\bw$}{ The bias is plotted with
  respect to $\bw$ for different choices of $\beta$ and for the
  Laplace and Gaussian kernels. Details for the plot are given in Section \ref{sec:experimentssynthetic}}
\label{fig:exp2}
 \end{figure}


\label{sec:additionalresults}

How about write: Before, $\bw \effdim \asymp 1$.
Here we consider the regimes $\bw \effdim \to \infty$ 

This subsection studies different cases where $\bw$ is not equal to
$\frac{1}{\effdim}$. Clearly, it is not difficult to verify that we
can extend Theorem \ref{thm:main_text} to the case where $\bw \asymp
\frac{1}{\effdim}$. Hence, we are only interested in settings where
$\bw = o(\frac{1}{\effdim})$ or $\bw =
\omega(\frac{1}{\effdim})$. Unfortunately, since this Lemma
\ref{lm:innerpr} implies that in this case, the norm of $\bw
\xind{i}$, $ \| \bw\xind{i} \|_2^2 $, either almost surely diverges
or goes to zero, we cannot make the same general statement as
before. The following paper proves for the $\alpha$-exponential kernel
$\kerfunc{\xk}{\xkd} = \exp(-\| \xk-\xkd \|_2^{\alpha})$ with $\alpha \in
(0,2)$ how the kernel estimator cannot be overcome the polynomial approximation
barrier when $\bw\effdim\to\infty$ polynomially and $\bw\effdim \to 0$  


%%%%%%%%%%%%%%%%%%%%5%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% Theorem: different tau %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{theorem}
\label{thm:otherchoicesoftau}
Assume that the Assumptions in Theorem~\ref{thm:main_thm} hold
true. \fy{I think you need the same lower boundedness stuff for $\lambda \to 0$ as for Thm~\ref{thm:main_thm}?} Let $k$ be the $\alpha$-exponential kernel with $\alpha \in
(0,2)$. For any $\gamma>0$ and any $n$ sufficiently large, we have
that:
\begin{enumerate}
    \item If $\bw \to 0$ not fast enough, that is $\bw = \Omega(n^{-\beta+\epsilon})$ \fy{can we write instead $\bw\effdim = \Omega(n^\eps)$} with $\eps>0$, asymptotically as $n\to\infty$
    \begin{equation}
    \Bias(\fhatridge)\geq \EE_{\Xrv} \left| \ftrue(\Xrv) \right|^2 - \gamma  ~~~ a.s..
\end{equation} 
\item For the minimum norm interpolator, when $\bw \to 0$

\begin{equation}
     \lim_{\bw \to 0} \Bias(\fhatinterpol) \geq  \underset{\truncp \in \polyspacetrunc{m}{C}}{\inf} \EE{\Xrv} \left| \ftrue(\Xrv) - \truncp(\Xrv) \right|^2  - \gamma ~~~a.s.
\end{equation} 
\end{enumerate}
\end{theorem}

\kd{I will write this section after my talk tomorrow}
\fy{first is obvious - say in one sentence why - then second is hard}
%  In the "ridge-less" case, where $\lambda = 0$ and $\tilde{\bw} \overset{n\to \infty}{\to} 0$ the analysis turns out to be significantly more challenging. Here, we only study the extreme case where we analyse the flat limit, i.e. the solution obtained when for any fixed $n,d$ taking the limit of $\tilde{\bw} \to 0$,
% \begin{equation}
%     \forall n,d: ~~ \fhat_{\textrm{PS}}(\datamatrixtar) := \lim_{\tilde{\bw} \to 0} \fhat(\datamatrixtar) = \lim_{\tilde{\bw} \to 0} \y^\top  \kermat^{-1} \kstar.
% \end{equation}
% In general, it is not clear whether this solution exists. However, we can apply \cite[Theorem~3.12]{Lee2014} and \cite[Theorem~2.1]{Blumenthal60} to show that for any $\alpha \in (0,2)$, $\hat{f}_{\textrm{PS}}$ exists and exactly the \textit{Polyharmonic Spline Interpolator} introduced by \citet{Wahba90} with the closed form expression:
% \begin{equation}
%     \fhat_{\textrm{PS}}(\datamatrixtar) = \begin{pmatrix}y \\ 0 \end{pmatrix}^\top \begin{pmatrix} -D^{\alpha} & 1 \\ 1^\top & 0 \end{pmatrix}^{-1} \begin{pmatrix} d^{\alpha,*} \\ 1 \end{pmatrix}.
% \end{equation}
% % Here $D^{\alpha}$ is $n\times n$ matrix with entries $D^{\alpha}_{i,j} = \| \zind{i}-\zind{j} \|_2^{\alpha}$ and $d^{\alpha,*}$ is the vector with entries $d^{\alpha,*}_i = \| \zind{i} - \z^* \|_2^{\alpha}$ and with $\zind{i} = \bw\xind{i}$ and $\z^* = \bw \x^*$. We can now state the main theorem of this section. 




Theorem ~\ref{thm:otherchoicesoftau} shows that the bound on the bias
from Theorem ~\ref{thm:main_text} cannot be overcome in any of the
three studied cases. Surprisingly, we can see that the kernel
"ridge-less" regression differs significantly from the kernel ridge
regression with a constant non zero ridge parameter when $\tilde{\bw}
\to 0$. \fy{not surprising} Finally, we mention that \citet{Lee2014}
showed that the polyharmonic spline interplator $\fhat_{\textrm{PS}}$
is the flat limit of a much broad range of different kernel functions,
which implies that our results can be extended to a much broader class
of kernel functions. 

In this section, we discuss the relevance of regularisation in a
broader perspective and incorporate our results with the literature on
classical low dimensional settings. Our discussion concentrates again
on the setting described by the Assumptions A.1 and A.3, however, we
do not necessarily require that the regime is high dimensional,
i.e. Assumption A.2. Furthermore, in order to be able to apply the
classical results guaranteeing consistency, we require that the
support of $X$ is compact.

We call a kernel on a compact space $\XX$ \textit{universal} if its
corresponding RKHS is dense in the set of continuous functions
$C(\XX)$ with respect to the infinity norm
\cite[Definition~11]{Christmann07}. This definition applys to a braod
range of popular kernel functions including the Laplace kernel as
shown in \cite[Example~1]{Sriperumbudur11}. We can now summarise the
positive results on consistency of kernel ridge regression from
\cite[Thoerem~12]{Christmann07} and the negative results for the
special case of the Lapalace kernel by \citet{Rakhlin18} in the
following corollary:



Assume that the data is distributed according to Assumptions A.1 and
A.3. In addition, assume that the support of $X$ is compact and the
dimension $d$ is constant. Then, under a suitable choice of the ridge
parameter, kernel ridge regression for any universal kernel is
consistent. In particular, this holds true for the Laplace kernel.

In contrast, assume that the observations are generated by adding
$i.i.d$ Rademacher noise $\xi_i$ to the ground truth function,
i.e. $\y_i = \ftrue(\xi{i}) + \xi_i$ with $P(\xi_i = 1) = P(\xi_i =
-1) = 1/2$. Then, the kernel "rigde-less" regression for the Laplace
kernel is never consistent.

As a result of this corollary, we can see that regularisation is
explicitly required for the Laplace kernel to be consistent in fixed
dimensions $d$. Furthermore, as a result of our research, we can
conlcude:

As a result, we can conclude that the bias does never vanish when
$\ftrue$ is a highly non linear function. For instance, choosing
$\ftrue(\x) = \sin(\x_{(1)})$ would satisfy our assumptions and hence
can never be consistently learned in the described high dimensional
regimes. As a consequence of Corollary \ref{cr:lowdimcons} and
Corollary \ref{cr:highdimcons}, we can conclude that sufficiently non
polynomial functions in the sense that Equation
\ref{eq:polyrestriction} does not vanish can only be learned if the
input dimension is constant and regularisation is used.

